Hybrid Random Features

We propose a new class of random feature methods for linearizing softmax and Gaussian kernels called hybrid random features (HRFs) that automatically adapt the quality of kernel estimation to provide most accurate approximation in the defined regions of interest. Special instantiations of HRFs lead to well-known methods such as trigonometric (Rahimi and Recht, 2007) or (recently introduced in the context of linear-attention Transformers) positive random features (Choromanski et al., 2021). By generalizing Bochner's Theorem for softmax/Gaussian kernels and leveraging random features for compositional kernels, the HRF-mechanism provides strong theoretical guarantees - unbiased approximation and strictly smaller worst-case relative errors than its counterparts. We conduct exhaustive empirical evaluation of HRF ranging from pointwise kernel estimation experiments, through tests on data admitting clustering structure to benchmarking implicit-attention Transformers (also for downstream Robotics applications), demonstrating its quality in a wide spectrum of machine learning problems.

==> Hybrid Estimators (Camera-ready, Arxiv)/computation_arccos_kernels.tex <==
%% Add some of my results on arc cos kernels 
\subsection{Definitions and Some Results}
Arc cosine kernels introduced in~\cite{arccosnips, arccos} is defined as
\begin{equation}~\label{eqn:arccoskernel}
    k_n(x,y)  = 2 \int dw \frac{e^{\frac{-||w||^2}{2}}}{(2\pi)^{d/2}} \Theta(w\cdot x) \Theta(w \cdot y)(w \cdot x)^{n}(w \cdot y)^{n}.
     \end{equation}
     where, 
     $\Theta(x) = \frac{1}{2}(1+ \text{sign}(x))$ is the Heaviside function. 
     These kernels can be computed analytically for non-negative integers $n$ and moreover the integral converges for $n > - \frac{1}{2}$. 
     
    The above integral has a simple dependence on the magnitudes of $x$ and $y$ but a complicated relation on the angle $\theta$ between them. This dependence will be explored in detail below. Write, 
    \begin{equation}~\label{eqn:splitkernel}
        k_n(x,y) = \frac{1}{\pi} ||x||^{n}||y||^n J_n(\theta)
    \end{equation}

$J_n (\theta)$ is given the following differential equation. 
\begin{equation}~\label{eqn:cosdiff}
J_n(\theta)  =  (-1)^{n}(\text{sin}\theta)^{2n+1}\bigg(\frac{1}{sin\theta}\frac{\partial}{\partial \theta}\bigg)^{n} \bigg(\frac{\pi - \theta}{\text{sin}\theta}\bigg)
\end{equation}
Alternatively, $J_n(\theta)$ also has an integral representation
\begin{equation}~\label{eqn:cosint}
J_n(\theta) = n! (\text{sin}\theta)^{2n+1} \int_{0} ^{\pi/2}d\psi \frac{\text{cos}^{n}\psi}{(1-\text{cos}\theta \text{cos}\psi)^{n+1}}
\end{equation}
    
\begin{lemma}~\label{recrel}
$J_n(\theta)$ satisfies a recurrence relation of the form
\begin{equation*}
    J'_n(\theta) = (2n+1)\text{cot}(\theta)J_n(\theta) - \text{csc}(\theta)J_{n+1}(\theta)
\end{equation*}
\end{lemma}
\begin{proof}
Proof is a straightforward application of chain rule and differentiation under the integral sign. In the proof of the lemma we used the integral representation of $J_n (\theta)$~(Equation~\ref{eqn:cosint}). 
\end{proof}
%% Can come in handy for some other proofs

\subsection{Variants of the Arc Cos Kernel}
$J_0$ is not differentiable, since $\text{cos}^{-1}(z)$ is not differentiable at $z = \pm 1$. However the following easy lemma is true: 
\begin{lemma}
$\frac{J^{n}_{0}}{\pi^n}$ is differentiable at $\theta =0$ for $n \geq 2 $. 
\end{lemma}
\begin{proof}
Proof is a simple application of L'Hopital's rule.
\end{proof}
% An easy observation is : the variance of $\frac{J^{n}_{0}}{\pi^n}$ is a decreasing function of $n$. \\
However the above functions are still not differentiable at $\pi$. But the higher order $J_n$'s are. 

%%% Talk about the smoothed version and higher powers of J_0 and show that higher powers of J_0 are differentiable at 1. 

\section{Hybrid Kernels}
\subsection{Definition and Basic Properties}
The basic idea behind the hybrid kernels is to interpolate using the arc cosine kernels between the trigonometric kernel~\cite{rawat2019sampled} and the FAVOR+ kernel~\cite{performers}. The idea stems from the fact that in the two extreme data regimes, trigonometric and Favor+ kernels become deterministic. 

\begin{definition} (Hybrid Kernels)
Hybrid kernels $K(x,y)$ is defined as 
\begin{equation}
    K(x,y):= \frac{J_n(\theta)}{J_n(0)}K^{trig}(x,y) + (1-\frac{J_n(\theta)}{J_n(0)})K^{Favor+}(x,y)
\end{equation}
where $\theta$ is the angle between $x$ and $y$. 
\end{definition}
We can also replace $\frac{J_n(\theta)}{J_n(0)}$ by $\frac{J^n_{0}}{\pi^n}$ as well. Let $SM(x,y)$ denote the softmax kernel. Then,
\begin{lemma}
$\mathbb{E}(K(x,y)) = SM(x,y)$
\end{lemma}
\begin{proof}
Follows directly using the proof of lemma 1 and Theorem 1 in~\cite{orf}. 
\end{proof}
Thus these hybrid kernels are unbiased estimators of the softmax kernel.  \\

How to figure out the best weighing? 
The goal is to find the $\theta$ such that MSE($\hat{\text{K}}_{\text{trig}}) > $ MSE($\hat{\text{K}}_{\text{exp}})$ when $||x|| = ||y|| = 1$. 
\begin{proposition}
Let $||x|| = ||y|| =1.$ Then, MSE($\hat{\text{K}}_{\text{trig}}) > $ MSE($\hat{\text{K}}_{\text{exp}})$, iff $\text{cos}(\theta) < 1-\frac{1}{4}\text{log}(2e^{4}-1)$ 
\end{proposition}
\begin{proof}
 We use the MSE errors as proved in~\cite{performers}. Since $||x|| = ||y|| =1$, rewrite $x^{T}y = cos(\theta)$, $||x-y||^2 = 2 - 2\text{cos}(\theta)$ and similarly for $||x+y||^2$. The proof follows by plugging in the above relations in the MSE error formula.
\end{proof}

The proof shows that the MSE($\hat{\text{K}}_{\text{trig}}) > $ MSE($\hat{\text{K}}_{\text{exp}})$ when $\theta \in (11\pi/20, \pi)$. This gives us the justification that our weighing is optimal over all possible arc cos kernels~\cite{arccos}.
%%%Add more details. 

==> Hybrid Estimators (Camera-ready, Arxiv)/conclusion.tex <==
\vspace{-4mm}
\section{Conclusion}
\label{sec:conclusion}
\vspace{-4mm}
We presented a new class of random feature techniques, called \textit{hybrid random features} for softmax/Gaussian kernel estimation that more accurately approximate these kernels than previous algorithms. We also demonstrated their robustness in a wide range of applications from softmax sampling to Transformers/attention training, also for downstream Robotics tasks.
\vspace{-3mm}
\paragraph{Reproducibility Statement:} Section \ref{sec:experiments} and the Appendix include all experimental details (e.g. hyperparameter setup) needed to reproduce all the results presented in the paper. The part of the code that we could make publicly available can be found in the following anonymous github: \url{https://anonymous.4open.science/r/HRF_ICLR2022-B69C/}.
\vspace{-3mm}
\paragraph{Ethics Statement:} HRFs can be used in principle to train massive Transformer models with large number of parameters and proportional compute resources. Thus they should be used responsibly, in particular given $\mathrm{CO}_2$ emission challenges that scientific community tries to address now.

==> Hybrid Estimators (Camera-ready, Arxiv)/count_Sketches.tex <==
\section{Tensor sketching and its potential application to composite random feature}

\textbf{Brief summary of polynomial tensor sketching}

Given that $x, y \in \mathbb{R}^{d}$, we want to find out a random feature map $f(\cdot) : \mathbb{R}^{d} \rightarrow \mathbb{R}^{D}$ such that $\mathbb{E}[\langle f(x), f(y)\rangle] = {\langle x, y\rangle}^{p}$. When $p = 1$, we can apply count sketch to obtain random feature \cite{weinberger2009feature}. The random feature is constructed based on two 2-wise independent hash functions:
\begin{equation*}
    h(\cdot): [d] \rightarrow [D]\quad\quad s(\cdot): [d] \rightarrow \{-1, +1\}
\end{equation*}
The $k$-th dimension of random feature $f(x)$ for $x$ is defined as
\begin{equation*}
    f(x)_{k} = \sum_{i = 1}^{d}s(i)\delta\{h(i) = k\}x_{i} 
\end{equation*}

\textbf{Lemma}\quad $\mathbb{E}[\langle f(x), f(y) \rangle] = \langle x, y \rangle.$\\
Proof is provided in \cite{weinberger2009feature}. A general idea is:
\begin{align*}
    \mathbb{E}[\langle f(x), f(y) \rangle] &= \mathbb{E}_{h}[\mathbb{E}_{s}[\sum_{k = 1}^{D}\sum_{i, j = 1}^{d} s(i)s(j) \delta\{h(i) = k\}\delta\{h(j) = k\} x_{i}y_{j}]]\\
    &= \mathbb{E}_{h}[\mathbb{E}_{s}[\sum_{i, j = 1}^{d} s(i)s(j) x_{i}y_{j} \delta_{h(i)}^{T}\delta_{h(j)}]]\\
    &= \mathbb{E}_{h}[\sum_{i = 1}^{d} s(i)^{2} x_{i}y_{i} \delta_{h(i)}^{T}\delta_{h(i)}]\\
    &= \mathbb{E}_{h}[\sum_{i = 1}^{d}\sum_{k = 1}^{D}\delta\{h(i) = k\}x_{i}y_{i}]\\
    &= \sum_{i = 1}^{d}\mathbb{E}_{h}[\sum_{k = 1}^{D}\delta\{h(i) = k\}]x_{i}y_{i}\\
    &= \langle x, y\rangle
\end{align*}

Also, according to \citep{scholkopf2002learning} proposition 2.1, $\langle x^{(p)}, y^{(p)} \rangle = {\langle x, y\rangle}^{p}$, where $x^{(p)}$ denotes $p$-level tensor product and $x^{(p)} \in \mathbb{R}^{d^{p}}$. A simple case is that when $p=2$, $x^{(2)} = xx^{T}$. Therefore, if we can find a count sketch $C(x^{(p)})$ for $x^{(p)}$, then $\mathbb{E}[\langle C(x^{(p)}), C(y^{(p)}) \rangle] = {\langle x, y\rangle}^{p}$. \cite{pagh2013compressed} proposes a method to speed up the computation of the count sketch of two vectors' outer product $C(xy^{T})$. \cite{pham2013fast} generalizes the calculation to the $p$-th power when $y = x$. 

A simple case of $p = 2$ is demonstrated as an example. Given $x \in \mathbb{R}^{d}$, we leverage two different count sketches $\phi_{1}, \phi_{2}$ to obtain its random features, where $\phi_{1} = \{h_{1}, s_{1}\}$, $\phi_{2} = \{h_{2}, s_{2}\}$, and $h_{1}$, $s_{1}$, $h_{2}$, $s_{2}$ are two-wise independent. According to \cite{pagh2013compressed}, the count sketch of the outer product of two vectors can be approximated by the count sketch of the outer product of their corresponding count sketches. Consider independent and decomposable hash functions $H(\cdot): \mathbb{R}^{d\times d} \rightarrow \mathbb{R}^{D}$, and $S(\cdot): \mathbb{R}^{d\times d} \rightarrow \{-1, +1\}.$ Then we can decompose $H$ and $S$ by letting
\begin{equation*}
    H(i, j) = h_{1}(i) + h_{2}(j) \ mod\ D;\ \ S(i, j) = s_{1}(i) s_{2}(j)
\end{equation*}
Since the outer product of two different count sketches can be computed by polynomial multiplication, we can leverage FFT to reduce the computational time complexity. We represent $C_{1}(x) = [\sum_{i = 1}^{d}\delta\{h_{i} = 1\}s_{1}(i)x_{i}, ..., \sum_{i = 1}^{d}\delta\{h_{i} = D\}s_{1}(i)x_{i}]^{T} \in \mathbb{R}^{D}$ as a $D-1$ degree polynomial $P_{1}^{(x)}(\omega) = \sum_{i = 1}^{d}s_{1}(i)x_{i}\omega^{h_{1}(i)}$. Similar for $C_{2}(x)$, we can obtain a $D-1$ degree polynomial $P_{2}^{(x)}(\omega) = \sum_{i = 1}^{d}s_{2}(i)x_{i}\omega^{h_{2}(i)}$. Then the polynomial for the count sketch of $x^{(2)}$ with $\phi = {H, S}$ can be calculated as follows:
\begin{align*}
    P^{(x^{(2)})}(\omega) &= \sum_{i,j = 1}^{d} S(i, j)x_i x_j \omega^{H(i, j)}\\
    &= IFFT(FFT(P_{1}^{(x)}) \odot FFT(P_{2}^{(x)}))
\end{align*}
Then the coefficient of $P^{(x^{2})}(\omega)$ is exactly the count sketch of $x^{(2)}$. The time complexity is $\mathcal{O}(d + D\log D)$. Similar for $p$-level tensor product, we construct two 2-wise independent and decomposable hash functions $H$ and $S$ such that:
\begin{equation*}
    H(i_{1}, ..., i_{p}) = \sum_{j = 1}^{p}h_{i}(i_{j}) \ mod\ D;\ \ S(i_{1}, ..., i_{p}) = \Pi_{j = 1}^{p}s_{i}(i_{j})
\end{equation*}
Then the polynomial for the count sketch of $x^{(p)}$ with $\phi = {H, S}$ can be calculated as follows:
\begin{align*}
    P^{(x^{(p)})}(\omega) &= \sum_{i_{1},..., i_{p} = 1}^{d} S(i_{1}, ..., i_{p})\Pi_{k = 1}^{p}x_{i_{k}} \omega^{H(i_{1}, ..., i_{p})}\\
    &= IFFT(FFT(P_{i_{1}}^{(x)}) \odot ... \odot FFT(P_{i_{p}}^{(x)}))
\end{align*}
The computational time complexity is reduced from $\mathcal{O}(nd^{p})$ to $\mathcal{O}(np(d + D\log D))$.

\textbf{Relation to speed up composite random feature computation}

Instead of directly computing the composite random feature and perform dot product operation $\langle CRF(x), CRF(y) \rangle$, where $CRF(x)\in \mathbb{R}^{D_{1}\times D_{2}}$, and $D_{1}, D_{2}$ are dimensions of two different random features, we compute the count sketch of $CRF(x)$ and $CRF(y)$ as $C(CRF(x))$ and $C(CRF(y)) \in \mathbb{R}^{D}$. Since the count sketch of the outer product of the vectors can be approximated using the count sketch of the outer product of their corresponding count sketch, we compute count sketches $C_{1} (RF_1(x))$ and $C_{2} (RF_2(x))\in \mathbb{R}^{D}$, where $RF_1(x)RF_2(x)^{T} = CRF(x)$. Therefore,
\begin{align*}
    C(CRF(x)) &= C(RF_1(x)RF_2(x)^{T}) \\
    &= C( C_{1} (RF_1(x)) C_{2} (RF_2(x))^{T}) \\
    &= \text{coeff}(IFFT (FFT(P^{({RF_1(x)})}_1) \odot FFT(P^{({RF_2(x)})}_2))
\end{align*}
Then $\langle CRF(x), CRF(y) \rangle$ can be approximated by $\langle C(CRF(x), C(CRF(y) \rangle$. There is time complexity gain if we compute the dot product of composite random feature in this way. Originally, we require $\mathcal{O}(D_{1}D_{2}d)$ in order to compute the kernel approximation. Right now, we only need $\mathcal{O}(D_{1}d + D_{2}d + D\log D)$. However, an important problem is that we cannot guarantee the sketch for composite random feature is positive.

==> Hybrid Estimators (Camera-ready, Arxiv)/experiments-hrf.tex <==
%\newpage
\vspace{-4mm}
\section{Experiments}
\label{sec:experiments}
\vspace{-2.5mm}
In this section we conduct exhaustive evaluation of the mechanism of HRFs on several tasks.  

\vspace{-4.5mm}
\subsection{Pointwise Softmax Kernel Estimation}
\vspace{-3.5mm}
We start with ablation studies regarding empirical relative errors of different softmax kernel estimators across different inputs' lengths $r$ and angles $\theta_{\mathbf{x},\mathbf{y}}$. The results are presented in Fig. \ref{fig:pointwise}. Ablations over more lengths are presented in the Appendix (Sec. \ref{sec:pointwise_softmax_kernel_estimation}). The angular hybrid estimator most accurately approximates softmax kernel and has smaller max-relative-error than other estimators.

\small
\begin{figure}[h]
    \vspace{-4mm}
   \begin{center}
    \includegraphics[width=.72\textwidth]{img/new_plots/TrigFavorAngular_2rows.png}
   \end{center} 
    \vspace{-7.5mm}
    \caption{\small{Pointwise estimation of $\mathrm{SM}(\mathbf{x},\mathbf{y})$ for the same-length $64$-dim inputs ($r=1.0$ and $r=1.5$) and various angles $\theta_{\mathbf{x},\mathbf{y}}$. Red-dotted lines are for marking zero-level. We used $s=10000$ estimated softmax values in each subplot. The true value and the $5^{th}$ and $95^{th}$ quantile estimated values are shown by the left y-axis, and the empirical relative errors are shown by the right y-axis. Trigonometric estimator and FAVOR+ applied 128 random features. To make fair comparison, for the hybrid variant the configuration leading to the similar number of FLOPS operations per random feature map creation was applied. Similar gains as for the angular are obtained by the Gaussian hybrid variant. }}
\label{fig:pointwise}
\vspace{-4mm}
\end{figure}
\normalsize
\vspace{-2mm}



\paragraph{Comparison with QMC-methods:} Even though, as we explained in Section \ref{sec:intro}, our algorithm does not compete with various methods for variance reduction based on different sampling techniques (since those methods, as orthogonal to ours, can be easily incorporated into our framework), we decided to compare HRFs also with them. We tested angular hybrid HRF variant as well as well-established QMC baselines: orthogonal random features (ORF)\citep{orf} (regular variant ORF-reg as well as the one applying Hadamard matrices ORF-Had) and QMCs based on random Halton sequences (Halton-R)\citep{gQMC}. For HRFs, we tested two sub-variants: with orthogonal (HRF-ort) and regular iid random features (HRF-iid). We computed empirical MSEs by averaging over $100$ randomly sampled pairs of vectors from two UCI datasets: $\mathrm{wine}$ and $\mathrm{Boston}$. HRFs outperform all other methods, as we see in Table \ref{tab:uci}.   
\iffalse
\begin{table}[h!]
\vspace{-2mm}
    \centering
    \caption{\small{Comparison of different estimators of the softmax kernel on the datapoints from two UCI datasets: wine and Boston in terms of the MSE (measured in 10^{-3} units). The non-HRF estimators apply 512 random features and the HRF-ones are set up to match the non-HRFs in terms of the number of FLOPS (for a fair comparison). We also reported standard deviations.}}
    \vspace{-3mm}
    \begin{tabular}{|c|c|c|c|c|c|} \hline
    wine & HRF-ort & HRF-iid & ORF-reg & ORF-Had &  Halton-R  \\ \hline
     MSE [in $10^{-3}$] & $\mathbf{0.70 \pm 0.08}$ &  $0.85 \pm 0.05$ & $1.00 \pm 0.04$ & $1.10 \pm 0.06$ & $4.02 \pm 0.1$  \\ \hline % 33.0
    \end{tabular}
    \label{tab:uci}
\end{table}
\vspace{-2.0mm}
\begin{table}[h!]
    \centering
    \vspace{-3mm}
    \begin{tabular}{|c|c|c|c|c|c|} \hline
    Boston & HRF-ort & HRF-iid & ORF-reg & ORF-Had & Halton-R  \\ \hline
     MSE [in $10^{-3}$] &  $\mathbf{0.72 \pm 0.06}$ & $0.79 \pm 0.08$ & $1.05 \pm 0.03$ & $1.14 \pm 0.02$ & $2.53 \pm 0.08$ \\ \hline % 33.0
    \end{tabular}
\vspace{-1mm}
\end{table}
\fi


\small
\begin{table}[h!]
\vspace{-3mm}
    \centering
    \caption{\small{Comparison of different estimators of the softmax kernel on the datapoints from two UCI datasets: wine and Boston in terms of the MSE (measured in $10^{-3}$ units). The non-HRF estimators apply 512 random features and the HRF-ones are set up to match the non-HRFs in terms of the number of FLOPS (for a fair comparison). We also reported standard deviations.}}
    \vspace{-3mm}
    \scalebox{0.9}{
    \begin{tabular}{|c|c|c|c|c|c|} \hline
    Datasets & HRF-ort & HRF-iid & ORF-reg & ORF-Had &  Halton-R  \\ \hline
    Wine  & $\mathbf{0.70 \pm 0.08}$  &  $0.85 \pm 0.05$ & $1.00 \pm 0.04$ & $1.10 \pm 0.06$ & $4.02 \pm 0.1$  \\ \hline 
     Boston &  $\mathbf{0.72 \pm 0.06}$ & $0.79 \pm 0.08$ & $1.05 \pm 0.03$ & $1.14 \pm 0.02$ & $2.53 \pm 0.08$ \\ \hline % 33.0
    \end{tabular}}
\vspace{-5mm}
\label{tab:uci}
\end{table}
\normalsize
%MSE [in $10^{-3}$]



\vspace{0mm}
\subsection{Language Modeling}\label{Sec:LM}
\vspace{-3mm}
In this section, we apply HRFs to the language modeling task, training a $2$-layer LSTM with hidden size $h=200$ and applying RFs for softmax sampling in training as described in \citep{softmax_sampling_2}. Experimental results are obtained over $10$ runs. Experimental details and additional validation results are in the Appendix (Sec. \ref{sec:lm}, Table \ref{tab:ptb_std}).
% \small
% \begin{figure}
%   \begin{center}
%     \includegraphics[width=.7\textwidth]{img/new_plots/TrigFavorAngular_2rows.png}
%   \end{center} 
%     \vspace{-6.5mm}
%     \caption{\small{Pointwise estimation of $\mathrm{SM}(\mathbf{x},\mathbf{y})$ for the same-length $64$-dim inputs ($r=1.0$ and $r=1.5$) and various angles $\theta_{\mathbf{x},\mathbf{y}}$. We used $s=10000$ estimated softmax values in each subplot. The true softmax value and the $5^{th}$ and $95^{th}$ quantile estimated values are shown by the left y-axis, and the empirical relative errors are shown by the right y-axis. Trigonometric estimator and FAVOR+ applied 128 random features. To make fair comparison, for the hybrid variant the configuration leading to the similar number of FLOPS operations per random feature map creation was applied.}}
% \label{fig:pointwise}
% \vspace{-4mm}
% \end{figure}
% \normalsize
% \vspace{-5mm}
% \small
% \begin{figure} 
% \centering
% \includegraphics[width=.99\textwidth]{img/Cluster_result.png} 
% \vspace{-3.5mm}
% \caption{\small{Comparing different estimators for data with clustering structure. The empirical MSE is obtained by averaging over $s=20$ trials. For the HRFs, we apply deterministic $\lambda$-coefficients. We took: $s \in \{,\}$, $\sigma \in \{,\}$.}}
% \label{fig:clustering}
% \vspace{-4.5mm}
% \end{figure}
% \normalsize
% \vspace{-3mm}

\vspace{-4mm}
\begin{figure}[h]
    \centering
    \includegraphics[width=.93\textwidth]{img/PTB_metrics.png}
    \vspace{-3mm}
    \caption{\small{Statistical metrics measuring softmax matrix approximation quality on PennTree Bank. For standard estimators, the number of random features are $64, 128, 256, 512$. To make fair comparison, for the hybrid variants, the configurations leading to the similar number of FLOPS operations per random feature map creation were applied. Negative fractions were not reported for FAVOR+ since by definition they are equal to zero.}}
    \label{fig:PTB_metrics}
\vspace{-6mm}
\end{figure}
\vspace{2mm}


\vspace{0.5mm}
\textbf{Statistical Metrics.} We compute $1d$-Wasserstein distance and the Kolmogorov-Smirnov (KS) metric \citep{cuturi} between a true softmax distribution induced by a query on all the classes and the approximate one given by different RF-mechanisms. We also compute the fraction of all probability estimates with undesired negative values. The results on the PennTree Bank~\cite{marcus-etal-1993-building} are presented in Fig. \ref{fig:PTB_metrics}. In the Appendix (Sec. \ref{sec:lm}) we present additional results for the $\mathrm{WikiText2}$ dataset. We see that HRFs lead to most accurate softmax distribution estimation.





\vspace{-1mm}
%\small
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=.99\textwidth]{img/PTB_metrics.png}
%     \vspace{-3mm}
%     \caption{\small{Statistical metrics measuring softmax matrix approximation quality on PennTree Bank. For standard estimators, the number of random features are $64, 128, 256, 512$. To make fair comparison, for the hybrid variants, the configurations leading to the similar number of FLOPS operations per random feature map creation were applied. Negative fractions were not reported for FAVOR+ since by definition they are equal to zero.}}
%     \label{fig:PTB_metrics}
% \end{figure}
%\normalsize
%\vspace{-3mm}
% \vspace{-3.5mm}
% \small
% \begin{figure}[h]
%  \centering
%  \includegraphics[width=.85\textwidth]{img/PTB_training.png}
%  \vspace{-3mm}
%  \caption{\small{Language Modeling with softmax sampling: training results on PennTree Bank dataset (40-60 epoch window zoomed in on the right subfigure). FAVOR+/trigonometric mechanisms used $1024$ random features. To make fair comparison, for HRFs, the configurations leading to the similar number of FLOPS operations per random feature map creation were applied. HRFs turn out to be the most accurate random feature method. }}
%  \label{fig:PTB_training}
%  %\vspace{-1mm}
% \end{figure}
% \normalsize


\iffalse
\textbf{Validation Results.} We sampled $m=40$ negative (other than true) classes for softmax loss approximation in training, and calculated the validation loss using full softmax (see: Fig.~\ref{fig:PTB_training}). The uniform method sampled negative classes uniformly at random, the sampled softmax method sampled classes with the full softmax distribution as the sampling distribution. HRFs and positive random features outperform SOTA RF-mechanism based on trigonometric random features \citep{softmax_sampling_2}. The \textit{perplexity} score in Fig.~\ref{fig:PTB_training} is defined as $2^{\textrm{cross } \textrm{entropy } \textrm{loss}}$.
\fi

\vspace{-1mm}
\subsection{Training Speech Models with HRF-Conformers-Performers}
\vspace{-3.2mm}
We also tested HRFs on speech models with \textrm{LibriSpeech} ASR corpus \citep{panayotov}. We put implicit Performer's attention into $17$-layer Conformer-Transducer encoder \citep{gulati} and compared softmax kernel estimators in terms of word error rate (WER) metric, commonly used to evaluate speech models. 
We tested HRFs using angular hybrid variant as well as those clustering-based. For the latter ones, the clusters were created according to the $\mathrm{K}$-means algorithm after first $1000$ steps of training (and were frozen afterwards) and corresponding matrices $\mathbf{A}$ were constructed to minimize the loss given in Equation \ref{cluster la equation}.
The results are presented in Table \ref{tab:speech}. HRFs produce smallest WER models and the clustering-based variants fully exercising the most general formulation on HRFs (with general complex estimators) turn out to be the best. Additional details regarding speech experiments as well as additional experiments with clustering-based HRFs are presented in the Appendix (Sec. \ref{sec:app_speech} and Sec. \ref{synthetic:clustering} respectively).

%\vspace{-1mm}
\small
\begin{table}[h!]
    \centering
    \vspace{-2mm}
    \caption{\small{Comparison of WERs of Conformer-Transducer applying different RF-mechanisms for the implicit attention. For methods other than clustering-based HRFs (HRF-C), numbers next to method names define the values of $m$ or $(m,n)$. Method HRF-A stands for the angular hybrid variant. Numbers next to HRF-C correspond to the number of clusters constructed in the query and key space respectively. HRF-C uses $64$ random features. We also report standard deviations averaged over $10$ different training runs.}}
    \vspace{-2mm}
    \scalebox{0.9}{
    \begin{tabular}{|c|c|c|c|c|c|} \hline
    & HRF-C(3,3) & HRF-C(2, 3) & HRF-C(3,2) & HRF-C(2,2) &  HRF-A(16,8)  \\ \hline
     WER & $\mathbf{1.72 \pm 0.02\% }$ &  $1.75 \pm 0.03\%$ & $1.83 \pm 0.03\%$ & $1.85 \pm 0.04\%$ & $2.03 \pm 0.08\%$  \\ \hline % 33.0
    & HRF-A(8, 8) & FAVOR+ 432 & FAVOR+ 256 & Trig 432 & Trig 256  \\ \hline
     WER &  $2.05 \pm 0.05\%$ & $2.65 \pm 0.06\%$ & $2.77 \pm 0.04\%$ & $3.12 \pm 0.05\%$ & $3.3 \pm 0.06\%$ \\ \hline % 33.0
    \end{tabular}}
\label{tab:speech}
\vspace{-4mm}
\end{table}
\normalsize


\iffalse

\vspace{1mm}
\begin{table}[h!]
    \centering
    \caption{\small{Comparison of WERs of Conformer-Transducer applying different RF-mechanisms for the implicit attention. For methods other than clustering-based HRFs (HRF-C), numbers next to method names define the values of $m$ or $(m,n)$. Method HRF-A stands for the angular hybrid variant. Numbers next to HRF-C correspond to the number of clusters constructed in the query and key space respectively. HRF-C uses $64$ random features. We also report standard deviations averaged over $10$ different training runs.}}
    \begin{tabular}{|c|c|c|c|c|c|} \hline
    & HRF-C(3,3) & HRF-C(2, 3) & HRF-C(3,2) & HRF-C(2,2) &  HRF-A(16,8)  \\ \hline
     WER & $\mathbf{1.72 \pm 0.02\% }$ &  $1.75 \pm 0.03\%$ & $1.83 \pm 0.03\%$ & $1.85 \pm 0.04\%$ & $2.03 \pm 0.08\%$  \\ \hline % 33.0
    \end{tabular}
    \label{tab:speech}
\end{table}
\vspace{-4.0mm}
\begin{table}[h!]
    \centering
    \vspace{-3mm}
    \begin{tabular}{|c|c|c|c|c|c|} \hline
    & HRF-A(8, 8) & FAVOR+ 432 & FAVOR+ 256 & Trig 432 & Trig 256  \\ \hline
     WER &  $2.05 \pm 0.05\%$ & $2.65 \pm 0.06\%$ & $2.77 \pm 0.04\%$ & $3.12 \pm 0.05\%$ & $3.3 \pm 0.06\%$ \\ \hline % 33.0
    \end{tabular}
\vspace{-4mm}
\end{table}

\fi

\vspace{1mm}
\subsection{Downstream Robotics Experiments}
\vspace{-3mm}
In Robotics, we leverage the accuracy of HRFs to obtain inference improvements, critical for on-robot deployment. To abstract from a particular hardware characteristic, we measure it in the number 
of FLOPS. We conduct two experiments targeting: (a) quadruped locomotion and (b) robotic-arm manipulation. In the former, HRFs are applied as a replacement of the default mechanism using positive random features in the class of implicit-attention architectures for vision processing called \textit{Implicit Attention Policies} (or IAPs) \citep{IAP2021}. In the latter, HRFs become a part of the regular Vision-Performer stack used to process high-resolution (500 x 500 x 3) input. The results are presented in Fig. \ref{fig:mpc_perf}, where HRFs need \textbf{3x} fewer FLOPS to obtain same quality policies as baselines. All details regarding both experimental setups are given in the Appendix (Sec. \ref{sec:app_robotics}). Videos of the HRF-trained robotic policies are included in the supplementary material. 

\small
\begin{figure}[h]
\vspace{-3.5mm}
    \centering
    \includegraphics[width=.85\linewidth, valign=t, trim={0 0 0 0.25cm}, clip]{img/robotics_plots_3.pdf}
    \vspace{-3.5mm}
    \caption{\small{\textbf{Left}: Step-stone locomotion task. Comparison of the training curves for: the IAP using angular hybrid estimator of $m=n=8$ and IAP applying regular FAVOR+ mechanism from \citep{performers} with $m=256$. Both final policies are of similar quality, yet HRF-method requires \textbf{3x+} fewer FLOPS to run its trained policy. The visualization of the HRF policy in action and its attention (with filtered out pixels marked in red) is in the bottom right corner. \textbf{Right:} Similar setting (and conclusions) but for the robotic-arm manipulation task. The additional five regular RF-configurations did not train by producing $\mathrm{Nan}$ loss due to large variance of the underlying softmax kernel estimators. }}
    \label{fig:mpc_perf}
\vspace{-3mm}    
\end{figure}
\normalsize




==> Hybrid Estimators (Camera-ready, Arxiv)/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

% \url{https://arxiv.org/pdf/1609.04309.pdf}
% \url{https://papers.nips.cc/paper/7130-svd-softmax-fast-softmax-ap% proximation-on-large-vocabulary-neural-networks.pdf}
% \url{https://openreview.net/pdf?id=rkmDI85ge}
% All of the above is on softmax of word embeddings

%%%Wikitext2 Benchmark results https://arxiv.org/abs/1609.07843
To understand how close the random trigonometric features and the random positive orthogonal features approximate the softmax sampling, we evaluated it empirically on three datasets, \textbf{(a)} Penn Tree Bank, \textbf{(b)} WikiText2 and \textbf{(c)} WikiText103. 
%% Write a bit about the datasets. 
For the Penn Tree Bank dataset, we trained a $2$-layer LSTM with hidden size of $200$ and we tied the weights of the word embedding layer and the decoder layer. Thus we can treat the masked language modeling problem as minimizing the cross entropy loss between the dot product of the model output and the class embedding obtained from the embedding layer with the target word. After training, we replaced the softmax layer with the variants, \textbf{(a)} Random Trigonometric Features, \textbf{(a)} Positive Orthogonal Random Features and \textbf{(c)} Hybrid Random Features. To understand the relationship between the softmax distribution and the distribution coming from random features, we used Wasserstein metric to compute the difference between the distributions. Unlike the trigonometric or the hybrid variant, we can normalize the positive features across the classes and can treat them as probability distributions. We can easily compute the Wasserstein distance between the histograms given by the softmax sampling and the normalized positive features. However normalizing the trigonometric features yields negative probabilities.  In fact, we found examples where all the entries for a given row in our matrix is negative. (Other hack is normalize, apply ReLu and then normalize. Not sure if it is worth doing or a fair/proper comparison). So for a proper comparison, we normalized all the matrices (should we not do it?) and treated the vectors as samples from an empirical distribution. That allowed to compute the entropic regularized $2$-Wasserstein distance ~\cite{Cuturi} and the Sliced Wasserstein distance. For all the experiments, number of random features were chosen to be $64$. 

\begin{table}[h]
\begin{center}
\caption{Empirical Results comparing distributions from random features to the true softmax distribution}
\label{tab:wass}
\begin{tabular}{l c c c c} 
 \toprule
 Method &  \begin{tabular}[c]{@{}c@{}} Trigonometric Random \\ Features \end{tabular} & \begin{tabular}[c]{@{}c@{}} Positive Orthogonal\\  Random Features \end{tabular} & \begin{tabular}[c]{@{}c@{}} Hybrid Random \\ Features \end{tabular}  \\
 \midrule
 \begin{tabular}[c]{@{}c@{}} $1D$ Wasserstein Distance\\  between Histograms \end{tabular} &  N/A & $.0015 $ & N/A \\
 \begin{tabular}[c]{@{}c@{}} Entropic Regularized \\ Wasserstein Distance \end{tabular} & .0995  & .0902 & - \\
Sliced Wasserstein Distance & .0027  & .003 & - \\
 \bottomrule
\end{tabular}
\end{center}
\end{table}
%
% With the FavorPlus mechanism, the test losses for Penn Tree Bank are 9.3, 9.1, 8.7, 8.3 and the RMSE between Favorplus and the true softmax is .003, .003, .001, .0005 for 64,128, 256 and 512 features respectively. For RFF, the test losses are 9.4, 9.2, 8.8 and 8.3 respectively and the RMSE is .004, .003, .002 and .0006 for 64,128,256 and 512 features respectively and with the same features matrix. Surprisingly none of the dot products of trigonometric features is negative.

% Results for Wikitext2:
% ALL WITH UNNORMALIZED FEATURES:
% FAVORPLUS: 
% 64 random features : 11.98\\
% 128 random features: 11.08 \\
% 256 random features: 10.87 \\
% 512 random features: 10.2 \\
%% TODO Do normalized embeddings and the choose various \tau
RFF:
With 64 no negative features
64 random features: 12.01\\

\vspace{-2mm}
\small
\begin{table}[h]
    \caption{\small{NLP softmax sampling experiments.}}
    \begin{center}
    \vspace{-1mm}
    \scalebox{0.85}{
     \begin{tabular}{ c  c  c  c  c  c  c} 
    \toprule
      $\textbf{\textrm{Method}}$ & \multicolumn{2}{c}{$\textbf{\textrm{PTB}}$} & \multicolumn{2}{c}{$\textbf{\textrm{WikiText2}}$} & \multicolumn{2}{c}{$\textbf{\textrm{WikiText103}}$}\\
    
    & Test loss & RMSE & Test loss & RMSE & Test loss & RMSE\\
    \toprule
    $\textbf{\textrm{RFF (m = 64)}}$ & $9.4$ & $ .004$ & $12.01$ & & & \\ 
    $\textbf{\textrm{RFF (m = 128)}}$ & $9.2$ & $ .003$ & & & & \\ 
    $\textbf{\textrm{RFF (m = 256)}}$ & $8.8$ & $ .002$ & & & & \\ 
    $\textbf{\textrm{RFF (m = 512)}}$ & $8.3$ & $ .0006$ & & & & \\ 
    $\textbf{\textrm{Favor+ (m = 64)}}$ & $9.3$ & $ .003$ & $11.98$ & & & \\ 
    $\textbf{\textrm{Favor+ (m = 128)}}$ & $9.1$ & $ .003$ & $11.08$ & & & \\ 
    $\textbf{\textrm{Favor+ (m = 256)}}$ & $8.7$ & $ .001$ & $10.87$& & & \\ 
    $\textbf{\textrm{Favor+ (m = 512)}}$ & $8.3$ & $ .0005$ & $10.20$ & & & \\
    \bottomrule
     \end{tabular}}
\label{table:softmax_sampling}    
\end{center}
\end{table}
\normalsize

To understand why these hybrid estimators do not provide accuracy in sampling, we looked at the angles between keys and queries. The following figure~\ref{fig:hist-ptb} shows most of the angles are clustered around $\pi/2$. \\
To understand the nature of misclassifications, we calculated the average Euclidean distance between the true target embedding and the predicted target embedding. The following table shows the results for this difference between the Euclidean distances. 
\begin{figure}[h]

	\includegraphics[width=.49\columnwidth]{img/plots_arijit/Angle-Hist-PTB.png}
	\includegraphics[width=.49\columnwidth]{img/plots_arijit/Angle-Hist-wikitext2.png}
	\caption{Histogram of angles between keys and test query embeddings from our LSTM trained on Penn Tree Bank (Left) and WikiText2 (Right).}
	\label{fig:hist-ptb}
\end{figure}

\begin{figure}[h]

	\includegraphics[width=.33\columnwidth]{img/PTB_softmax_value_dist.png}
    \includegraphics[width=.33\columnwidth]{img/PTB_query_len_dist.png}
	\includegraphics[width=.33\columnwidth]{img/PTB_key_len_dist.png}
	\caption{Cumulative distribution plot about softmax values, and histogram plots for key length, query length in PTB dataset.}
	\label{ vhist2-ptb}
\end{figure}

\begin{table}[h]
    \centering
   \resizebox{\columnwidth}{!} {\begin{tabular}{cccc} 
   Number of random features  &  \begin{tabular}[c]{@{}c@{}}  Distance between predicted logits \\ 
   via regular softmax and actual targets \end{tabular} & \begin{tabular}[c]{@{}c@{}}  Distance between predicted logits \\ 
   via RFF and actual targets \end{tabular}
         & \begin{tabular}[c]{@{}c@{}}  Distance between predicted logits \\ via FAVOR and actual targets \end{tabular} \\
         \midrule
      512   &  .036  & .088 & .025 \\
      \bottomrule
    \end{tabular}
    }
    \caption{Average Euclidean Distance between predicted classes and true classes in the Penn Tree Bank}
    \label{tab:my_label}
\end{table}

%% Still need help in calculating the metrics for the full dataset. This crashes when I try to run it. I can only do 1D Wasserstein distance. 
For the Sliced Wasserstein distance, we took $60$ random projections where the dimensions are spaced evenly on a log scale in $[1,4]$. \\
The code for the numerical experiments can be found at \url{https://github.com/arijitthegame/hybrid-sampling}.
Question: Should we look at the Alias sampling~\cite{walker1977} for positive features? 


We compare the average 1D Wasserstein distance and Kolmogorov–Smirnov distance between the true softmax matrix and the approximated softmax matrix with different random feature techniques. The number of random features for FAVOR+ and RFF are $64, 128, 256, 512$. In order to maintain the same budget, we use $48, 112, 240, 496$ random features for base estimators, and $16$ for coefficient estimators. The results shown in Figure \ref{fig:PTB_1d_wass} and \ref{fig:PTB_ks} are obtained by averaging over $10$ repetitions.

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/PTB_wass_dist.png}
    \end{center} 
    \label{fig:PTB_1d_wass}
    \caption{1D Wasserstein distances with different random feature techniques for estimating softmax value matrix in PTB dataset.}
\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/PTB_KS_dist.png}
    \end{center} 
    \label{fig:PTB_ks}
    \caption{Kolmogorov–Smirnov distances with different random feature techniques for estimating softmax value matrix in PTB dataset.}
\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/PTB_KL_dist.png}
    \end{center} 
    \label{fig:PTB_ks}
    \caption{KL divergence with different random feature techniques for estimating softmax value matrix  in PTB dataset.}
\end{figure}



Results for hybrid estimators based on clustering, for two   
normalized clusters with Gaussian noise in $\R^{50}$. The mean square errors is computed by running 5 times of simulations. Here $\tau$ is the $\tau$ used in the lambda estimator expressed by
(\ref{hybrid for matrix x}) and (\ref{hybrid for matrix y}).


 




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/cluster_synthetic_dim_50_nrff_50.png}
    \end{center}
    \end{minipage}	\caption{Results for synthetic Gaussian clusters when the number of random features is 50}
\end{figure}


\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/cluster_synthetic_dim_50_nrff_150.png}
    \end{center}  \caption{Results for synthetic Gaussian clusters when the number of random features is 150}
\end{figure}




\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/new_plots/Cluster_FAVOR_PLUS_results}
    \end{center}  \caption{Results for synthetic normalized two Gaussian clusters with FAVOR+ as the base estimator}
\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/new_plots/Cluster_Trig_results.eps}
    \end{center}  \caption{Results for synthetic normalized two Gaussian clusters with Trigonometry as the base estimator}
\end{figure}


\clearpage

==> Hybrid Estimators (Camera-ready, Arxiv)/intro-HRF.tex <==
\vspace{-4mm}
\section{Introduction \& Related Work}
\label{sec:intro}
\vspace{-2mm}
Consider the \textit{softmax} and \textit{Gaussian kernel} functions $\mathrm{K}:\mathbb{R}^{d \times d} \rightarrow \mathbb{R}$ defined as follows:
\vspace{-2mm}\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y})\overset{\mathrm{def}}{=}\exp(\mathbf{x}^{\top}\mathbf{y}), \qquad \mathrm{K}_{\mathrm{gauss}}(\mathbf{x},\mathbf{y}) \overset{\mathrm{def}}{=}\exp(-\frac{\|\mathbf{x}-\mathbf{y}\|_{2}^{2}}{2}).
\vspace{-1mm}\end{equation}
These two are %some of the most 
prominent examples of functions used in the so-called \textit{kernel methods} \citep{km_1, km_2} and beyond, i.e. in softmax-sampling \citep{softmax_sampling}.
Random features (RFs, \citealp{fourierapprox, rfms_survey, rfa-paper}) yield a powerful mechanism for linearizing and consequently scaling up kernel methods with dot-product kernel decompositions disentangling $\mathbf{x}$ from $\mathbf{y}$ in the formulae for kernel value $\mathrm{K}(\mathbf{x},\mathbf{y}) \approx \phi(\mathbf{x})^{\top}\phi(\mathbf{y})$ via data-agnostic probabilistic (random feature) maps $\phi:\mathbb{R}^{d} \rightarrow \mathbb{R}^{m}$.
The tight relationship between softmax and Gaussian kernels given by the transformation $ \mathrm{K}_{\mathrm{gauss}}(\mathbf{x},\mathbf{y})= \exp(-\frac{\|\mathbf{x}\|_{2}^{2}}{2})\mathrm{SM}(\mathbf{x},\mathbf{y})\exp(-\frac{\|\mathbf{y}\|_{2}^{2}}{2})$ provides a mapping of any random feature vector $\phi_{\mathrm{SM}}(\mathbf{u})$ for the softmax kernel to the corresponding one $\phi_{\mathrm{gauss}}(\mathbf{u}) = \exp(-\frac{\|\mathbf{u}\|_{2}^{2}}{2}) \phi_{\mathrm{SM}}(\mathbf{u})$ for the Gaussian kernel, thus %from now on 
we will focus on the former kernel.
The classic random feature map mechanism $\phi^{\mathrm{trig}}_{m}$ for the softmax kernel, obtained from Bochner's Theorem applied to the Gaussian kernel \citep{fourierapprox}, is of the form:
\vspace{-1mm}\begin{equation}
\label{tri}
\phi^{\mathrm{trig}}_{m}(\mathbf{u}) = \frac{1}{\sqrt{m}} \exp(\frac{\|\mathbf{u}\|^{2}}{2})\left(\sin(\omega_{1}^{\top}\mathbf{u}),...,\sin(\omega_{m}^{\top}\mathbf{u}),\cos(\omega_{1}^{\top}\mathbf{u}),...,\cos(\omega_{m}^{\top}\mathbf{u})\right)^{\top},
\vspace{-3mm}\end{equation}
where $m$ stands for the number of random features and $\omega_{1},...,\omega_{m} \overset{\mathrm{iid}}{\sim} \mathcal{N}(0,\mathbf{I}_{d})$. 

The above (common in most downstream use-cases) method for linearizing softmax/Gaussian kernels was recently shown to fail in some of the new impactful applications of scalable kernel methods such as implicit-attention Transformer architectures called Performers \citep{performers}. %Despite the fact that 
We denote by MSE the mean squared error of the estimator (i.e. its variance since all estimators considered in this paper are unbiased).
The above mechanism struggles to accurately approximate close-to-zero kernel values, as characterized by the particularly large MSE in that region. % of space.
This is a crucial problem since most of the entries of the attention matrices in Transformers' models are very small and the approximators need to be particularly accurate there. Otherwise the renormalizers computed to make attention matrices row-stochastic (standard attention normalization procedure in Transformers) would be estimated imprecisely, potentially even by negative values.

The solution to this problem was presented in FAVOR+ mechanism \citep{performers}, where a new positive random feature map for unbiased softmax kernel estimation was applied:
\vspace{-3mm}\begin{equation}
\label{plusplus}
\phi^{\mathrm{++}}_{m}(\mathbf{u}) = \frac{1}{\sqrt{2m}} \exp(-\frac{\|\mathbf{u}\|^{2}}{2})\left(\exp(\omega_{1}^{\top}\mathbf{u}),...,\exp(\omega_{m}^{\top}\mathbf{u}),\exp(-\omega_{1}^{\top}\mathbf{u}),...,\exp(-\omega_{m}^{\top}\mathbf{u})\right)^{\top}.
\vspace{-5mm}\end{equation}

Even though, very accurate in estimating small softmax kernel values (which turns out to be crucial in making RFs work for Transformers training), this mechanism is characterized by larger MSE for large kernel values. In several applications of softmax kernels (in particular Transformers, where attention matrices typically admit sparse combinatorial structure with relatively few but critical large entries and several close-to-zero ones or softmax sampling) the algorithm needs to process simultaneously very small and large kernel values.
The following natural questions arise:

\textit{Is it possible to get the best from both the mechanisms to obtain RFs-based estimators particularly accurate for both very small and large softmax kernel values ?
Furthermore, can those estimators be designed to have low variance in more generally pre-defined regions ?
}

We give affirmative answers to both of the above questions by constructing a new class of random feature maps techniques called \textit{hybrid random features} or HRFs. Theoretical methods used by us to develop HRFs: (a) provide a unifying perspective, where trigonometric random features from Bochner's Theorem and novel mechanisms proposed in \citep{performers} are just special corollaries of the more general result from complex analysis, (b) integrate in the original way several other powerful probabilistic techniques such as Goemans-Willimson method \citep{goemans} and random features for the compositional kernels \citep{daniely}. 

We provide detailed theoretical analysis of HRFs, showing in particular that they provide strictly more accurate worst-case softmax kernel estimation than previous algorithms and lead to computational gains. We also conduct their thorough empirical evaluation on tasks ranging from pointwise kernel estimation to downstream problems involving training Transformer-models or even end-to-end robotic controller-stacks including attention-based architectures.  
\vspace{-4mm}
\paragraph{Related Work:} The literature on different random feature map mechanisms for Gaussian (and thus also softmax) kernel estimation is voluminous. Most focus has been put on reducing the variance of trigonometric random features from \citep{fourierapprox} via various Quasi Monte Carlo (QMC) methods, where directions and/or lengths of Gaussian vectors used to produce features are correlated, often through geometric conditions such as orthogonality \citep{unrea, rowland, orf, uomc, recycling}. 
Our HRFs do not compete with those techniques (and can be in fact easily combined with them) since rather than focusing on improving sampling mechanism for a given approximation algorithm, they provide a completely new algorithm. 
The new application of random features for softmax kernel in Transformers proposed in \citep{masked,performers} 
led to fruitful research on the extensions and limitations of these methods. \citet{schlag} replaced random features by sparse deterministic constructions (no longer approximating softmax kernel).  \citet{luo2021stable} observed that combining $L_{2}$-normalization of queries and keys for variance reduction of softmax kernel estimation with FFT-based implementations of relative position encoding and FAVOR+ mechanism from Performers helps in training. Trigonometric random features were applied for softmax sampling in \citep{softmax_sampling_2}.
Several other techniques such as Nystr{\"{o}}m method \citep{nystrom, williamsseeger, rudi1} were proposed to construct data-dependent feature representations. Even though, as we show in Sec. \ref{sec:instantiations}, certain instantiations of the HRF mechanism clearly benefit from some data analysis, our central goal remains an unbiased estimation of the softmax/Gaussian kernels which is no longer the case for those other techniques.
\vspace{-3mm}

==> Hybrid Estimators (Camera-ready, Arxiv)/intro.tex <==
\section{Introduction}



==> Hybrid Estimators (Camera-ready, Arxiv)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Hybrid Estimators (Camera-ready, Arxiv)/proofs_MSE.tex <==
\section*{APPENDIX: Proofs for MSE of Multiple Estimators}



% $\lambda_n(x,y)=\mathbb{E}_{\omega \sim N(0,1_d)}[(\frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{x})}{2}(\mathbf{\omega}^{\top}\mathbf{x})^n)(\frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{y})}{2}(\mathbf{\omega}^{\top}\mathbf{y})^n)]$


% $\lambda_0(x,y)=\mathbb{E}_{\omega \sim N(0,1_d)}[\frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{x})}{2}  \frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{y})}{2}]$


% let $ u_i \sim N(0,1_d),  v_i \sim N(0,1_d), \omega_i \sim N(0,1_d)$ chosen independently

% $\hat{\lambda}_0(x,y)=\frac{1}{r}\sum_{i=1}^{r}\xi_{\lambda}(\mathbf{x},\omega_i)\xi_{\lambda}(\mathbf{y},\omega_i) $

% where $\xi_{\lambda}(\mathbf{x},\omega^1_i)=\frac{1+\mathrm{sign}(\mathbf{\omega_i}^{\top}\mathbf{x})}{2}$

% $\mathbb{E}[\hat{\lambda}_0(x,y)]=\mathbb{E}[\frac{1+\mathrm{sign}(\mathbf{\omega_i}^{\top}\mathbf{x})}{2}\frac{1+\mathrm{sign}(\mathbf{\omega_i}^{\top}\mathbf{y})}{2}]=\frac{1}{4}+$


% $\mathbb{E}[\hat{\lambda}_0(x,y)^2]=$




% $\phi_m^{1,++}(\mathbf{x})=\frac{1}{\sqrt{2}}\exp(-\frac{\|\mathbf{x} \|^{2}}{2})\exp({\mathbf{u}}^{\top}\mathbf{x}),   \phi_m^{2,++}(\mathbf{x})=\frac{1}{\sqrt{2}}\exp(-\frac{\|\mathbf{x} \|^{2}}{2})\exp({-\mathbf{u}}^{\top}\mathbf{x})$

% $\phi_m^{1,\mathrm{trig}}(\mathbf{x})=\exp(\frac{\|\mathbf{x} \|^{2}}{2})\sin({\mathbf{v}}^{\top}\mathbf{x}),   \phi_m^{2,\mathrm{trig}}(\mathbf{x})=\frac{1}{\sqrt{2}}\exp(-\frac{\|\mathbf{x} \|^{2}}{2})\cos({\mathbf{v}}^{\top}\mathbf{x})$



% \begin{align}
% \begin{split}
% \widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})=\widehat{\lambda}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y}) + (1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y}) \\
% = (\frac{1}{r}\sum_{i=1}^r \xi_{\lambda}(\mathbf{x},\omega_i)\xi_{\lambda}(\mathbf{y},\omega_i))(\frac{1}{m}\sum_{j=1}^2 \sum_{k=1}^m \phi_{m,k}^{j,++}(\mathbf{x})\phi_{m,k}^{j,++}(\mathbf{y}))  \\ + (1 - \frac{1}{r}\sum_{i=1}^r \xi_{\lambda}(\mathbf{x},\omega_i)\xi_{\lambda}(\mathbf{y},\omega_i))(\frac{1}{m}\sum_{j=1}^2 \sum_{k=1}^m \phi_{m,k}^{j,\mathrm{trig}}(\mathbf{x})\phi_{m,k}^{j,\mathrm{trig}}(\mathbf{y})) \\
% = \frac{1}{mr}\sum_{i=1}^{r}\sum_{k=1}^{m}(\xi_{\lambda}(\mathbf{x},\omega_i)\phi_{m,k}^{1,++}(\mathbf{x})\xi_{\lambda}(\mathbf{y},\omega_i)\phi_{m,k}^{1,++}(\mathbf{y})+\xi_{\lambda}(\mathbf{x},\omega_i)\phi_{m,k}^{2,++}(\mathbf{x})\xi_{\lambda}(\mathbf{y},\omega_i)\phi_{m,k}^{2,++}(\mathbf{y})) \\
% + 
% \end{split}
% \end{align}


In the following subsections, $k$ represents the number of samples we use to estimate $\hat{\lambda}(\mathbf{x},\mathbf{y})$. $m_1$ and $m_2$ are the number of samples we use to estimate $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$ respectively.


\subsection{Lambda-Angular Hybrid Estimator}


\begin{equation}
\lambda(\theta) = \frac{\theta}{\pi} = 
\frac{1}{2} - \frac{1}{2}\mathbb{E}[(\phi_{n}^{\mathrm{ang}}(\mathbf{x}))^{\top}\phi_{n}^{\mathrm{ang}}(\mathbf{y})]
\end{equation}

\begin{equation}
\hat{\lambda}(\theta) =
\frac{1}{2} - \frac{1}{2k}\sum_{i=1}^k \mathrm{sgn}(\tau_{i}^{\top}\mathbf{x})\mathrm{sgn}(\tau_{i}^{\top}\mathbf{y})
\end{equation}


Thus we can construct random feature maps for $\widehat{\lambda}_{k}(\mathbf{x},\mathbf{y}) = a - (\phi_{k}^{\lambda}(\mathbf{x}))^{\top}
\phi_{k}^{\lambda}(\mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = \frac{1}{2} \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{2k}}(\mathrm{sgn}(\tau_{1}^{\top}\mathbf{z}),...,\mathrm{sgn}(\tau_{n}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{k} \sim \mathcal{N}(0,\mathbf{I}_{d})$.


To calculate the MSE, we have:

\begin{align}
\begin{split}
\mathrm{Var}[\hat{\lambda}(\theta)]=\mathrm{Var}[\frac{1}{2} - \hat{\lambda}(\theta)]=\mathrm{Var}[\frac{1}{2k}\sum_{i=1}^k\mathrm{sgn}(\tau_{i}^{\top}\mathbf{x})\mathrm{sgn}(\tau_{i}^{\top}\mathbf{y})] 
=\frac{1}{4k}\mathrm{Var}[\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y})]\\
=\frac{1}{4k}(\mathbb{E}[(\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y}))^2] - \mathbb{E}[\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y})]^2) 
= \frac{1}{4k}(1 - (1-
\frac{2\theta}{\pi})^2) 
=\frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})]
\end{split}
\end{align}


\begin{align}
\begin{split}
\mathrm{E}[\hat{\lambda}(\theta)^2] = Var[\hat{\lambda}] + \mathrm{E}[\hat{\lambda}(\theta)]^2 = \frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] + \frac{\theta^2}{\pi^2} 
\end{split}
\end{align}


\begin{align}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\theta))^2] = 1-2\mathrm{E}[\hat{\lambda}(\theta)] + \mathrm{E}[\hat{\lambda}(\theta)^2] = 1 - \frac{2\theta}{\pi} + \frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] + \frac{\theta^2}{\pi^2}
 = (1-\frac{\theta}{\pi})^2 +\frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] 
\end{split}
\end{align}



\begin{align}
\begin{split}
\mathrm{E}[\hat{\lambda}(\theta)(1-\hat{\lambda}(\theta))] = \mathrm{E}[\hat{\lambda}(\theta)] - \mathrm{E}[\hat{\lambda}(\theta)^2] = \frac{\theta}{\pi} - (\frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] + \frac{\theta^2}{\pi^2} ) = \frac{\theta}{\pi}(1-\frac{\theta}{\pi})(1-\frac{1}{k})
\end{split}
\end{align}


If we generate $\omega_i$ independently for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
= [\frac{\theta^2}{\pi^2}+ \frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y}))  +  [(1-\frac{\theta}{\pi})^2 +\frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{split}
\end{align}


with $\|x\|^2=\|y\|^2=r^2$:

\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)) \\
= [\frac{\theta^2}{\pi^2}+ \frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r))  +  [(1-\frac{\theta}{\pi})^2 +\frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{split}
\end{align}


If we use exactly the same $\omega_i$ for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))\\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]\\
= [\frac{\theta^2}{\pi^2}+ \frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y}))  +  [(1-\frac{\theta}{\pi})^2 +\frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\frac{\theta}{\pi}(1-\frac{\theta}{\pi})(1-\frac{1}{k})
\end{split}
\end{align}



$\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r))$ will remain the same when $\|x\|^2=\|y\|^2=r^2$ since $\cos(\|x\|_2^2-\|y\|_2^2)=1$.





\subsection{Arc-cosine Kernel with $n\geq1$}

We could derive MSE for arccosine kernel with $n\geq1$ if we could calculate the following expectation:
 $\mathbb{E}_{\tau \sim N(0,1_d)}[\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y})(\tau^{\top}\mathbf{x})^{2n}(\tau^{\top}\mathbf{y})^{2n}]$, where $n\in N^{+}$ .
 
 
 
\subsection{Gaussian Hybrid Estimator}
 
\begin{equation}
\lambda(\mathbf{x},\mathbf{y}) = 1- \exp(-\frac{\lambda^2}{2}\|\mathbf{x-y}\|^{2}) = 1- \mathbb{E}[\cos(\lambda \omega^{\top}(\mathbf{x-y}))]
\end{equation}

\begin{equation}
\hat{\lambda}(\mathbf{x},\mathbf{y}) = 1- \frac{1}{k}\sum_{i=1}^k \cos(\lambda (\omega_i^{\top}(\mathbf{x}-\mathbf{y})))
\end{equation}



Thus we can construct random feature maps for $\widehat{\lambda}_{k}(\mathbf{x},\mathbf{y}) = a - (\phi_{k}^{\lambda}(\mathbf{x}))^{\top}
\phi_{k}^{\lambda}(\mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = 1 \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{k}}(\sin(\tau_{1}^{\top}\mathbf{z}), \cos(\tau_{1}^{\top}\mathbf{z}),...,\sin(\tau_{k}^{\top}\mathbf{z}), \cos(\tau_{k}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{k} \sim \mathcal{N}(0,\mathbf{I}_{d})$.


To calculate the MSE, we have:



Using the fact that (see: Lemma 1 in \cite{yu2016ORF}):

\begin{equation}
\mathrm{Var}[\cos(\lambda\omega^{\top}\Delta)] = \frac{1}{2}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{equation}

\begin{equation}
\mathrm{E}[\cos(\lambda\omega^{\top}\Delta)] = \exp(-\frac{\lambda^2}{2}\|\Delta\|^2)
\end{equation}

Then we could derive:

\begin{equation}
\begin{split}
\mathrm{E}[\cos(\lambda\omega^{\top}\Delta)^2] = \mathrm{Var}[\cos(\lambda\omega^{\top}\Delta)] + \mathrm{E}[\cos(\lambda\omega^{\top}\Delta)]^2   = \frac{1}{2}(1-\exp(-\lambda^2\|\Delta\|^2))^2 + \exp(-\frac{\lambda^2}{2}\|\Delta\|^2)^2
\\ = \frac{1}{2} + \frac{1}{2}\exp(-2\lambda^2\|\Delta\|^2) -\exp(-\lambda^2\|\Delta\|^2) + \exp(-\lambda^2\|\Delta\|^2) 
= \frac{1}{2}(1+\exp(-2\lambda^2\|\Delta\|^2))
\end{split}
\end{equation}


Therefore, 

\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \mathrm{E}[(\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega_i^{\top}\Delta))^2] = 
\frac{1}{k}\mathrm{E}[\cos(\lambda \omega^{\top}\Delta)^2] + (1-\frac{1}{k})\mathrm{E}[\cos(\lambda \omega^{\top}\Delta)]^2 \\= 
 \frac{1}{2k}(1+\exp(-2\lambda^2\|\Delta\|^2)) + (1-\frac{1}{k})\exp(-\lambda^2\|\Delta\|^2) \\
 = \exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1+\exp(-2\lambda^2\|\Delta\|^2)-2\exp(-\lambda^2\|\Delta\|^2)) \\
 = \exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}




\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})^2] = 1-2\mathrm{E}[1-\hat{\lambda}(\mathbf{x},\mathbf{y})] + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] 
= 1 - 2\mathrm{E}[\cos(\lambda\omega^{\top}\Delta)] + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= 1 - 2 \exp(-\frac{\lambda^2}{2}\|\Delta\|^2) +  \exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= (1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}



\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))] = \mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})] - \mathrm{E}[(\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\ 
= 1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}) - (1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 - \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}))-\frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 
\end{split}
\end{equation}


For $\|x\|_2^2=\|y\|_2^2=r^2$, we could rewrite as:

\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{r},\mathbf{\theta}))^2] 
 = \exp(-4\lambda^2 r^2 \sin(\frac{\theta}{2})^2) + \frac{1}{2k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}


\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{r},\mathbf{\theta})^2] 
= (1-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}




If we generate $\omega_i$ independently for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
= [(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{split}
\end{align}





\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)) \\
=  [(1-\exp(-2\lambda^2r^2\sin(\frac{\theta}{2})^2))^2 + \frac{1}{2k}(1-\exp(-4\lambda^2r^2\sin(\frac{\theta}{2})^2))^2]   \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) \\ +      [\exp(-4\lambda^2r^2\sin(\frac{\theta}{2})^2) + \frac{1}{2k}(1-\exp(-4\lambda^2r^2\sin(\frac{\theta}{2})^2))^2] \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{split}
\end{align}




If we use exactly the same $\omega_i$ for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))\\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]\\
= [(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
-\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))[\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}))-\frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]
\end{split}
\end{align}





If we do not have the condition $\|x\|^2=\|y\|^2=r^2$, the MSE of gaussian hybrid estimator will be positive (rather than equal to zero) at $\theta=\pi$. This might be problematic since $\lambda(\mathbf{x}, \mathbf{y})$ is a very small positive number at $\theta=\pi$.





\subsection{Truncated Gaussian Hybrid Estimator}

If we have the condition $\|x\|^2=\|y\|^2=r^2$, we could propose a truncated version of the gaussian hybrid estimator, which will satisfy ${\lambda}(\mathbf{x},\mathbf{y})=0$ at $\theta=0$, and ${\lambda}(\mathbf{x},\mathbf{y})=1$ at $\theta=\pi$.

\begin{equation}
\lambda(\mathbf{x},\mathbf{y}) = \frac{1-\exp(-\frac{\lambda^2}{2}\|\mathbf{x-y}\|^{2})}{1-\exp(-2\lambda^2r^2)} = \frac{1-\exp(-2\lambda^2r^2\sin(\frac{\theta}{2})^2)}{1-\exp(-2\lambda^2r^2)}
\end{equation}

Take $\gamma=1-\exp(-2\lambda^2r^2)$, we have:

\begin{equation}
\lambda(\mathbf{x},\mathbf{y}) = \frac{1-\exp(-\frac{\lambda^2}{2}\|\mathbf{x-y}\|^{2})}{\gamma} \\ 
= \frac{1- \mathbb{E}[\cos(\lambda \omega^{\top}(\mathbf{x-y}))]}{\gamma}
\end{equation}


\begin{equation}
\hat{\lambda}(\mathbf{x},\mathbf{y}) = \frac{1}{\gamma} - \frac{1}{k\gamma}\sum_{i=1}^k \cos(\lambda (\omega_i^{\top}(\mathbf{x}-\mathbf{y})))
\end{equation}



Thus we can construct random feature maps for $\widehat{\lambda}_{k}(\mathbf{x},\mathbf{y}) = a - (\phi_{k}^{\lambda}(\mathbf{x}))^{\top}
\phi_{k}^{\lambda}(\mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = \frac{1}{\gamma} \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{k\gamma}}(\sin(\tau_{1}^{\top}\mathbf{z}), \cos(\tau_{1}^{\top}\mathbf{z}),...,\sin(\tau_{k}^{\top}\mathbf{z}), \cos(\tau_{k}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{k} \sim \mathcal{N}(0,\mathbf{I}_{d})$.


To calculate the MSE, we have:


\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \frac{1}{\gamma^2} \mathrm{E}[(\gamma-1+\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\ 
= \frac{1}{\gamma^2} \mathrm{E}[ (\gamma-1)^2 + 2(\gamma-1)(\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y}))) + (\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y})))^2 ] \\
=\frac{(1-\gamma)^2}{\gamma^2}+\frac{2(\gamma-1)}{\gamma^2}\mathrm{E}[\cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y}))]+\frac{1}{\gamma^2}\mathrm{E}[(\frac{1}{k}\sum_{i=1}^k\cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\
= \frac{(1-\gamma)^2}{\gamma^2}+\frac{2(\gamma-1)}{\gamma^2}\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})+\frac{1}{\gamma^2}\exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= \frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}



\begin{equation}
\begin{split}
\mathrm{E}[(\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] = 1-2\mathrm{E}[1-\hat{\lambda}(\mathbf{x},\mathbf{y})] + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] 
= -1 + \frac{2}{\gamma}- \frac{2}{\gamma}\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}) + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= -1 + \frac{2}{\gamma}- \frac{2}{\gamma}\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}) + \frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= \frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}



\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))] = \mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})] - \mathrm{E}[(\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\ 
= \frac{1}{\gamma}(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})) - \frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 - \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 
\end{split}
\end{equation}




For $\|x\|_2^2=\|y\|_2^2=r^2$, we could rewrite as:

\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{r},\mathbf{\theta}))^2] 
 = \frac{1}{\gamma^2}((1-\gamma)-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}


\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{r},\mathbf{\theta})^2] 
= \frac{1}{\gamma^2}(1-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}


This truncated version with be the same as the vanilla version if $\gamma=1$.




If we generate $\omega_i$ independently for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
= [\frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{split}
\end{align}





\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)) \\
=  [\frac{1}{\gamma^2}(1-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2]   \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) \\ +      [\frac{1}{\gamma^2}((1-\gamma)-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2] \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{split}
\end{align}




If we use exactly the same $\omega_i$ for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))\\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]\\
= [\frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) 
-\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})* \\
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))  [\frac{1}{\gamma}(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})) - \frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 - \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 ]
\end{split}
\end{align}






\subsection{Product Hybrid Estimator}

We could rewrite the softmax kernel as product of $\mathrm{SM}^{++}(\mathbf{x},\mathbf{y})$ and $\mathrm{SM}^{\mathrm{trig}}(\mathbf{x},\mathbf{y})$:

\begin{equation}
\exp(2\mathbf{x}^{\top} \mathbf{y}) = \exp(-\frac{\|\mathbf{x}-\mathbf{y}\|^2}{2})\exp(\frac{\|\mathbf{x}+\mathbf{y}\|^2}{2}) = \mathrm{E}[\cos(\omega^{\top}\Delta)]\mathrm{E}[\frac{\exp(\omega^{\top}\mathbf{z})+\exp(-\omega^{\top}\mathbf{z})}{2}] 
\end{equation}


Define:
\begin{equation}
\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\mathbf{x},\mathbf{y}) = \frac{1}{m_1}\sum_{i=1}^{m_1} \cos(\omega_i^{\top}\Delta)
\end{equation}

\begin{equation}
\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\mathbf{x},\mathbf{y}) = \frac{1}{2 m_2}\sum_{j=1}^{m_2} (\exp(\omega_j^{\top}\mathbf{z})+\exp(-\omega_j^{\top}\mathbf{z}))
\end{equation}

Then our hybrid estimator could be defined as:
\begin{equation}
\widehat{\mathrm{SM}}_{m_1,m_2}^{\mathrm{hyb}}(\mathbf{x},\mathbf{y}) = \widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})
\end{equation}

Next, the variance of these two estimators are:

\begin{equation}
\mathrm{Var}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\mathbf{x},\mathbf{y})] = \frac{1}{2 m_1}(1-\exp(-\|\Delta\|^2))^2
\end{equation}

\begin{equation}
\mathrm{Var}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\mathbf{x},\mathbf{y})] = \frac{1}{2 m_2}(\exp(\|\mathbf{z}\|^2)-1)^2
\end{equation}


We could then calculate the MSE of this hybrid estimator:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m_1, m_2}(\mathbf{x},\mathbf{y})) 
= \mathrm{Var}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]\mathrm{Var}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})] \\
+ \mathrm{Var}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]\mathrm{E}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]^2 + \mathrm{Var}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]\mathrm{E}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]^2 \\
= \frac{1}{4 m_1 m_2}(1-\exp(-\frac{\|\Delta\|^2}{2}))^2(\exp(\frac{\|\mathbf{z}\|^2}{2})-1)^2 \\
+ \frac{1}{2 m_1}(1-\exp(-\frac{\|\Delta\|^2}{2}))^2\exp(\frac{\|\mathbf{z}\|^2}{2}) + \frac{1}{2 m_2}(\exp(\frac{\|\mathbf{z}\|^2}{2})-1)^2\exp(-\frac{\|\Delta\|^2}{2})
\end{split}
\end{align}


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m_1, m_2}(r,\mathbf{\theta})) 
= \frac{1}{4 m_1 m_2}(1-\exp(-2r^2\sin(\frac{\theta}{2})^2))^2(1-\exp(2r^2\cos(\frac{\theta}{2})^2))^2 \\
+ \frac{1}{2 m_1}(1-\exp(-2r^2\sin(\frac{\theta}{2})^2))^2\exp(2r^2\cos(\frac{\theta}{2})^2) + \frac{1}{2 m_2}(1-\exp(2r^2\cos(\frac{\theta}{2})^2))^2\exp(-2r^2\sin(\frac{\theta}{2})^2)
\end{split}
\end{align}








\newpage


\subsection{Lambda Hybrid Estimator}

If the input matrices $\mathbf{Q}, \mathbf{K}$ can be clustered into $n_q$ and $n_k$ groups respectively (using k-means clustering algorithm for example), with the center point of each group as $\mathbf{r}_i$, ($i=1,...,n_k$) and $\mathbf{r}_j$, ($j=1,...,n_q$), then there exist $n_q n_k$ pairs of $(\mathbf{r}_i, \mathbf{r}_j)$, ($i=1,...,n_q, j=1,...,n_k$), so we can construct $n_q n_k$ softmax estimators to estimate cross-group softmax values. \textcolor{red}{In the next subsection, we use $\mathbf{x}$ and $\mathbf{y}$ to represent a pair of such centers $\mathbf{r}_i$ and $\mathbf{r}_j$}.


\subsubsection{Construction for matrix $\mathbf{A}$}

Consider $\mathbf{z} = \mathbf{Ax} + \mathbf{(A^{\top})^{-1}y}$ for an invertible (in $\mathbb{C}^{d \times d})$ matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$, an estimator based on this mechanism has variance equal to $0$ if:
\begin{equation}
\label{eq:z_ax_by_0}
\mathbf{z} = \mathbf{Ax} + \mathbf{(A^{\top})^{-1}y} = 0
\end{equation}

We assume here that $\mathbf{A}$ is a diagonal matrix, so $\mathbf{A}=\mathbf{A^{\top}}$. Then we can rewrite the above equation as:
\begin{equation}
\mathbf{z} = \mathbf{Ax} + \mathbf{(A)^{-1}y} = 0
\end{equation}

Since position $(k,k)$ in matrix $\mathbf{A}$ has the form $\alpha_k + \beta_k i$, we need to satisfy the following equation for each k=1,...,d:
\begin{equation}
(\alpha_k + \beta_k i)x_k + \frac{1}{\alpha_k + \beta_k i}y_k = 0
\end{equation}

\begin{equation}
(\alpha_k + \beta_k i)x_k + \frac{\alpha_k - \beta_k i}{\alpha_k^2 + \beta_k^2 }y_k = 0
\end{equation}

We can simplify this equation and separate into real and imaginary part:
\begin{equation}
\left\{ \begin{array}{rcl}
\mathbf{Re}: (\alpha_k^2+\beta_k^2)\alpha_k x_k + \alpha_k y_k = 0 \\ 
\mathbf{Im}: (\alpha_k^2+\beta_k^2)\beta_k x_k - \beta_k y_k = 0 \\ 
\end{array}\right.
\end{equation}

Our goal now is to choose values for $\alpha_k$ and $\beta_k$ given $x_k$ and $y_k$.

If $x_k y_k>0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=0 \\ 
\beta_k=\sqrt{y_k/x_k} \\ 
\end{array}\right.
\end{equation}

And if $x_k y_k<0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=\sqrt{-y_k/x_k} \\ 
\beta_k= 0\\ 
\end{array}\right.
\end{equation}


When $x_k=y_k=0$,  we could assume $\alpha_k=\beta_k=1$. However, if $x_k=0, y_k\neq 0$ or $x_k\neq 0, y_k=0$, then we cannot satisfy the above equation perfectly. We could assume $\alpha_k$ to some large positive value and set $\beta_k=0$ if  $x_k=0, y_k\neq 0$. And assume $\alpha_k=\beta_k$ to be some small positive value close to zero if $x_k\neq 0, y_k=0$.


Now suppose 
$\mathbf{A} = \mathrm{diag}(a_1,\cdots,a_d) \in \R^{d \times d}$, then maybe we cannot make
$\mathbf{Ax} + \mathbf{(A)^{-1}y} = 0$. However, we can still    minimize $\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|
= \sqrt{\sum_{k=1}^d (a_k x_k + \frac{1}{a_k}y_k)^2}$ by taking

\begin{equation}
 a_k = \sqrt{\left|
\frac{y_k}{x_k}
\right|} 
\end{equation}

if $x_k \neq 0$. If $x_k = 0$, we could set $a_k$ to some large positive value.




\subsubsection{Construction for Softmax Estimator}

From equation (16):
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{Ax}\|^{2}}{2})  
\mathrm{exp}(\frac{\|\mathbf{A}^{-1}\mathbf{y}\|^{2}}{2})\mathrm{SM}(\mathbf{x},\mathbf{y})  
= \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{Ax}+\mathbf{A}^{-1}\mathbf{y})]
\end{equation}


The softmax can be estimated as:

\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{\mathbf{A}^{-1}}(\mathbf{y})]
\end{equation}

where

\begin{equation}
\Psi^{m}_{\mathbf{A}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{Ax}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{Ax}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Ax}))^{\top}
\end{equation}

\begin{equation}
\Psi^{m}_{\mathbf{A^{-1}}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A^{-1}y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A^{-1}y}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A^{-1}y}))^{\top}
\end{equation}

for $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$.

And such softmax estimator will have variance of zero if $\mathbf{x}=\mathbf{r}_x$ and $\mathbf{y}=\mathbf{r}_y$, where $\mathbf{r}_x$ and $\mathbf{r}_y$ are the centes vector $\mathbf{x}$ and $\mathbf{y}$ belong to respectively. For other pairs of vectors close to $\mathbf{r}_x$ and $\mathbf{r}_y$, the variance should be small.  


\subsubsection{Construction for Lambda Coefficients}
\begin{align}
\begin{split}
\mathrm{exp}(-\frac{\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|^{2}}{2\tau^2}) = 
\mathrm{exp}(-\frac{\|\mathbf{Ax}\|^2 + \|\mathbf{(A)^{-1}y}\|^{2} + 2 (\mathbf{Ax})^{\top}(\mathbf{(A)^{-1}y})}{2\tau^2}) \\
= \mathrm{exp}(-\frac{\|\mathbf{Ax}\|^{2}}{2\tau^2})\mathrm{exp}(-\frac{\|\mathbf{(A)^{-1}y}\|^{2}}{2\tau^2})\mathrm{exp}(\frac{\mathbf{x}^{\top}(\mathbf{-y})}{\tau^2})
\end{split}
\end{align}

where $\mathrm{exp}(\frac{\mathbf{x}^{\top}(\mathbf{-y})}{\tau^2}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}}(\mathbf{x}/\tau)^{\top} 
\Psi^{m}_{\mathbf{A}^{-1}}(\mathbf{-y}/\tau)]$

and $\Psi^{m}_{\mathbf{A}}(\mathbf{z}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{Mz}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{Mz}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Mz}))^{\top}$ and $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$, for $\mathbf{z}=\{\frac{\mathbf{x}}{\tau}, \frac{\mathbf{-y}}{\tau}$\}.


we can put it together and derive:
\begin{align}
\begin{split}
\mathrm{exp}(-\frac{\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|^{2}}{2\tau^2}) = \mathbb{E}[\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{\tau, m}_{\mathbf{A}^{-1}}(\mathbf{-y})]
\end{split}
\end{align}

where
\begin{equation}
\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{Ax}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{Ax}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Ax}/\tau))^{\top}
\end{equation}
\begin{equation}
\Psi^{\tau, m}_{\mathbf{A^{-1}}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|\mathbf{(A^{-1}y)}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}\mathbf{A^{-1}\mathbf{y}}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}\mathbf{A^{-1}\mathbf{y}}/\tau))^{\top}
\end{equation}


Recall from (\ref{exp - norm cos}) that
\begin{equation} 
\mathrm{exp}(-\frac{\|\mathbf{x}-\mathbf{y}\|^{2}}{2}) = \mathbb{E}[\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))],   
\end{equation}
we can derive


\begin{align}
\begin{split}
\mathrm{exp}(-\frac{\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|^{2}}{2\tau^2}) = \mathbb{E}[\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{\tau, m}_{\mathbf{A}^{-1}}(\mathbf{-y})]
\end{split}
\end{align}

where
\begin{equation} \label{hybrid for matrix x}
\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x}) =     
\sqrt{\frac{1}{m}}
(\sin(\omega_{1}^{\top}\mathbf{Ax}/\tau),
\cos(\omega_{1}^{\top}\mathbf{Ax}/\tau),
...,
\sin(\omega_{m}^{\top}\mathbf{Ax}/\tau),
\cos(\omega_{m}^{\top}\mathbf{Ax}/\tau)
)^{\top}
\end{equation}

\begin{equation} \label{hybrid for matrix y}
\Psi^{\tau, m}_{\mathbf{A^{-1}}}(\mathbf{y}) =   
\sqrt{\frac{1}{m}}  
(\sin(-\omega_{1}^{\top}\mathbf{A^{-1}y}/\tau),
\cos(-\omega_{1}^{\top}\mathbf{A^{-1}y}/\tau),
...,
\sin(-\omega_{m}^{\top}\mathbf{A^{-1}y}/\tau),
\cos(-\omega_{m}^{\top}\mathbf{A^{-1}y}/\tau)
)^{\top}
\end{equation}

\subsubsection{Multiple Softmax Estimators}

We assume here that we need $p=n_q n_k$ softmax estimators, with $n_q, n_k$ defined at the beginning of this section. Then as stated in Section 1.5, we denote $\mathcal{E}=( \widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of the softmax-kernel $\mathrm{SM}^{i,j}(\mathbf{x},\mathbf{y})$ and $\Lambda = \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of $\lambda^{i,j}(\mathbf{x},\mathbf{y})$ for some functions $\lambda^{i,j}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, constructed independently from $\mathcal{E}$.

Then our hybrid estimator takes the following:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y})
\end{equation}

with constraint:

\begin{equation}
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) = 1
\end{equation}


If we define $\mathbf{A}^{i,j}$ as the composite matrix satisfies Eq. \ref{eq:z_ax_by_0} with $\mathbf{x}, \mathbf{y}$ replaced by center $\mathbf{r}_i, \mathbf{r}_j$ from $\mathbf{Q}$ and $\mathbf{K}$, then:

\begin{equation}
\widehat{\lambda}^{i,j}(\mathbf{x}, \mathbf{y}) = \Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} \Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) 
\end{equation}

with $\Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y})$ given by:


\begin{equation}
\Psi^{\tau, m}_{\mathbf{A}^{i,j}} (\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j} \mathbf{x}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau))^{\top}
\end{equation}

\begin{equation}
\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau))^{\top}
\end{equation}



\begin{equation}
\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top}\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})
\end{equation}

with $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})$ given by:

\begin{equation}
\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j}\mathbf{x}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j}\mathbf{x}))^{\top}
\end{equation}

\begin{equation}
\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}),...,\mathrm{exp}(\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}))^{\top}
\end{equation}




% \subsubsection{Multiple Softmax Estimators}

% we assume here that we need $p+1={n \choose 2}+1$ softmax estimators, with the fist ${n \choose 2}$ estimators generated with of $(\mathbf{r}_i,\mathbf{r}_j)$, ($i\neq j \in 1, ..., n$), and the last one as tri-geometric softmax estimator.


% As stated in Section 1.5, we denote $\mathcal{E}=( \asm )_{k=1}^{p+1}$ as a list of estimators of the softmax-kernel $\sm$ and $\Lambda = ( \alamgen )_{k=1}^{p}$ as a list of estimators of: 
% $\{\lambda^{k}(\mathbf{x},\mathbf{y})\}_{k=1}^{p}$ for some functions
% $\lambda^{k}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, constructed independently from $\mathcal{E}$.

% Then our hybrid
% Take the following estimator of $\sm$:
% \begin{equation}
% \widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
% \sum_{k=1}^{p} \alamgen \asm + \left(1-\sum_{k=1}^{p} \alamgen \right)\widehat{\mathrm{SM}}^{p+1}(\mathbf{x},\mathbf{y})
% \end{equation}

% where 
% \begin{equation}
% \hat{\lambda}^k(\mathbf{x}, \mathbf{y}) = \Psi^{\tau, m}_{\mathbf{A_k}}(\mathbf{x})^{\top} \Psi^{\tau, m}_{\mathbf{A_k^{-1}}}(\mathbf{-y}) 
% \end{equation}

% with $\Psi^{\tau, m}_{\mathbf{A_k}}(\mathbf{x})$ and $\Psi^{\tau, m}_{\mathbf{A_k^{-1}}}(\mathbf{-y})$ given by:


% \begin{equation}
% \Psi^{\tau, m}_{\mathbf{A}_k}(\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{A_k x}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{A_k x}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A_k x}/\tau))^{\top}
% \end{equation}
% \begin{equation}
% \Psi^{\tau, m}_{\mathbf{A_k^{-1}}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|\mathbf{(A^{-1}_k y)}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}\mathbf{A^{-1}_k \mathbf{y}}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}\mathbf{A^{-1}_k \mathbf{y}}/\tau))^{\top}
% \end{equation}


% and $\mathbf{A}_k$ constructed from $(\mathbf{r}_i,\mathbf{r}_j)$, ($i\neq j \in 1, ..., n$) as stated in subsection 2.6.1.

% \begin{equation}
% \widehat{\mathrm{SM}}^{\mathrm{k}}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}_k}(\mathbf{x})^{\top}\Psi^{m}_{\mathbf{A^{-1}}_k}(\mathbf{y})
% \end{equation}

% with $\Psi^{m}_{\mathbf{A}_k}(\mathbf{x})$ and $\Psi^{m}_{\mathbf{A^{-1}}_k}(\mathbf{y})$ given by:

% \begin{equation}
% \Psi^{m}_{\mathbf{A_k}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A_k x}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A_k x}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A_k x}))^{\top}
% \end{equation}

% \begin{equation}
% \Psi^{m}_{\mathbf{A_k^{-1}}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A_k^{-1}y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A_k^{-1}y}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A_k^{-1}y}))^{\top}
% \end{equation}


% and the last softmax estimator is just the tri-geometric estimator:
% \begin{equation}
% \widehat{\mathrm{SM}}^{p+1}(\mathbf{x},\mathbf{y}) = \widehat{\mathrm{SM}}^{\mathrm{trig}}_m(\mathbf{x},\mathbf{y})
% \end{equation}






\newpage


\newpage


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1 d=64 m=128 unmodified.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1 d=64 m=16384 unmodified.png}}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Angular r=1, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Gaussian r=1, d=64 sigma=4.png}
    \end{center}
    \end{minipage}
\end{figure}



\newpage


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.25 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.25 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep16 ERR Angular r=1.25, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep16 ERR Gaussian r=1.25, d=64 sigma=4.png}
    \end{center}
    \end{minipage}
\end{figure}




\newpage




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.5 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.5 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1.5 d=64 m=128 unmodified.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1.5 d=64 m=16384 unmodified.png}}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Angular r=1.5, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Gaussian r=1.5, d=64 sigma=2.png}
    \end{center}
    \end{minipage}
\end{figure}




\newpage



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Angular r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep16 ERR Gaussian r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\iffalse


\newpage

\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/With relative error Angular r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/With relative error Truncated Gaussian r=2, sigma=1, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/With relative error Angular r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\newpage

\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/TrigPos r=2 d=64 m=128.png}
    \end{center}
    \end{minipage}
\end{figure}



\fi


\newpage


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep26 Comparison on PTB Dataset.png}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/ComparisonOfFullSoftmaxWithDifferentTau.png}
    \end{center}
    \end{minipage}
\end{figure}





\iffalse

\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/r=1, lambda=1, k=m=32.png}
    \end{center}
    \end{minipage}
\end{figure}




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/r=1.5, lambda=1, k=m=32.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/r=2, lambda=1, k=m=32.png}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/new_plots/TrigPos r=1 d=64 m=128.png}
    \end{center}
    \end{minipage}
\end{figure}








\fi



==> Hybrid Estimators (Camera-ready, Arxiv)/redo_wasserstein.tex <==
POS:  normalize=True (i.e. divide by sqrt(D)) (Need this otherwise too spiky gets division by 0 or blows up) 
Wass between 1 D :
(Current issues with the logic. Redo )
-----
64 dims : (previous calc: 0.0001733546709
3873.522346493703

128 dims:
(Prev calc : 0.0001751364405407047)
3834.3128269357208

256 dims:
(prev calc: 0.00017551147489137665)
3836.4489776151413

512 dims : 
prev calc: 0.0001757072986050169
3832.2541091130906

------
RFF (Same normalization as before)
64 dims: #neg probabilities = 389655751
1273 rows of all negatives
(prev calc: 0.00017034180235048712)
3918.9444470390827

128 dims: 382700527
1200 rows of all negatives
(prev calc: 0.00017037847641404884)
3919.3135769811192

256 dims: 380736251
1092 rows of all negs
(prev calc: 0.00017053129410996915)
3917.8634291038607

512 dims: 366352621
965 rows of all negs
(prev calc: 0.00017061456789765432)
3913.5533617588962

1024 dims: 348862312
907 rows of all negatives 

------
Hybrid features
64 dim: no neg 
3998.771141585179

128 dim: no neg values
3994.5118933801004

256 dim: no neg values
3993.625978735541

512 dim:
3994.526124077072

-----
Hybrid (ang-hyb-att)
64 feats (8,8) 129550769 negs and no rows where all the rows are negative
3860.6802630547463

(32,4) 128 feats 148405849 negs and no rows all neg
3877.355791158878

(16,8): 128711703 negs
3872.474239515384

(8,16) 132652334 negs
3851.985026028889

256 feats:
----
(16,16)
128957063 negs
3882.2713117105845

(32, 8)
130409083 negs
3876.2982834701675

(8,32)
126829994 negs
3870.452882061927

512 feats:
(32,32) 128023674 negs
3879.110326448242

(64,8) 127018768 negs
3896.134624287219

(8, 64)
126331310 negs
University 3863.3471578142558

---------------------------------------------

WIKITEXT:
POS : 64
3.091665103802842e-05

128:
4.574975195924697e-05

256:
3.09050922059733e-05

512:
3.1471821742058816e-05

==> Hybrid Estimators (Camera-ready, Arxiv)/related_work-HRF.tex <==
\section{Related work}

==> Hybrid Estimators (Camera-ready, Arxiv)/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

==> Hybrid Estimators (Camera-ready, Arxiv)/theory-HRF.tex <==
\section{Hybrid Random Features}
\label{sec:hrf}
\vspace{-3mm}
\subsection{Preliminaries}
\vspace{-2mm}
Whenever we do not say explicitly otherwise, all presented lemmas and theorems are new.
We start with the following basic definitions and results.

\begin{definition}[Kernel with a Random Feature Map Representation]
We say that a kernel function $\mathrm{K}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ \textit{admits a random feature (RF) map representation} if it can be written as
\vspace{-2mm}\begin{equation}
\mathrm{K}(\mathbf{x},\mathbf{y}) = \mathbb{E}_{\omega \sim \Omega}\left[\sum_{i=1}^{l} \xi_{i}(\mathbf{x},\omega)\xi_{i}(\mathbf{y},\omega)\right]  ,  
\vspace{-2mm}\end{equation}
for some $\xi_{i}: \mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, and where $\omega$ is sampled from some probabilistic distribution $\Omega \in \mathcal{P}(\mathbb{R}^{d})$.
The corresponding random feature map, for a given $m \in \mathbb{N}$, is defined as
\vspace{-2mm}\begin{equation}
\label{random_feature_map_formula}
\phi_{m}(\mathbf{u}) = \frac{1}{\sqrt{m}} \phi_{m}^{1}(\mathbf{u}) \star ... \star \phi_{m}^{l}(\mathbf{u}) \in \mathbb{R}^{ml},  
\vspace{-2mm}\end{equation}
where $\phi_{m}^{i} = (\xi_{i}(\mathbf{u},\omega_{1}),...,\xi_{i}(\mathbf{u},\omega_{m}))^{\top}$, $\star$ stands for vertical concatenation, and %furthermore 
$\omega_{1},...,\omega_{m} \overset{\mathrm{iid}}{\sim} \Omega$.
\end{definition}
Random feature maps can be used to unbiasedly approximate corresponding kernels, as follows:
\begin{equation}
\widehat{\mathrm{K}}(\mathbf{x},\mathbf{y}) = \phi_{m}(\mathbf{x})^{\top}
\phi_{m}(\mathbf{y}).    
\end{equation}
Using the above notation, a trigonometric random feature $\phi_{m}^{\mathrm{trig}}$ from Equation \ref{tri} can be encoded as applying 
$l=2$, $\xi_{1}(\mathbf{u},\omega) = \sin(\omega^{\top}\mathbf{u})$, $\xi_{2}(\mathbf{u}, \omega) = \cos(\omega^{\top}\mathbf{u})$. Similarly, positive random features can be encoded as taking $l=2$ and $\xi_{1}(\mathbf{u},\omega) = \frac{1}{\sqrt{2}}\exp(\omega^{\top}\mathbf{u})$, $\xi_{2}(\mathbf{u}, \omega) = \frac{1}{\sqrt{2}}\exp(-\omega^{\top}\mathbf{u})$.   

The following result from \citep{performers} shows that the mean squared error (MSE) of the trigonometric estimator is small for large softmax kernel values and large for small softmax kernel values, whereas an estimator applying positive random features behaves in the opposite way.

Denote by $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})$ an estimator of $\mathrm{SM}(\mathbf{x}, \mathbf{y})$ for $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$ using trigonometric RFs and $\omega_{1}, ..., \omega_{m} \overset{\mathrm{iid}}{\sim} \mathcal{N}(0,\mathbf{I}_{d})$. Denote by $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})$ its analogue using positive RFs. We have:

\begin{lemma}[positive versus trigonometric RFs]
\label{mse-lemma}
Take $\Delta = \mathbf{x} - \mathbf{y}$, $\mathbf{z} = \mathbf{x} + \mathbf{y}$, 
$f_{1}(u) = (2m)^{-1}\exp(u^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})$,
$f_{2}(u) = (2m)^{-1}\exp(u^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})$,
$f_{3}(u)=(1-\exp(-u^{2}))^{2}$. The MSEs of these estimators are:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})) = f_{1}(\|\mathbf{z}\|_{2})f_{3}(\|\Delta\|_{2}), \textrm{ }
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})) = f_{2}(\|\mathbf{z}\|_{2})f_{3}(\|\mathbf{z}\|_{2}).
\end{split}
\end{align}
\end{lemma}



\subsection{The Algorithm}
\label{sec:algorithm}
We are ready to present the mechanism of \textit{Hybrid Random Features} (HRFs).
Denote by $\mathcal{E}=( \asm )_{k=1}^{p+1}$ a list of estimators of $\sm$ (the so-called \textit{base estimators}) and by $\Lambda = ( \alamgen )_{k=1}^{p}$ a list of estimators of 
$\{\lambda^{k}(\mathbf{x},\mathbf{y})\}_{k=1}^{p}$ for some functions
$\lambda^{k}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow [0,1]$, constructed independently from $\mathcal{E}$.
Take the following estimator of $\sm$:
\begin{equation}
\vspace{-2mm}
\label{gen-hyb-eque}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{k=1}^{p} \alamgen \asm + \left(1-\sum_{k=1}^{p} \alamgen \right)\widehat{\mathrm{SM}}^{p+1}(\mathbf{x},\mathbf{y})
\vspace{-2mm}\end{equation}

In the next section, we explain in detail how base estimators are chosen.
We call $\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y})$ a hybrid random feature (HRF) estimator of $\sm$ parameterized by $\mathcal{E},\Lambda$. 
The role of the $\lambda$-coefficients is to dynamically (based on the input $(\mathbf{x},\mathbf{y})$) prioritize or deprioritize certain estimators to promote those which are characterized by lower variance for a given input.
Note that if elements of $\mathcal{E}$ are unbiased estimators of $\sm$, then trivially $\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y})$ is also an unbiased estimator of $\sm$. Assume that each $\asm$ is of the form
$\asm = (\phi_{1,m}^{k}(\mathbf{x}))^{\top}\phi_{2,m}^{k}(\mathbf{y})$
for $\phi_{j,m}^{k}(\mathbf{u}) = \frac{1}{\sqrt{m}} 
\phi_{j,m}^{1,k}(\mathbf{u}) \star ... \star \phi_{j,m}^{t_{k},k}(\mathbf{u})$, $t_{k}>0$ and $\phi_{j,m}^{1,k},..., \phi_{j,m}^{t_{k},k}:\mathbb{R}^{d} \rightarrow \mathbb{R}^{m}$, where $j \in \{1,2\}$. Assume also that $\lambda^{k}(\mathbf{x},\mathbf{y})$ can be written as:
\begin{equation}
\label{lambda-eq}
\lambda^{k}(\mathbf{x},\mathbf{y}) = a_{k} + \mathbb{E}_{\tau \sim \Omega}[\sum_{i=1}^{l_{k}}f^{i}_{1,k}(\mathbf{x},\tau)f^{i}_{2,k}(\mathbf{y}, \tau)]  
\end{equation}
for some scalars $a_{k} \in \mathbb{R}$, distribution $\Omega \in \mathcal{P}(\mathbb{R}^{d})$ (where $\mathcal{P}(\mathbb{R}^{d}$ stands for the set of probabilistic distributions on $\mathbb{R}^{d}$), mappings $\xi^{i}_{k}, \eta^{i}_{k}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ and that the corresponding estimator $\widehat{\lambda}^{k}(\mathbf{x},\mathbf{y})=\widehat{\lambda}^{k}_{n}(\mathbf{x},\mathbf{y})$ of $\lambda^{k}(\mathbf{x},\mathbf{y})$ is of the form:
\begin{equation}
\label{lambda-eq-estimate}
\widehat{\lambda}^{k}_{n}(\mathbf{x},\mathbf{y}) = a_{k} + (\rho_{1,n}^{k}(\mathbf{x}))^{\top}   
\rho_{2,n}^{k}(\mathbf{y})
\end{equation}
for 
$
\rho_{j,n}^{k}(\mathbf{u}) =  \frac{1}{\sqrt{n}}\rho_{j,n}^{1,k}(\mathbf{u}) \star ... \star \rho_{j,n}^{l_{k},k}(\mathbf{u})
$, $\rho_{j,n}^{i,k}(\mathbf{u})=
(f^{i}_{j,k}(\mathbf{u},\tau_{1}),...,f^{i}_{j,k}(\mathbf{u},\tau_{n}))^{\top}$, $\tau_{1},...,\tau_{n} \sim \Omega$, and where
$j \in \{1,2\}$. Linearization of the $\lambda$-coefficients given by Equation \ref{lambda-eq} is crucial to obtain linearization of the hybrid estimators, and consequently random feature map decomposition.

We denote a hybrid estimator using $n$ random features for its base estimators and $m$ to approximate $\lambda$-coefficients as $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$. Furthermore, for two vectors $\mathbf{u},\mathbf{v}$, we denote their vectorized outer-product by $\mathbf{u} \otimes \mathbf{v}$. Finally, we denote by $\prod^{\star}$  vectors-concatenation.
Estimator  $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y})$ can be rewritten as a dot-product of two (hybrid) random feature vectors, as the next lemma shows. 

\begin{lemma}
\label{composite-lemma}
The HRF estimator $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y})$ satisfies
$\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y})=\Psi_{1}(\mathbf{x})^{\top}\Psi_{2}(\mathbf{y})$,
where $\Psi_{j}$
for $j \in \{1,2\}$
is given as $\Psi_{j}(\mathbf{z})=\Psi_{j}^{1}(\mathbf{z}) \star \Psi_{j}^{2}(\mathbf{z}) \star \Psi_{j}^{3}(\mathbf{z}) \star \Psi_{j}^{4}(\mathbf{z})$ and:
\begin{align}
\begin{split}
\label{hyb-all-2}
\Psi^{1}_{j}(\mathbf{z})=\prod_{k=1,...,p}^{\star} \sqrt{\frac{a_{k}}{m}}\phi_{j,m}^{1,k}(\mathbf{z})\star ... \star \phi_{j,m}^{t_{k},k}(\mathbf{z})\\
\Psi^{2}_{j}(\mathbf{z})=\frac{1}{\sqrt{mn}}\prod_{k=1,...,p}^{\star} \prod^{\star}_{i,j \in \{1,...,l_{k}\}\times\{1,...,t_{k}\}} \rho_{j,n}^{i,k}(\mathbf{z}) \otimes \phi_{j,m}^{j,k}(\mathbf{z})\\
\Psi^{3}_{j}(\mathbf{z})=\sqrt{\frac{1-\sum_{k=1}^{p} a_{k}}{m}}\phi_{j,m}^{1,p+1}(\mathbf{z})\star ... \star \phi_{j,m}^{t_{p+1},p+1}(\mathbf{z})\\
\Psi^{4}_{j}(\mathbf{z})=\frac{\mathbf{i}}{\sqrt{mn}}\prod_{k=1,...,p}^{\star} \prod^{\star}_{i,j \in \{1,...,l_{k}\}\times\{1,...,t_{p+1}\}} \rho_{j,n}^{i,k}(\mathbf{z}) \otimes \phi_{j,m}^{j,p+1}(\mathbf{z})\\
\end{split}    
\end{align}
\end{lemma}

\paragraph{Bipolar estimators:} A prominent special case of the general hybrid estimator defined above is the one
where: $\mathcal{E} = (\widehat{\mathrm{SM}}^{++}(\mathbf{x},\mathbf{y}),\widehat{\mathrm{SM}}^{\mathrm{trig}}(\mathbf{x},\mathbf{y}))$. Thus consider the following estimator $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y})=\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y}) + (1-\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y}).   
\end{equation}

The question arises whether  $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ defined in such a way can outperform both  $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$ and $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$. That of course depends also on the choice of $\lambda:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$.
If we consider a (common) normalized setting where all input vectors have the same norm, we can rewrite $\lambda(\mathbf{x},\mathbf{y})$ ad $\lambda(\theta_{\mathbf{x},\mathbf{y}},r)$, where $\theta_{\mathbf{x},\mathbf{y}}$ is an angle between $\mathbf{x}$ and $\mathbf{y}$ and $\|\mathbf{x}\|=\|\mathbf{y}\|=r$. By our previous analysis we know that $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$ becomes perfect for $\theta=\pi$ and $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$ becomes perfect for $\theta=0$. That suggests particularly simple linear dependence of $\lambda$ on $\theta$ to guarantee vanishing variance for both the critical values: $\theta=0$ and $\theta=\pi$. It remains to show that such a $\lambda$-coefficient can be linearized. It turns out that this can be done with a particularly simple random feature map mechanism, as we will show later, leading to the  so-called angular hybrid variant (see: Section \ref{sec:instantiations}).  

\subsection{Choosing base estimators for HRFs: Complex Exponential Estimators}
\label{sec:complex_estimators}
In this section, we explain how we choose base estimators in Equation \ref{gen-hyb-eque}. 
We denote by  $\mathbf{i}$ a complex number such that $\mathbf{i}^{2}=-1$.
The following lemma is a gateway to construct unbiased base estimators.
\begin{lemma}
\label{complex}
Let $\omega \sim \mathcal{N}(0,\mathbf{I}_{d})$. Then for every $\mathbf{z}=(z_{1},...,z_{d})^{\top} \in \mathbb{C}^{d}$ the following holds:
\begin{equation}
\mathbb{E}\left[\exp(\omega^{\top}\mathbf{z})\right] = \exp\left(\frac{\sum_{i=1}^{d}z_{i}^{2}}{2}\right).    
\end{equation}
\vspace{-5mm}
\end{lemma}
For a complex vector $\mathbf{z}=(z_{1},...,z_{d}) \in \mathbb{C}^{d}$, we denote $\mathbf{z}^{2} = \sum_{i=1}^{d} z_{i}^{2}$. Consider $\mathbf{z} = \mathbf{Ax} + \mathbf{(A^{\top})^{-1}y}$ for an invertible (in $\mathbb{C}^{d \times d})$ matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$.
Using Lemma \ref{complex}, we get:
\begin{equation}
\mathrm{exp}\left(\frac{(\mathbf{Ax})^{2}}{2}\right)  
\mathrm{exp}\left(\frac{((\mathbf{A}^{\top})^{-1}\mathbf{y})^{2}}{2}\right)\mathrm{SM}(\mathbf{x},\mathbf{y}) 
= \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{Ax}+(\mathbf{A}^{\top})^{-1}\mathbf{y})]
\end{equation}
Thus for 
$\Psi^{m}_{\mathbf{M}}(\mathbf{u}) \overset{\mathrm{def}}{=}\frac{1}{\sqrt{m}}\mathrm{exp}(-\frac{(\mathbf{Mu})^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{Mu}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Mu}))^{\top}$ and $\omega_{i} \sim \mathcal{N}(0,\mathbf{I}_{d})$:
\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{\top})^{-1}}(\mathbf{y})].
\vspace{-2mm}
\end{equation}

We obtain the new random feature map mechanism providing unbiased estimation of the softmax kernel. In general it is \textit{asymmetric} since it applies different parameterization for $\mathbf{x}$ and $\mathbf{y}$, i.e. one using $\mathbf{A}$, the other one ($\mathbf{A}^{\top})^{-1}$.
Asymmetric random features is a simple generalization of the model using the same $\phi$ for both $\mathbf{x}$ and $\mathbf{y}$, presented earlier.
The resulting estimators $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y})$,
that we call \textit{complex exponential} (CE) will serve as base estimators, and are defined as:
\begin{equation}
\vspace{-3mm}
\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y}) \overset{\mathrm{def}}{=} \Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{\top})^{-1}}(\mathbf{y})    
%\vspace{-2.0mm}
\end{equation}
For $\mathbf{A} = \mathbf{i}\mathbf{I}_{d}$, CE-estimator becomes trigonometric and for $\mathbf{A} = \mathbf{I}_{d}$, it becomes
$\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}(\mathbf{x},\mathbf{y})$.
Note also that an estimator based on this mechanism has variance equal to zero if
\begin{equation}
\label{imp_rel}
\mathbf{x} = -(\mathbf{A}^{-1})(\mathbf{A}^{\top})^{-1}\mathbf{y}.    
\end{equation}
In fact we can relax that condition. It is easy to check that for the variance to be zero, we only need:
\begin{equation}
\mathrm{Re}(\mathbf{A})\mathbf{x} + \mathrm{Re}((\mathbf{A}^{T})^{-1})\mathbf{y}=0 \textrm{ and }  
\mathrm{Im}(\mathbf{A})\mathbf{x} + \mathrm{Im}((\mathbf{A}^{T})^{-1})\mathbf{y}=0
\end{equation}

\subsection{Adapting HRF estimators: how to instantiate hybrid random features}
\label{sec:instantiations}

We will use complex exponential estimators from Section \ref{sec:complex_estimators} as base estimators in different insantiations of HRF estimators (that by definition admit random feature map decomposition).
The key to the linearization of the HRF estimators is then Equation \ref{lambda-eq} which implies linearization of the shifted versions of $\lambda$-coefficients 
(Equation \ref{lambda-eq-estimate}) and consequently - desired random feature map decomposition via the mechanism of compositional kernels (details in the Appendix). The questions remains how to construct $\lambda$-coefficients to reduce variance of the estimation in the desired regions of interest.

\paragraph{Accurate approximation of small and large softmax kernel values simultaneously:} As we explained earlier, in several applications of softmax estimators a desired property is to provide accurate estimation in two antipodal regions - small and large softmax kernel values.
This can be done in particular by choosing $p=1$, $\widehat{\mathrm{SM}}^{1}=\widehat{\mathrm{SM}}^{++}$, $\widehat{\mathrm{SM}}^{2}=\widehat{\mathrm{SM}}^{\mathrm{trig}}$ and 
$\lambda(\mathbf{x},\mathbf{y}) = \frac{\theta_{\mathbf{x},\mathbf{y}}}{\pi}$, where $\theta_{\mathbf{x},\mathbf{y}}$ stands for an angle between $\mathbf{x}$ and $\mathbf{y}$. The key observation is that $\lambda(\mathbf{x},\mathbf{y})$ can be unbiasedly approximated via the mechanism of $\mathrm{sgn}$ random features (following from Goemans-Willimson algorithm \citep{goemans}) as follows (details in the Appendix, Sec. \ref{sec:app_angular_hybrid}):
\begin{equation}
\widehat{\lambda}(\mathbf{x},\mathbf{y}) = 
\frac{1}{2} + \rho_{n}(\mathbf{x})^{\top}\rho_{n}(\mathbf{y}),
\end{equation}
where $\rho_{1,n}(\mathbf{z})=\rho_{2,n}(\mathbf{z})=\rho_{n}(\mathbf{z}) \overset{\mathrm{def}}{=}\frac{\mathbf{i}}{\sqrt{2n}}(\mathrm{sgn}(\tau_{1}^{\top}\mathbf{z}),...,\mathrm{sgn}(\tau_{n}^{\top}\mathbf{z}))^{\top}$ for $\tau_{1},...,\tau_{n} \sim \mathcal{N}(0,\mathbf{I}_{d})$ and $\mathbf{i}^{2}=-1$.
We call the resulting estimator of the softmax kernel \textit{angular hybrid}.
As we show in Sec. \ref{sec:theoretical_res}, this estimator is indeed particularly accurate in approximating both small and large softmax kernel values. For instance, for the prominent case when input vectors are of fixed length, its variance is zero for both the smallest ($\theta_{\mathbf{x},\mathbf{y}}=\pi$) and largest ($\theta_{\mathbf{x},\mathbf{y}}=0$) softmax kernel values (see: Fig. \ref{fig:3dplots}).
\paragraph{Gaussian Lambda Coefficients:}
Another tempting option is to instantiate $\lambda$-coefficients with approximate Gaussian kernel values (estimated either via positive or trigonometric random features). In that setting, functions $\alamgen$ are defined as
$
\alamgen = \exp(-\frac{\|\mathbf{x}+\mathbf{M}_{k}\mathbf{y}\|_{2}^{2}}{2c_{k}^{2}}),    
$
for some $\mathbf{M}_{1},...,\mathbf{M}_{p} \in \mathbb{R}^{d \times d}$ and $c_{1},...,c_{p} \in \mathbb{R}$. Since this time $\lambda$-coefficients are the values of the Gaussian kernel between vectors $\frac{\mathbf{x}}{c_{k}}$ and $-\frac{\mathbf{M}_{k}\mathbf{y}}{c_{k}}$, we can take $a_{k}=0$ and define $\rho_{1,\cdot}^{k}$,$\rho_{2,\cdot}^{k}$ as:
\begin{equation}
\rho_{1,\cdot}^{k}(\mathbf{x}) = \exp(-\frac{\|\mathbf{x}\|_{2}^{2}}{2c_{k}^{2}})\phi^{\mathrm{SM}}(\frac{\mathbf{x}}{c_{k}}) \textrm{ and }    
\rho_{2,\cdot}^{k}(\mathbf{y}) = \exp(-\frac{\|\mathbf{M}_{k}\mathbf{y}\|_{2}^{2}}{2c_{k}^{2}})\phi^{\mathrm{SM}}(-\frac{\mathbf{M}_{k}\mathbf{y}}{c_{k}}), 
\end{equation}
where $\phi^{\mathrm{SM}}$ is the random feature map corresponding to a particular estimator of the softmax kernel.
Note that the resulting hybrid estimator, that we call \textit{Gaussian hybrid} has nice pseudo-combinatorial properties. The coefficients $\lambda^{k} \in (0,1]$ fire if $\mathbf{x} \approx -\mathbf{M}_{k}\mathbf{y}$ (the firing window can be accurately controlled via hyperparameters $c_{k}$). Thus matrices $\mathbf{M}_{k}$ can be coupled with the base estimators particularly accurate in the regions, where $\mathbf{x} \approx -\mathbf{M}_{k}\mathbf{y}$. The mechanism can be thus trivially applied to the setting of accurate approximation of both small and large softmax kernel values for inputs of fixed length, yet it turns out to be characterized by the larger variance than its angular hybrid counterpart and cannot provide variance vanishing property for both $\theta_{\mathbf{x},\mathbf{y}}=0$ and $\theta_{\mathbf{x},\mathbf{y}}=\pi$.


\paragraph{Adaptation to data admitting clustering structure:}
Assume now that the inputs $\mathbf{x}$ come from a distribution $\mathcal{P}(X)$ admitting certain clustering structure with clusters $X_{1},...,X_{u} \subseteq \mathbb{R}^{d}$ of centers $\mathbf{x}_{1},...,\mathbf{x}_{u} \in \mathbb{R}^{d}$ and that the analogous fact is true for $\mathbf{y}$ with the corresponding clusters $Y_{1},...,Y_{w} \subseteq \mathbb{R}^{d}$ and centers $\mathbf{y}_{1},...,\mathbf{y}_{w} \in \mathbb{R}^{d}$.
For a fixed pair of clusters' centers $(\mathbf{x}_{i},\mathbf{y}_{j})$, one can associate a complex exponential estimator $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{(\mathbf{x}_{i},\mathbf{y}_{j})}$ with the corresponding matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$ (see: Sec. \ref{sec:complex_estimators}) that minimizes the following loss, where $|\mathbf{z}|$ for $\mathbf{z} \in \mathbb{C}^{d}$ is defined as
$|\mathbf{z}| = \sqrt{\sum_{i=1}^{d}|z_{i}|^{2}}$:
\begin{equation}
%\label{eq:cl-loss}
l(\mathbf{A}) = |\mathbf{A} \mathbf{x}_{i} + (\mathbf{A}^{\top})^{-1}\mathbf{y}_{j}|^{2}   \label{cluster la equation}
\end{equation}  
Note that, by Equation \ref{imp_rel}, if one can find $\mathbf{A}$ such that $l(\mathbf{A})=0$, then $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{(\mathbf{x}_{i},\mathbf{y}_{j})}$ makes no error in approximating softmax kernel value on the centers $\mathbf{x}_{i}, \mathbf{y}_{j}$. Furthermore, if sampled points are close to the centers and $l(\mathbf{A})$ is small, the corresponding variance of the estimator will also be small. Thus one can think about $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{(\mathbf{x}_{i},\mathbf{y}_{j})}$ as an estimator adapted to a pair of clusters $(\mathbf{x}_{i},\mathbf{y}_{j})$. We can add additional constraints regarding $\mathbf{A}$, i.e. $\mathbf{A} \in \mathbb{R}^{d \times d}$ or $\mathbf{A}$ being diagonal (or both) for closed-form formulae of the optimal $\mathbf{A}$, yet not necessarily zeroing out $l(\mathbf{A})$ (details in the Appendix, Sec. \ref{sec:app_clustering}). 
Complex exponential estimators defined in this way can be combined together, becoming base estimators in the HRF estimator. The corresponding $\lambda$-coefficients can be chosen to be Gaussian as described in the previous paragraph (with optimized matrices $\mathbf{M}_{k}$ so that a coefficient fires for the corresponding pair of clusters' centers), but there is another much simpler choice of $\lambda$s. We index different base estimators by pairs of clusters' centers $(\mathbf{x}_{i},\mathbf{y}_{j})$. One can simply take $\rho^{(\mathbf{x}_{i},\mathbf{y}_{j})}_{1}(\mathbf{x})=1$ if $\mathbf{x}$ belongs to the cluster of center $\mathbf{x}_{i}$ and 
$\rho^{(\mathbf{x}_{i},\mathbf{y}_{j})}_{1}(\mathbf{x})=0$ otherwise. Vectors
$\rho_{2}^{(\mathbf{x}_{i},\mathbf{y}_{j})}(\mathbf{y})$ (that also become scalars in this scenario) are defined analogously (the $n$ symbol vanishes since $\rho$ is deterministic). Thus effectively the hybrid estimator activates precisely this random feature mechanism that is optimal for the particular pair of clusters. This scheme is feasible if cluster-membership calculation is computationally acceptable, otherwise aforementioned Gaussian coefficients can be applied.

\vspace{-1mm}
We conclude with an observation that in principle (to reduce the number of base estimators if needed) one can also construct HRF estimators that take base estimators defined in the above way only for the most massive pairs of clusters and add an additional default base estimators (for instance $\widehat{\mathrm{SM}}^{++}$).

\begin{figure} 
\centering
\includegraphics[width=.98\textwidth]{img/mseplots.pdf}  
\caption{\small{MSEs for three softmax kernel estimators (from left to right): $\widehat{\mathrm{SM}}^{\mathrm{trig}}$, $\widehat{\mathrm{SM}}^{\mathrm{++}}$ and angular hybrid  for $m=10, n=1$ and input of lenghts $r=5$. MSEs are given as functions of: an angle $\theta_{\mathbf{x},\mathbf{y}} \in [0, \pi]$ between $\mathbf{x}$ and $\mathbf{y}$ and $r$ (symmetrized along $0$ for length axis) . For each plot, we marked in grey its slice for a fixed $r$ to illustrate that only for the angular hybrid estimator, the MSE goes to zero for both $\theta_{\mathbf{x},\mathbf{y}} \rightarrow 0$ and $\theta_{\mathbf{x},\mathbf{y}} \rightarrow \pi$.}}
\label{fig:3dplots}
\vspace{-2mm}
\end{figure}



\section{Theoretical guarantees}
\label{sec:theoretical_res}
\vspace{-2mm}

We provide here theoretical guarantees regarding HRF estimators. We focus on the bipolar setting with two base estimators: $\widehat{\mathrm{SM}}^{\mathrm{trig}}$ and $\widehat{\mathrm{SM}}^{++}$. The following is true:

\begin{theorem}[MSE of the bipolar hybrid estimator]
\label{general-hybrid}
Take the bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y})$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y})$ is constructed independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$). Then the following holds:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m, n}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}_{n}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{equation}
Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator is further reduced, namely we have:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m, n}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}_{n}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}))]
\end{split}
\end{align}

\vspace{-4mm}

The exact formula on $\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y}))$ and $\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))$ is given in Lemma \ref{mse-lemma}.
\end{theorem}

We can apply this result directly to the angular hybrid estimator, since:

\begin{lemma}
\label{theta-lemma}
For the angular hybrid estimator the following holds:
\begin{align}
\begin{split}    
\mathbb{E}[\widehat{\lambda}_{n}^{2}(\mathbf{x},\mathbf{y})] = \frac{\theta_{\mathbf{x},\mathbf{y}}}{\pi}\left(\frac{\theta_{\mathbf{x},\mathbf{y}}}{\pi}-\frac{\theta_{\mathbf{x},\mathbf{y}}}{n\pi}+\frac{1}{n}\right),
\mathbb{E}[\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y})] = \frac{\theta_{\mathbf{x},\mathbf{y}}}{\pi}.
\end{split}
\end{align}
\end{lemma}

\vspace{-3mm}

We see that, as mentioned before, the variance of the angular hybrid estimator is zero for both $\theta_{\mathbf{x},\mathbf{y}}=0$ and $\theta_{\mathbf{x},\mathbf{y}}=\pi$ if inputs $\mathbf{x},\mathbf{y}$ have the same length.
We need one more definition.

\begin{definition}
Assume that the inputs to the estimators are taken from some given bounded set $\mathcal{C} \subseteq \mathbb{R}^{d}$. For a given estimator $\widehat{\mathrm{SM}}$ on feature vectors $\mathbf{x},\mathbf{y} \in \mathcal{C}$, we define its max-relative-error with respect to $\mathcal{C}$ as
$
\epsilon_{\mathcal{C}}(\widehat{\mathrm{SM}}) = \max_{\mathbf{x},\mathbf{y} \in \mathcal{C}} \eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}}), \textrm{where }
\eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}})=\frac{\sqrt{\mathrm{MSE}(\widehat{\mathrm{SM}}(\mathbf{x},\mathbf{y}))}}{\mathrm{SM}(\mathbf{x},\mathbf{y})}.
$
Denote by $S(r)$ a sphere centered at $0$ and of radius r. Define $\eps_{\theta, r}(\widehat{\mathrm{SM}})\overset{\mathrm{def}}{=}\eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}})$ for $\mathbf{x},\mathbf{y} \in S(r)$ and such that $\theta=\theta_{\mathbf{x},\mathbf{y}}$ (note that the mean squared errors of the considered estimators depend only on the angle $\theta_{\mathbf{x},\mathbf{y}}$ for $\mathbf{x},\mathbf{y}$ chosen from a fixed sphere).
\end{definition}

This definition captures the critical observation that in several applications of the softmax kernel estimation, e.g. efficient softmax sampling or linear-attention Transformers \citep{performers}, small relative errors are a much more meaningful measure of the quality of the method than small absolute errors.
It also enables us to find hidden symmetries between different estimators:
\begin{lemma}
\label{tri-exp-imp-lemma}
The following holds:
\begin{align}
\begin{split}
\label{mm-1}
\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}})=\epsilon_{\pi-\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}})=\frac{1}{\sqrt{2m}}\exp(2r^{2}\sin^{2}(\frac{\theta}{2}))\left(1-\exp(-4r^{2}\sin^{2}(\frac{\theta}{2}))\right),
\end{split}
\end{align} and consequently for $W(r)=\exp(2r^{2})\left(1-\exp(-4r^{2})\right)$:
\begin{equation}
\label{mm-2}
\epsilon_{S(r)}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}) = 
\epsilon_{S(r)}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}) = \lim_{\theta \rightarrow \pi} \epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}) = 
\lim_{\theta \rightarrow 0} \epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}) =
\sqrt{\frac{1}{2m}}W(r)
\end{equation}
\end{lemma}
\vspace{-3mm}
Our main result shows that HRF estimators can be applied to reduce the max-relative-error of the previously applied estimators of the softmax kernel.
In the next theorem we show that the max-relative-error of the angular hybrid estimator scales as
$\frac{1}{r}\exp(2r^{2})$ in the length $r$ of its inputs as opposed to $\exp(2r^{2})$ as it is the case for $\widehat{\mathrm{SM}}^{\mathrm{trig}}$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}$ (see: Lemma \ref{tri-exp-imp-lemma}). Furthermore, the max-relative-error scales as $\sqrt{\theta}$ and $\sqrt{\pi-\theta}$ as $\theta \rightarrow 0$ and $\theta \rightarrow \pi$ respectively, in particular goes to $0$ in both critical cases. This is not true for $\widehat{\mathrm{SM}}^{\mathrm{trig}}$ nor for 
$\widehat{\mathrm{SM}}^{\mathrm{++}}$.

\begin{theorem}
\label{maxerror_theorem}
The max-relative-error of the angular hybrid estimator for the inputs $\mathbf{x},\mathbf{y}$ on the sphere $S(r)$ of radius $r \geq 1$ satisfies for $W(r)=\exp(2r^{2})
\left(1-\exp(-4r^{2})\right)$:
\begin{equation}
\label{hybang_upper}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{anghyb}}) \leq \frac{1}{r}\sqrt{\frac{1}{2m}}W(r)\sqrt{\frac{1}{\pi} - \frac{1}{n \pi} + \frac{1}{n\sqrt{\pi}}}  
\end{equation}
Furthermore,
$
\lim_{\theta \rightarrow 0} \frac{\eps_{\theta, r}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{anghyb}})}{\sqrt{\theta}}= 
\lim_{\theta \rightarrow \pi} \frac{\eps_{\theta, r}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{anghyb}})}{\sqrt{\theta-\pi}} = \sqrt{\frac{1}{2\pi mn}}W(r).
$
\end{theorem}

Additional implications of Theorem \ref{maxerror_theorem}, using the fact that $\Theta(mn)$-dimensional HRFs can be constructed in time $O(nd+md+mn)$ (regular RFs need $O(mnd)$), are in the Appendix (Sec. \ref{sec:app_discussion}).


==> Hybrid Estimators (Camera-ready, Arxiv)/theory.tex <==
\section{Robust Estimation of Softmax and Gaussian Kernels}
\label{sec:theory}

\subsection{Preliminaries}
\label{sec: prel}

In this work we focus on the following kernel functions:

\begin{definition}[Softmax and Gaussian kernel]
For $\mathbf{x},\mathbf{y} \in \mathbb{R}^{d}$, the softmax ($\mathrm{SM}$) and Gaussian kernels are defined as follows:
\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y})\overset{\mathrm{def}}{=}\exp(\mathbf{x}^{\top}\mathbf{y}), \qquad \mathrm{K}_{\mathrm{gauss}} \overset{\mathrm{def}}{=}\exp(-\frac{\|\mathbf{x}-\mathbf{y}\|_{2}^{2}}{2}).
\end{equation}
\end{definition}

We will approximate these kernels with estimators leveraging random feature map representations.

\begin{definition}[Kernel with a Random Feature Map Representation]
We say that a kernel function $\mathrm{K}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ \textit{admits a random feature map representation} if it can be written as:
\begin{equation}
\mathrm{K}(\mathbf{x},\mathbf{y}) = \mathbb{E}_{\omega \sim \Omega}\left[\sum_{i=1}^{l} \xi_{i}(\mathbf{x},\omega)\xi_{i}(\mathbf{y},\omega)\right]  ,  
\end{equation}
for some $\xi_{i}: \mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, and where $\omega$ is sampled from some probabilistic distribution $\Omega \in \mathcal{P}(\mathbb{R}^{d})$.
The corresponding regular random feature map, for a given $m \in \mathbb{N}$, is defined as:
\begin{equation}
\label{random_feature_map_formula}
\phi^{\mathrm{iid}}_{m}(\mathbf{u}) = \frac{1}{\sqrt{m}} \phi_{m}^{1}(\mathbf{u}) \star ... \star \phi_{m}^{l}(\mathbf{u}) \in \mathbb{R}^{ml},  
\end{equation}
where $\phi_{m}^{i} = (\xi_{i}(\mathbf{u},\omega_{1}),...,\xi_{i}(\mathbf{u},\omega_{m}))^{\top}$ for $i=1,...,l$, the symbol $\star$ stands for vertical concatenation, and %furthermore 
$\omega_{1},...,\omega_{m} \overset{\mathrm{iid}}{\sim} \Omega$.
\end{definition}
It is not hard to see that regular feature maps can be used to unbiasedly approximate corresponding kernels, leading to estimators of the form: 
\begin{equation}
\widehat{\mathrm{K}}^{\mathrm{iid}}(\mathbf{x},\mathbf{y}) = \phi^{\mathrm{iid}}_{m}(\mathbf{x})^{\top}
\phi^{\mathrm{iid}}_{m}(\mathbf{y}).    
\end{equation}

If $\Omega$ is isotropic, there exists another procedure for constructing random feature maps that still leads to the unbiased estimator, yet often implies better concentration results. In that procedure $\omega_{1},...,\omega_{m}$ are sampled in such a way that $\omega_{i} \sim \Omega$ still holds for $i=1,...,m$, however this time different $\omega_{i}$ are constrained to be exactly orthogonal, i.e. $\omega_{i}^{\top}\omega_{j}=0$ for $i \neq j$ (with probability $1$, not only on expectation). See: \citep{unrea} for straightforward explicit constructions of such ensembles.
We call feature maps $\phi^{\mathrm{ort}}_{m}$ obtained in such a way, \textit{orthogonal random feature maps}. Of course for the above construction we assume that $m \leq d$ (there exist extensions of the above mechanism for $m > d$, where vectors $\omega$ are partitioned into independently choden blocks such that vectors within a block are orthogonal).

\textbf{Note:} It was shown in \citep{geometry} that orthogonal random features asymptotically for large enough $d$ lower the variance of the estimation, yet this result cannot be extended to any $d$. The analysis breaks for arbitrary $d$ because produced random features can be of arbitrary signs.

It is a well known fact (\cite{fourierapprox}) that Gaussian kernel admits random feature map representation utilizing trigonometric functions, namely: $l=2$, $\Omega=\mathcal{N}(0,\mathbf{I}_{d})$ (see: Eq. \ref{random_feature_map_formula}) and:
\begin{equation}
\xi_{1}(\mathbf{u},\omega) = \sin(\omega^{\top}\mathbf{u}), \textrm{ } \xi_{2}(\mathbf{u}, \omega) = \cos(\omega^{\top}\mathbf{u}).    
\end{equation}

This decomposition directly leads to the random feature map mechanism for the softmax kernel with:
\begin{equation}
\label{trig-features}
\xi_{1}(\mathbf{u},\omega) = \exp(\frac{\|\mathbf{u}\|^{2}}{2})\sin(\omega^{\top}\mathbf{u}), \textrm{ }     
\xi_{2}(\mathbf{u},\omega) = \exp(\frac{\|\mathbf{u}\|^{2}}{2})\cos(\omega^{\top}\mathbf{u}),
\end{equation}
since:
\begin{equation}
\label{gaussian_to_softmax}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \exp(\frac{\|\mathbf{x}\|^{2}}{2})\mathrm{K}_{\mathrm{gauss}}(\mathbf{x},\mathbf{y})\exp(\frac{\|\mathbf{y}\|^{2}}{2}). 
\end{equation}

\subsection{Positive Random Features}

The above mechanism produces random features that in principle can be negative even though values of kernels under consideration are strictly positive. This is not a problem if approximated kernel values are bounded away from $0$ since introduced estimators are unbiased.
However if very small kernel values are involved, the quality of the approximation deteriorates and using the mechanism is even more problematic if those kernel values appear in denominators of more complex expressions (for instance in renormalization procedures as in standard softmax mechanism producing discrete probabilistic distributions). 

In response, a new random feature map mechanism for unbiasedly approximating softmax kernels and thus consequently, also Gaussian kernels was introduced in \citep{performers}. This mechanism can be further integrated with the orthogonal random feature techniques described above, to provide more accurate, still unbiased mechanism, with provably lower estimation variance for any $d>0$, as we later show.
\begin{lemma}[Positive Random Features]
\label{pos_random_features_lemma}
For $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$, the following is true:
\begin{equation}
\label{main_eq}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = 
\mathbb{E}_{\omega \sim \mathcal{N}(0,\mathbf{I}_{d})}\left[\mathrm{exp}(\omega^{\top}\mathbf{x} - \frac{\|\mathbf{x}\|^{2}}{2})\mathrm{exp}(\omega^{\top}\mathbf{y}-\frac{\|\mathbf{y}\|^{2}}{2})\right]=\\
\Lambda \mathbb{E}_{\omega \sim \mathcal{N}(0,\mathbf{I}_{d})}\cosh(\omega^{\top}\mathbf{z})
\end{equation}
for $\mathbf{z}=\mathbf{x}+\mathbf{y}$ and $\Lambda = \exp(-\frac{\|\mathbf{x}\|^{2}+\|\mathbf{y}\|^{2}}{2})$.
Consequently, softmax kernel admits a positive random feature map decomposition with $l=1$ and $\xi_{1}(\mathbf{u}, \omega) = \mathrm{exp}(\omega^{\top}\mathbf{u} - \frac{\|\mathbf{u}\|^{2}}{2})$, (and by Eq. \ref{gaussian_to_softmax} so does Gaussian kernel with $l=1$ and 
$\xi_{1}(\mathbf{u}, \omega)=
\mathrm{exp}(\omega^{\top}\mathbf{u} - \|\mathbf{u}\|^{2})$).
Furthermore, softmax kernel admits also a hyperbolic random feature map decomposition (leveraging the formula for hyperbolic cosine) with $l=2$ and: $\xi_{1}(\mathbf{u},\omega)=\frac{1}{\sqrt{2}}\exp(\omega^{\top}\mathbf{u}-\frac{\|\mathbf{u}\|^{2}}{2})$, $\xi_{2}(\mathbf{u},\omega)=\frac{1}{\sqrt{2}}\exp(-\omega^{\top}\mathbf{u}-\frac{\|\mathbf{u}\|^{2}}{2})$.

\end{lemma}





\subsection{Positive versus Trigonometric Random Features}

The following is true:

\begin{lemma}[positive versus trigonometric random features]
\label{mse-lemma}
Denote by $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})$ an estimator of the value $\mathrm{SM}(\mathbf{x}, \mathbf{y})$ of the softmax kernel
in points $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$ using trigonometric mechanism from Equation \ref{trig-features} and independent random projections $\omega_{1}^{\mathrm{iid}}, ..., \omega_{m}^{\mathrm{iid}}$. Denote by $\widehat{\mathrm{SM}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})$ its analogue using independent positive random features from Lemma \ref{pos_random_features_lemma} with $l=1$ and by $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})$ the one with $l=2$. The mean squared errors ($\mathrm{MSE}$s) of these estimators are given by:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})) =
\frac{1}{2m} \exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})
(1-\mathrm{exp}(-\|\Delta\|^{2}))^{2}, \\ 
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2})),\\
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{2m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2}))^{2},
\end{split}
\end{align}
where $\Delta = \mathbf{x} - \mathbf{y}$ and $\mathbf{z} = \mathbf{x} + \mathbf{y}$.
\end{lemma}

From now on we will focus on $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$.
An interesting special case to analyze is for $\|\mathbf{x}\|=\|\mathbf{y}\|=r$. Denote by $\theta \in [0, \pi]$ and angle between $\mathbf{x}$ and $\mathbf{y}$. The following is a direct implication of Lemma \ref{mse-lemma}.

\begin{lemma}
\label{normalized_input_lemma}
The following is true for $\|\mathbf{x}\|=\|\mathbf{y}\|=r$ with an angle $\theta \in [0, \pi]$ between them:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{2m}\exp(2r^{2})(1-\exp(-4r^{2}\sin^{2}(\frac{\theta}{2})))^{2}\\ 
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{2m}\exp(8r^{2}\cos^{2}(\frac{\theta}{2})-2r^{2})
(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2})))^{2}
\end{split}
\end{align}
\end{lemma}

\subsection{Positive \& Trigonometric Random Features as Special Cases of the complex Exponential Estimator}

We present below the unification angle of the techniques presented above, showing that these are just two special instantiations of the more general mechanism.

We start with the following lemma which is a simple consequence of the theory of complex functions, yet also a gateway to the aforementioned unification:

\begin{lemma}
\label{complex}
Let $\omega \sim \mathcal{N}(0,\mathbf{I}_{d})$. Then for every $\mathbf{z} \in \mathbb{C}^{d}$ the following holds:
\begin{equation}
\mathbb{E}[\exp(\omega^{\top}\mathbf{z})] = \exp(\frac{\mathbf{z}^{2}}{2}),    
\end{equation}
where $\mathbf{z}^{2} \overset{\mathrm{def}}{=}  z_{1}^{2} + ... + z_{d}^{2}$.
\end{lemma}
\begin{proof}
From the independence of $\omega_{1},...,\omega_{d}$ we get:
\begin{equation}
\mathbb{E}[\exp(\omega^{\top}\mathbf{z})] = \prod_{i=1}^{d} \mathbb{E}[\mathrm{exp}(\omega_{i}z_{i})]    
\end{equation}
Thus it suffices to show that for $g \sim \mathcal{N}(0,1)$ and any $z \in \mathbb{C}$ the following holds:
\begin{equation}
\mathbb{E}[\mathrm{exp}(gz)] = \mathrm{exp}(\frac{z^{2}}{2})    
\end{equation}
Define $f(z) = \mathbb{E}[\mathrm{exp}(gz)]$. 
Note that $f(z) = \mathrm{exp}(\frac{z^{2}}{2})$ for $z = \mathbf{i}x$, where $\mathbf{i}^{2}=-1$ and $x \in \mathbb{R}$ which follows from the formulae of the characteristic function of the gaussian distribution. Similarly, $f(z) = \mathrm{exp}(\frac{z^{2}}{2})$ for $z \in \mathbb{R}$ which follows from the formulae of the moment generating function of the gaussian distribution.
We now use the fact from complex analysis that if two analytic functions $\mathbb{C} \rightarrow \mathbb{C}$ are identical on uncountably many points then they are equal on $\mathbb{C}$ to complete the proof (we leave to the reader checking that both $f(z)$ and $g(z)\overset{\mathrm{def}}{=}\mathrm{exp}(\frac{z^{2}}{2})$ are analytic).
\end{proof}

Take: $\mathbf{z} = \mathbf{i}(\mathbf{x}-\mathbf{y})$. Using Lemma \ref{complex}, we get:
\begin{equation} \label{exp - norm cos}
\mathrm{exp}(-\frac{\|\mathbf{x}-\mathbf{y}\|^{2}}{2}) = \mathbb{E}[\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))],   
\end{equation}
which leads to the trigonometric estimator.
Now take: $\mathbf{z} = \mathbf{x} + \mathbf{y}$.
Using Lemma \ref{complex}, we get:
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{x}+\mathbf{y}\|^{2}}{2}) = \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{x}+\mathbf{y}))],    
\end{equation}
which implies the estimator based on positive random features (nonhyperbolic one). 

Finally, consider $\mathbf{z} = \mathbf{Ax} + \mathbf{(A^{\top})^{-1}y}$ for an invertible (in $\mathbb{C}^{d \times d})$ matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$. Using Lemma \ref{complex}, we get this time:
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{Ax}\|^{2}}{2})  
\mathrm{exp}(\frac{\|(\mathbf{A}^{\top})^{-1}\mathbf{y}\|^{2}}{2})\mathrm{SM}(\mathbf{x},\mathbf{y}) 
= \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{Ax}+(\mathbf{A}^{\top})^{-1}\mathbf{y})]
\end{equation}
Thus for 
$\Psi^{m}_{\mathbf{M}}(\mathbf{z}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{Mz}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{Mz}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Mz}))^{\top}$ and $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$:
\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{\top})^{-1}}(\mathbf{y})]
\end{equation}

Therefore we have a new random feature map mechanism leading to an estimator unbiasedly approximating softmax kernel. In general it is asymmetric (different parameterization for $\mathbf{x}$ and $\mathbf{y}$; one uses $\mathbf{A}$, the other one $\mathbf{A}^{-1}$).
We call an estimator $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y})$ defined as:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y}) \overset{\mathrm{def}}{=} \Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{\top})^{-1}}(\mathbf{y})    
\end{equation}
a \textit{complex exponential} estimator of the softmax kernel.

Note that if we take $\mathbf{A} \overset{\mathrm{def}}{=} \mathbf{i}\mathbf{I}_{d}$ then $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y})$ becomes $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}(\mathbf{x},\mathbf{y})$ and if we take $\mathbf{A} \overset{\mathrm{def}}{=} \mathbf{I}_{d}$ then
$\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y})$ becomes $\widehat{\mathrm{SM}}_{m}^{\mathrm{+}}(\mathbf{x},\mathbf{y})$.

Note also that an estimator based on this mechanism has variance equal to $0$ if:
\begin{equation}
\mathbf{x} = -(\mathbf{A}^{-1})(\mathbf{A}^{\top})^{-1}\mathbf{y}    
\end{equation}
In fact we can relax the above condition. It is easy to check that for the variance to zero out, we only need:
\begin{equation}
\left\{ \begin{array}{rcl}
\mathrm{Re}(\mathbf{A})\mathbf{x} + \mathrm{Re}((\mathbf{A}^{T})^{-1})\mathbf{y}=0 \\ 
\mathrm{Im}(\mathbf{A})\mathbf{x} + \mathrm{Im}((\mathbf{A}^{T})^{-1})\mathbf{y}=0
\end{array}\right.
\end{equation}



\subsection{Hybrid Random Features for the Softmax Kernel}
\label{hybrid}

Denote by $\mathcal{E}=( \asm )_{k=1}^{p+1}$ a list of estimators of $\sm$ (the so-called \textit{base estimators}) and by $\Lambda = ( \alamgen )_{k=1}^{p}$ a list of estimators of: 
$\{\lambda^{k}(\mathbf{x},\mathbf{y})\}_{k=1}^{p}$ for some functions
$\lambda^{k}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, constructed independently from $\mathcal{E}$.
Take the following estimator of $\sm$:
\begin{equation}
\label{gen-hyb-eque}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{k=1}^{p} \alamgen \asm + \left(1-\sum_{k=1}^{p} \alamgen \right)\widehat{\mathrm{SM}}^{p+1}(\mathbf{x},\mathbf{y})
\end{equation}
We call $\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y})$ a \textit{general hybrid estimator} of $\sm$ parameterized by $\mathcal{E},\Lambda$. Note that if elements of $\mathcal{E}$ are unbiased estimators of $\sm$, then trivially $\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y})$ is also an unbiased estimator of $\sm$. Assume that each $\asm$ is of the form:
\begin{equation}
\asm = (\phi_{m}^{k}(\mathbf{x}))^{\top}\phi_{m}^{k}(\mathbf{y})    
\end{equation}
for $\phi_{m}^{k}(\mathbf{z}) = \frac{1}{\sqrt{m}} 
\phi_{m}^{1,k}(\mathbf{z}) \star ... \star \phi_{m}^{t_{k},k}(\mathbf{z})$ and some: $t_{k}>0$ and $\phi_{m}^{1,k},..., \phi_{m}^{t_{k},k}:\mathbb{R}^{d} \rightarrow \mathbb{R}^{m}$. Assume also that $\lambda^{k}(\mathbf{x},\mathbf{y})$ can be written as:
\begin{equation}
\label{lambda-eq}
\lambda^{k}(\mathbf{x},\mathbf{y}) = a_{k} + \mathbb{E}_{\tau \sim \Lambda}[\sum_{i=1}^{l_{\lambda_{k}}}\xi^{i}_{\lambda_{k}}(\mathbf{x},\tau)\xi^{i}_{\lambda_{k}}(\mathbf{y}, \tau)]  
\end{equation}
for some scalars $a_{k} \in \mathbb{R}$, distribution $\Lambda \in \mathcal{P}(\mathbb{R}^{d})$ and mappings $\xi^{i,k}_{\lambda}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ and that the corresponding estimator $\widehat{\lambda}^{k}(\mathbf{x},\mathbf{y})=\widehat{\lambda}^{k}_{n}(\mathbf{x},\mathbf{y})$ is of the form:
\begin{equation}
\label{lambda-eq-estimate}
\widehat{\lambda}^{k}_{n}(\mathbf{x},\mathbf{y}) = a_{k} + (\phi_{n}^{\lambda_{k}}(\mathbf{x}))^{\top}    
\phi_{n}^{\lambda_{k}}(\mathbf{y})
\end{equation}
for 
\begin{equation}
\phi_{n}^{\lambda_{k}}(\mathbf{x}) =  \frac{1}{\sqrt{n}}\phi_{n}^{1,\lambda_{k}}(\mathbf{x}) \star ... \star \phi_{n}^{l_{\lambda_{k}},\lambda_{k}}(\mathbf{x})
\end{equation}
and $\phi_{n}^{i,\lambda_{k}}(\mathbf{x})=
(\xi^{i}_{\lambda_{k}}(\mathbf{x},\tau_{1}),...,\xi^{i}_{\lambda_{k}}(\mathbf{x},\tau_{n}))^{\top}$ for $\tau_{1},...,\tau_{n} \sim \Lambda$.
We then get:
\begin{align}
\begin{split}
\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y}) = \sum_{k=1}^{p}
\frac{a_{k}}{m}(\phi_{m}^{1,k}(\mathbf{x}) \star ... \star \phi_{m}^{t_{k},k}(\mathbf{x}))^{\top}(\phi_{m}^{1,k}(\mathbf{y}) \star ... \star \phi_{m}^{t_{k},k}(\mathbf{y})) + \\
\frac{1}{mn}\sum_{k=1}^{p}\sum_{i=1}^{l_{\lambda_{k}}}\sum_{j=1}^{t_{k}}
(\phi_{n}^{i,\lambda_{k}}(\mathbf{x}) \otimes \phi_{m}^{j,k}(\mathbf{x}))^{\top}(\phi_{n}^{i,\lambda_{k}}(\mathbf{y}) \otimes \phi_{m}^{j,k}(\mathbf{y}))+ \\
\frac{1-\sum_{k=1}^{p} a_{k}}{m}(\phi_{m}^{1,p+1}(\mathbf{x}) \star ... \star \phi_{m}^{t_{p+1},p+1}(\mathbf{x}))^{\top}(\phi_{m}^{1,p+1}(\mathbf{y}) \star ... \star \phi_{m}^{t_{p+1},p+1}(\mathbf{y})) - \\
\frac{1}{mn}\sum_{k=1}^{p}\sum_{i=1}^{l_{\lambda_{k}}}\sum_{j=1}^{t_{p+1}}
(\phi_{n}^{i,\lambda_{k}}(\mathbf{x}) \otimes \phi_{m}^{j,p+1}(\mathbf{x}))^{\top}(\phi_{n}^{i,\lambda_{k}}(\mathbf{y}) \otimes \phi_{m}^{j,p+1}(\mathbf{y})) = 
\Psi(\mathbf{x})^{\top}\Psi(\mathbf{y}),
\end{split}
\end{align}
where $\mathbf{u} \otimes \mathbf{v}$ stands for the vectorized outer-product of $\mathbf{u}$ and $\mathbf{v}$ and furthermore 
\begin{equation}
\label{hyb-all-1}
\Psi(\mathbf{z})=\Psi_{1}(\mathbf{z}) \star \Psi_{2}(\mathbf{z}) \star \Psi_{3}(\mathbf{z}) \star \Psi_{4}(\mathbf{z})
\end{equation}
for $\Psi_{1},\Psi_{2}, \Psi_{3}, \Psi_{4}$ defined as:

\begin{align}
\begin{split}
\label{hyb-all-2}
\Psi_{1}(\mathbf{z})=\prod_{k=1,...,p}^{\star} \sqrt{\frac{a_{k}}{m}}\phi_{m}^{1,k}(\mathbf{z})\star ... \star \phi_{m}^{t_{k},k}(\mathbf{z})\\
\Psi_{2}(\mathbf{z})=\frac{1}{\sqrt{mn}}\prod_{k=1,...,p}^{\star} \prod^{\star}_{i,j \in \{1,...,l_{\lambda_{k}}\}\times\{1,...,t_{k}\}} \phi_{n}^{i,\lambda_{k}}(\mathbf{z}) \otimes \phi_{m}^{j,k}(\mathbf{z})\\
\Psi_{3}(\mathbf{z})=\sqrt{\frac{1-\sum_{k=1}^{p} a_{k}}{m}}\phi_{m}^{1,p+1}(\mathbf{z})\star ... \star \phi_{m}^{t_{p+1},p+1}(\mathbf{z})\\
\Psi_{4}(\mathbf{z})=\frac{\mathbf{i}}{\sqrt{mn}}\prod_{k=1,...,p}^{\star} \prod^{\star}_{i,j \in \{1,...,l_{\lambda_{k}}\}\times\{1,...,t_{p+1}\}} \phi_{n}^{i,\lambda_{k}}(\mathbf{z}) \otimes \phi_{m}^{j,p+1}(\mathbf{z})\\
\end{split}    
\end{align}
Here $\prod^{*}$ stands for the concatenation operator and $\mathbf{i}^{2}=-1$. 
We conclude that $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ admits a random feature map representation.

\subsubsection{Scoring different general hybrid estimators}

To rank different hybrid estimators that we will consider later in the paper, we define softmax-kernel estimator's error in the following way. 

\begin{definition}
Assume that the inputs to the estimators are taken from some given bounded set $\mathcal{C} \subseteq \mathbb{R}^{d}$. For a given hybrid estimator $\widehat{\mathrm{SM}}$ on feature vectors $\mathbf{x},\mathbf{y} \in \mathcal{C}$, we define its max-relative-error with respect to $\mathcal{C}$ as:
\begin{equation}
\epsilon_{\mathcal{C}}(\widehat{\mathrm{SM}}) = \max_{\mathbf{x},\mathbf{y} \in \mathcal{C}} \eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}}), \textrm{where }
\eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}})=\frac{\sqrt{\mathrm{MSE}(\widehat{\mathrm{SM}}(\mathbf{x},\mathbf{y}))}}{\mathrm{SM}(\mathbf{x},\mathbf{y})}.
\end{equation}
\end{definition}

This definition captures the critical observation that in several applications of the softmax-kernel estimation, e.g. efficient softmax-sampling or linear-attention Transformers \citep{performer}, small relative errors are a much more meaningful measure of the quality of the method than small absolute errors.
As we will show below, it is also a gateway to find hidden symmetries between different estimators. 
Before providing specific instantiations of the class of general hybrid estimators given above and analyzing their corresponding error functions, we conduct such an analysis for the base estimators $\tri$ and $\expo$.

\begin{lemma}
\label{tri-exp-imp-lemma}
Denote by $S(r)$ a sphere centered at $0$ and of radius r. Let 
$\eps_{\theta, r}(\widehat{\mathrm{SM}})=\eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}})$ for $\mathbf{x},\mathbf{y} \in S(r)$ and such that $\theta=\theta_{\mathbf{x},\mathbf{y}}$ (note that the mean squared errors of the considered estimators depend only on the angle $\theta_{\mathbf{x},\mathbf{y}}$ for $\mathbf{x},\mathbf{y}$ chosen from a fixed sphere). Then the following holds:
\begin{align}
\begin{split}
\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}})=\frac{1}{\sqrt{2m}}\exp(2r^{2}\sin^{2}(\frac{\theta}{2}))\left(1-\exp(-4r^{2}\sin^{2}(\frac{\theta}{2}))\right)\\
\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}})=\frac{1}{\sqrt{2m}}\exp(2r^{2}\cos^{2}(\frac{\theta}{2}))
\left(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2}))\right),
\end{split}
\end{align} and consequently for $W(r)=\exp(2r^{2})
\left(1-\exp(-4r^{2})\right)$:
\begin{equation}
\epsilon_{S(r)}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}) = 
\epsilon_{S(r)}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}) = \lim_{\theta \rightarrow \pi} \epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}) = 
\lim_{\theta \rightarrow 0} \epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}) =
\sqrt{\frac{1}{2m}}W(r)
\end{equation}
\end{lemma}
Thus interestingly there is a symmetry between both the mechanisms that is captured by the defined relative error since $\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}})$ can be obtained from $\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}})$ by the transformation $\theta \rightarrow \pi - \theta$.

Thus both mechanisms achieve the same max-relative-error yet, as we have noticed before, in different regions of space. Estimator $\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}$ works much better than $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}$ for linear attention in Performers \citep{performer}, since in the attention tensor there are many more small values (where it is more accurate) than large values (where the latter one is more accurate).

\begin{proof}
The first two equations follow directly from Lemma \ref{normalized_input_lemma}:
Notice that this error is the increasing function of $\sin^{2}(\frac{\theta}{2})$ and thus is largest for $\theta=\pi$. Plugging in this value into the formula of the max-relative-error gives us thee expression from the statement of the lemma. By the analogous analysis, we obtain second equation (this time the error is maximized for $\theta=0$).
\end{proof}

\subsubsection{Computational gains of hybrid estimators}

Consider the general hybrid estimator of $\mathrm{SM}(\mathbf{x},\mathbf{y})$ from Equation \ref{gen-hyb-eque}, using $p+1$ base estimators.
Assume that the $k^{th}$ base estimator for $k=1,...,p+1$ applies $m$ random features in each of the corresponding $t_{k}$ random maps  and that $n$ random features are used in each of the corresponding $l_{\lambda_{k}}$ random maps to approximate $k^{th}$ $\lambda$-coefficient for $k=1,...,p$.
From Equation \ref{hyb-all-1} and Equation \ref{hyb-all-2}, we conclude that time complexity of constructing $\Psi(\mathbf{z})$ is:
\begin{equation}
T = O\left((t_{1}+...+t_{p+1})md + 
(nd + md + mn)\sum_{k=1}^{p+1}\sum_{r=1}^{p}t_{k}l_{\lambda_{r}}\right)
\end{equation}
Thus the resulting $\Theta(mn)$-dimensional random feature map $\Psi(\mathbf{z})$. 



\subsubsection{Hybrid Gaussian-mixtures estimators}

We consider now the prominent special case of the general hybrid estimator mechanism described above, the so-called \textit{hybrid gaussian-mixtures estimators}. In that setting, functions $\alamgen$ are defined as:
\begin{equation}
\alamgen = \exp(-\frac{\|\mathbf{x}+\mathbf{M}_{k}\mathbf{y}\|_{2}^{2}}{2\tau_{k}^{2}}),    
\end{equation}
for some $\mathbf{M}_{1},...,\mathbf{M}_{p} \in \mathbb{R}^{d \times d}$ and $\tau_{1},...,\tau_{p} \in \mathbb{R}$. Since lambda-coefficients are here the values of the Gaussian kernel between vectors: $\frac{\mathbf{x}}{\tau_{k}}$ and $-\frac{\mathbf{M}_{k}\mathbf{y}}{\tau_{k}}$ and furthermore Gaussian and softmax-kernels are related as given by Eq. \ref{gaussian_to_softmax}, we can take $a_{k}=0$ and define corresponding $\phi_{n}^{\lambda_{k}}$ as:

\begin{equation}
\left\{ \begin{array}{rcl}
\phi_{n}^{\lambda_{k}}(\mathbf{z}) = \exp(-\frac{\|\mathbf{z}\|_{2}^{2}}{2\tau_{k}^{2}})\phi_{n}^{\mathrm{SM}}(\frac{\mathbf{z}}{\tau_{k}}) \textrm{ if $\mathbf{z}=\mathbf{x}$}  \\
\phi_{n}^{\lambda_{k}}(\mathbf{z}) = \exp(-\frac{\|\mathbf{M}_{k}\mathbf{z}\|_{2}^{2}}{2\tau_{k}^{2}})\phi_{n}^{\mathrm{SM}}(-\frac{\mathbf{M}_{k}\mathbf{z}}{\tau_{k}}) \textrm{ if $\mathbf{z}=\mathbf{y}$}
\end{array}\right.
\end{equation}

where $\phi_{n}^{\mathrm{SM}}$ is the random feature map corresponding to a particular estimator of the softmax-kernel.



\subsubsection{Bipolar hybrid estimators}
Now take another special case of the general hybrid estimator defined above,
where $\mathcal{E} = (\widehat{\mathrm{SM}}^{++}(\mathbf{x},\mathbf{y}),\widehat{\mathrm{SM}}^{\mathrm{trig}}(\mathbf{x},\mathbf{y}))$. Thus consider estimator $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ of the softmax kernel $\mathrm{SM}$:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y})=\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y}) + (1-\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y}).   
\end{equation}

The question arises what concentration results can be obtained for $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ and how they compare to those for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$ and $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$. That of course depends also on the choice of $\lambda:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$.

If we consider a renormalized case where all input vectors have the same norm $r$, we can rewrite $\lambda(\mathbf{x},\mathbf{y})$ ad $\lambda(\theta_{\mathbf{x},\mathbf{y}})$, where $\theta_{\mathbf{x},\mathbf{y}}$ is an angle between $\mathbf{x}$ and $\mathbf{y}$ (we will use shorter notation $\theta$ if $\mathbf{x}$ and $\mathbf{y}$ are known from the context).
If $\|\mathbf{x}\|=\|\mathbf{y}\|=r$, then by Lemma \ref{normalized_input_lemma} we know that $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$ becomes perfect for $\theta=\pi$ and $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$ becomes perfect for $\theta=0$. That suggests particular forms of the mapping $\lambda$. Before exploring this further, we provide some general concentration results regarding bipolar hybrid estimators.

\subsubsection{General results for bipolar hybrid estimators}
\label{general-hybrid-section}

Below we present several general concentration results regarding hybrid estimators. We will refer to those estimators as
$\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})$ since the implicit dependence on $n$ will be hidden in the expressions involving estimators $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ that we will treat as blackboxes now. Analysis of the particular important instantiations of $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ will be conducted later.

\begin{theorem}[MSE of the general bipolar hybrid estimator]
\label{general-hybrid}
Take the bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$). Then the following holds:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{equation}
Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator is further reduced, namely we have:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]
\end{split}
\end{align}
\end{theorem}

\begin{proof}
The following holds:
\begin{align}
\begin{split}
\label{main_var_formulae}
\mathrm{Var}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = 
\mathrm{Var}\left(\widehat{\lambda}(\theta)\widehat{\mathrm{SM}}^{++}_{m}(\mathbf{x},\mathbf{y})\right) + \mathrm{Var}\left((1-\widehat{\lambda}(\theta))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})\right) + \\
2\mathrm{Cov}\left(\widehat{\lambda}(\theta)\widehat{\mathrm{SM}}^{++}_{m}(\mathbf{x},\mathbf{y}), (1-\widehat{\lambda}(\theta))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})\right) 
\end{split}
\end{align}

We will focus now on the covariance term.
Assume first easier to analyze case where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently. Then the following is true:

\begin{align}
\begin{split}
\cov\left(\alam \expo, \aonelam \tri\right) = \\ 
\mathbb{E}[\alam \aonelam \expo \tri] - \mathbb{E}[\alam \expo]\mathbb{E}[\aonelam \tri] \\
= \left(\mathbb{E}[\alam \aonelam]-\mathbb{E}[\alam]\mathbb{E}[\aonelam]\right)\mathbb{E}[\expo]\mathbb{E}[\tri] \\ = -(\sm)^{2}\var(\alam)
\end{split}
\end{align}


Now assume that $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ use the exact same random projections. Then, using similar analysis as before, we get:
\begin{align}
\begin{split}
\cov\left(\alam \expo, \aonelam \tri\right) = \\
\mathbb{E}[\expo \tri]\mathbb{E}[\alam \aonelam] - (\sm)^{2}\mathbb{E}[\alam]\mathbb{E}[\aonelam]
\end{split}    
\end{align}
This time however it is no longer the case that $\mathbb{E}[\expo \tri]\mathbb{E}[\alam \aonelam] = \mathbb{E}[\expo]\mathbb{E}[\tri]=(\sm)^{2}$ since $\expo$ and $\tri$ are no longer independent.
In order to compute $\mathbb{E}[\expo \tri]\mathbb{E}[\alam \aonelam]$, we will first introduce useful denotation.

Denote by $\omega_{1},...,\omega_{m} \overset{\mathrm{iid}}{\sim} \mathcal{N}(0,\mathbf{I}_{d})$ the random projections sampled to construct both $\expo$ and $\tri$. Denote: $Y_{i}=\cosh(\omega_{i}^{\top}(\mathbf{x}+\mathbf{y}))\overset{\mathrm{def}}{=}\frac{\exp(\omega_{i}^{\top}(\mathbf{x}+\mathbf{y}))+\exp(-\omega_{i}^{\top}(\mathbf{x}+\mathbf{y}))}{2}$. We have:
\begin{equation}
\expo = \exp\left(-\frac{\|\mathbf{x}\|^{2}+\|\mathbf{y}\|^{2}}{2}\right)\frac{Y_{1}+...+Y_{m}}{m}    
\end{equation}
If we denote: $Z_{i} = \cos(\omega_{i}^{\top}(\mathbf{x}-\mathbf{y}))$, then we can write $\tri$ as:
\begin{equation}
\tri = \exp\left(\frac{\|\mathbf{x}\|^{2}+\|\mathbf{y}\|^{2}}{2}\right)\frac{Z_{1}+...+Z_{m}}{m}    
\end{equation}

We can then rewrite $\mathbb{E}[\expo \tri]$ as:
\begin{align}
\begin{split}
\mathbb{E}[\expo \tri] = 
\frac{1}{m^{2}}\left[\sum_{i \neq j} \mathbb{E}[Y_{i}Z_{j}] +  \sum_{i=1}^{m}\mathbb{E}[Y_{i}Z_{i}]\right]
= \\ \frac{1}{m^{2}}\left[ {m \choose 2} (\sm)^{2} + m \mathbb{E}[\cosh(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))]\right],
\end{split}
\end{align}
where $\omega \sim \mathcal{N}(0,\mathbf{I}_{d})$. The equality follows from the unbiasedness of $\tri$ and $\expo$ and the fact that different $\omega_{i}$ are chosen independently. Thus it remains to compute $\rho = \mathbb{E}[\cosh(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))]$. Note first that 
$\rho = \mathbb{E}[\exp(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))]$
since $-\omega \sim \gauss$ and $\cos$ is an even function. Denote $\mathbf{z}=\mathbf{x}+\mathbf{y} + \mathbf{i}(\mathbf{x}-\mathbf{y})$. We have:
\begin{align}
\begin{split}
\mathbb{E}[\exp(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))] 
= \mathrm{Re}\left[\mathbb{E}[\exp(\omega^{\top}\mathbf{z})]\right] = \mathrm{Re}[\prod_{i=1}^{d}\exp(\frac{z_{i}^{2}}{2})] = \\
\mathrm{Re}\left[\exp\left(\frac{\sum_{j=1}^{d}(x_{j}+y_{j})^{2}+2\mathbf{i}(x_{j}^{2}-y_{j}^{2})-(x_{j}-y_{j})^{2}}{2}\right)\right]=(\sm)^{2}\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2})
\end{split}
\end{align}
Thus we conclude that:
\begin{equation}
\mathbb{E}[\expo \tri] = (1-\frac{1}{m})(\sm)^{2} + \frac{1}{m}(\sm)^{2}\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2})    
\end{equation}

Therefore we get the formulae for the covariance term in both: the setting where random projections of $\tri$ and $\expo$ are shared (variant II) and when they are not (variant I). The following is true 
for $Z=\frac{1}{m}(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2})\mathbb{E}[\alam \aonelam]$:

\begin{equation}
\cov(\alam \expo, \aonelam \tri)=
\left\{ \begin{array}{rcl}
-(\sm)^{2}\mathrm{Var}(\alam) \textrm{ for variant I}  \\ 
-(\sm)^{2}(\mathrm{Var}(\alam)+Z) \textrm{ for variant II}
\end{array}\right.
\end{equation}

We also have the following:
\begin{align}
\begin{split}
\mathrm{Var}(\alam \expo) = \mathbb{E}[(\alam)^{2} (\expo)^{2}] - (\mathbb{E}[\alam \expo])^{2} = \\
\mathbb{E}[(\alam)^{2}]\left(\mathrm{MSE}(\expo)+(\sm)^{2}\right) - (\mathbb{E}[\alam])^{2}(\sm)^{2} = \\
(\sm)^{2}\mathrm{Var}(\alam) + \mathbb{E}[(\alam)^{2}]\mathrm{MSE}(\expo)
\end{split}
\end{align}
and furthermore (by the analogous analysis):
\begin{equation}
\mathrm{Var}(\aonelam \tri)  =    
(\sm)^{2}\mathrm{Var}(\alam) + \mathbb{E}[\aonelam^{2}]\mathrm{MSE}(\tri)
\end{equation}

By putting the derived formulae for the above variance terms as well as covariance terms back in the Equation \ref{main_var_formulae}, we complete the proof of the theorem (note that the mean squared error of the hybrid estimator is its variance since it is unbiased).

\end{proof}

\subsubsection{Lambda-angular bipolar hybrid estimators}

From the discussion just before Section \ref{general-hybrid-section}, we conclude that, for the renormalized case,  by choosing $\lambda: \mathbb{R} \rightarrow \mathbb{R}$ such that $\lambda(0)=0$ and $\lambda(\pi)=1$, and furthermore: $\widehat{\lambda}(0)=\widehat{\lambda}(\pi)=0$, we zero out the variance of $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ in \textbf{both}: $\theta=0$ and $\theta=\pi$ rather than just in one of these points (as it is the case for $\widehat{\mathrm{SM}}_{m}^{++}$ or $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}$). Below we propose such a $\lambda$ and $\widehat{\lambda}$.
The easiest choice is to take $\lambda$ to be linear, i.e.:
\begin{equation}
\lambda(\theta) = \frac{\theta}{\pi}    
\end{equation}
To construct $\widehat{\lambda}$, we notice first that the random feature map $\phi_{\mathrm{ang}}$ for the \textit{angular kernel} given as:
\begin{equation}
\mathrm{K}_{\mathrm{ang}}(\mathbf{x},\mathbf{y}) = 1 - \frac{2\theta_{\mathbf{x},\mathbf{y}}}{\pi}    
\end{equation}
is, for $\tau_{1},...,\tau_{n} \sim \mathcal{N}(0,\mathbf{I}_{d})$, defined as:
\begin{equation}
\phi_{n}^{\mathrm{ang}}(\mathbf{z}) = \frac{1}{\sqrt{n}}(\mathrm{sgn}(\tau_{1}^{\top}\mathbf{z}),...,\mathrm{sgn}(\tau_{n}^{\top}\mathbf{z}))^{\top} 
\end{equation}
Therefore we have: 
\begin{equation}
\lambda(\theta) = \frac{\theta}{\pi} = 
\frac{1}{2} - \frac{1}{2}\mathbb{E}[(\phi_{n}^{\mathrm{ang}}(\mathbf{x}))^{\top}\phi_{n}^{\mathrm{ang}}(\mathbf{y})]
\end{equation}
Thus we can construct $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ from Equation \ref{lambda-eq} by taking: 
\begin{equation}
\left\{ \begin{array}{rcl}
a = \frac{1}{2} \\ 
\phi_{n}^{\lambda}(\mathbf{z}) = \frac{i}{\sqrt{2}}\phi_{n}^{\mathrm{ang}}(\mathbf{z})
\end{array}\right.
\end{equation}

We call a hybrid estimator applying such a $\widehat{\lambda}$ as the \textit{lambda-angular bipolar hybrid estimator}. 

We will now compute:
$\alpha = \mathbb{E}[\widehat{\lambda}(\theta)^{2}], \beta = \mathbb{E}[\aonelam^{2}]$ and $\gamma = \mathbb{E}[\alam \aonelam]$ to obtain the formulae of the MSE of the lambda-angular bipolar hybrid estimator according to Theorem \ref{general-hybrid}.
Denote: 
$X_{i} = (\phi_{n}^{\mathrm{ang}}(\mathbf{x}))[i]\phi_{n}^{\mathrm{ang}}(\mathbf{y})[i]$. We have:
\begin{equation}
\widehat{\lambda}(\theta) = \frac{1}{2}\left(1 - 
\sum_{i=1}^{n}X_{i}\right).
\end{equation}
Note first that by the construction of $\widehat{\lambda}(\theta)$, we have: $\mathbb{E}[\widehat{\lambda}(\theta)] = \frac{\theta}{\pi}$ and thus: $\mathbb{E}[\sum_{i=1}^{n} X_{i}] = 1-\frac{2\theta}{\pi}$.
Therefore we conclude that:
\begin{align}
\begin{split}
\label{alpha_eq}
\alpha = \frac{1}{4}\mathbb{E}\left[1-2\sum_{i=1}^{n}X_{i}+
\left(\sum_{i=1}^{n}X_{i}\right)^{2}\right]
= \frac{1}{4}\left(1-2(1-\frac{2\theta}{\pi})+\sum_{i=1}^{n}\mathbb{E}[X_{i}^{2}]+\sum_{i \neq j}\mathbb{E}[X_{i}]\mathbb{E}[X_{j}]\right) \\ =
\frac{1}{4}\left(1-2(1-\frac{2\theta}{\pi})+n \cdot \frac{1}{n^{2}}+n(n-1) \cdot \frac{1}{n^{2}}(1-\frac{2\theta}{\pi})^{2}\right)=
\frac{1}{4}\left(4\frac{\theta}{\pi} + (1-\frac{1}{n})(1-\frac{2\theta}{\pi})^{2}\right) \\
= \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)
\end{split}
\end{align}

Now to calculate $\beta$, it suffices to observe that $1 - \widehat{\lambda}(\theta)$ has the same distribution as $\widehat{\lambda}(\mathbf{x},-\mathbf{y})$. Therefore we only need to substitute in Equation \ref{alpha_eq} angle $\theta$ with $\pi - \theta$ and we get:
\begin{equation}
\beta = \frac{\pi-\theta}{\pi}\left(\frac{\pi-\theta}{\pi}-\frac{\pi-\theta}{n\pi}+\frac{1}{n}\right) = 
\left(1-\frac{\theta}{\pi}\right)\left(1-\frac{\theta}{\pi}+\frac{\theta}{n\pi}\right)
\end{equation}
Finally, the following holds:
\begin{equation}
\gamma = \mathbb{E}[\widehat{\lambda}(\theta)] - \alpha = 
\frac{\theta}{\pi} - \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right) = \frac{\theta}{\pi}
\left(1-\frac{1}{n}-\frac{\theta}{\pi}+\frac{\theta}{n \pi}\right)
\end{equation}

Using Theorem \ref{general-hybrid}, we conclude that:

\begin{theorem}[MSE of the lambda-angular bipolar hybrid estimator]
\label{lambda-bipolar-hybrid}
Take the lambda-angular bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$). Then the following holds:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})) = \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)\frac{1}{2m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2}))^{2} + \\   
= 
\left(1-\frac{\theta}{\pi}\right)\left(1-\frac{\theta}{\pi}+\frac{\theta}{n\pi}\right)\frac{1}{2m} \exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})
(1-\mathrm{exp}(-\|\Delta\|^{2}))^{2}
\end{split}
\end{align}
for $\Delta = \mathbf{x} - \mathbf{y}$ and $\mathbf{z} = \mathbf{x} + \mathbf{y}$.
Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator is further reduced, namely we have:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})) = \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)\frac{1}{2m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2}))^{2} + \\   
\left(1-\frac{\theta}{\pi}\right)\left(1-\frac{\theta}{\pi}+\frac{\theta}{n\pi}\right)\frac{1}{2m} \exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})
(1-\mathrm{exp}(-\|\Delta\|^{2}))^{2} \\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\frac{\theta}{\pi}
\left(1-\frac{1}{n}-\frac{\theta}{\pi}+\frac{\theta}{n \pi}\right)
\end{split}
\end{align}
\end{theorem}

Thus, based on the above and Lemma \ref{normalized_input_lemma}, if $\|\mathbf{x}\|_{2}=\|\mathbf{y}\|_{2}=r$ then regardless of whether the same sets of random projections are applied or not, we get:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})) = \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)\frac{1}{2m}\exp(8r^{2}\cos^{2}(\frac{\theta}{2})-2r^{2}) \cdot \\
(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2})))^{2} +    
\frac{\theta}{\pi}
\left(1-\frac{1}{n}-\frac{\theta}{\pi}+\frac{\theta}{n \pi}\right)\frac{1}{2m}\exp(2r^{2})(1-\exp(-4r^{2}\sin^{2}(\frac{\theta}{2})))^{2}
\end{split}
\end{align}

Below we estimate the max-relative-error of the lambda-angular bipolar hybrid estimator on the sphere $S(r)$ of radius r. We see that the max-relative-error scales as:
$\frac{1}{r}\exp(2r^{2})$ in $r$ as opposed to $\exp(2r^{2})$ as it is the case for the estimators based solely on positive or trigonometric random features (see: Lemma \ref{tri-exp-imp-lemma}). Furthermore, the max-relative-error scales as $\sqrt{\theta}$ and $\sqrt{\pi-\theta}$ as $\theta \rightarrow 0$ and $\theta \rightarrow \pi$ respectively, in particular goes to $0$ in both critical cases. This is not the case for the estimators based solely on positive or trigonometric random features (for a fixed radius $r$ and the number of random features used).  

\begin{theorem}
The max-relative-error of the lambda-angular bipolar hybrid estimator on the sphere $S(r)$ of radius $r \geq 1$ satisfies for $W(r)=\exp(2r^{2})
\left(1-\exp(-4r^{2})\right)$:
\begin{equation}
\label{hybang_upper}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}}) \leq \frac{1}{r}\sqrt{\frac{1}{2m}}W(r)\sqrt{\frac{1}{\pi} - \frac{1}{n \pi} + \frac{1}{n\sqrt{\pi}}}  
\end{equation}
Furthermore:
\begin{equation}
\label{lim_eq}
\lim_{\theta \rightarrow 0} \frac{\eps_{\theta, r}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}})}{\sqrt{\theta}}= 
\lim_{\theta \rightarrow \pi} \frac{\eps_{\theta, r}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}})}{\sqrt{\theta-\pi}} = \sqrt{\frac{1}{2\pi mn}}W(r)
\end{equation}
\end{theorem}
\begin{proof}
Note first that from the derived above formulae of the MSE of the lambda-angular bipolar hybrid estimator and the definition of the max-relative-error, we obtain:
\begin{equation}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}}) =
\frac{\exp(r^{2})}{\sqrt{2m}}\sqrt{\max_{\theta \in [0, \pi]} h_{r}(\theta)},
\end{equation}
where:
\begin{align}
\begin{split}
h_{r}(\theta) = a_{r}(\theta) + a_{r}(\pi-\theta)
\end{split}
\end{align}
and $a_{r}(\theta)$ is defined as:
\begin{equation}
a_{r}(\theta)=\frac{\theta}{\pi}(\frac{\theta}{\pi}-\frac{\theta}{n \pi}+\frac{1}{n})\exp(2r^{2}\cos(\theta))\left(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2}))\right)^{2}.    
\end{equation}
Therefore we have:
\begin{equation}
\label{hyb-rel-error-1}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}})
\leq \frac{\exp(r^{2})}{\sqrt{m}}\sqrt{\max_{\theta \in [0, \pi]} a_{r}(\theta)}
\end{equation}
Notice that:
\begin{equation}
\label{hyb-rel-error-2}
a_{r}(\theta) \leq b_{r}(\theta)
(1-\exp(-4r^{2}))^{2}
\end{equation}
where:
\begin{equation}
b_{r}(\theta) = b^{1}_{r}(\theta) + b^{2}_{r}(\theta)   
\end{equation}
and
\begin{equation}
b^{1}_{r}(\theta) = (1-\frac{1}{n}) \frac{\theta^{2}}{\pi^{2}}\exp(2r^{2}\cos(\theta)), 
\end{equation}
\begin{equation}
b^{2}_{r}(\theta) = \frac{1}{n}\cdot\frac{\theta}{\pi} \exp(2r^{2}\cos(\theta)).         
\end{equation}
Therefore: 
\begin{equation}
\label{hyb-rel-error-3}
\max_{\theta \in [0, \pi]}b_{r}(\theta) \leq \max_{\theta \in [0, \pi] }b^{1}_{r}(\theta)+
\max_{\theta \in [0, \pi] }b^{2}_{r}(\theta)
\end{equation}
Denote: $b^{1} = \max_{\theta \in [0, \pi] }b^{1}_{r}(\theta)$ and $b^{2} = \max_{\theta \in [0, \pi] }b^{2}_{r}(\theta)$.
Note that:
\begin{equation}
\frac{d b^{1}_{r}(\theta)}{d \theta} = 
\exp(2r^{2}\cos(\theta))
(1-\frac{1}{n})\frac{2\theta}{\pi^{2}}(1-r^{2}\theta \sin(\theta)) 
\end{equation}
and
\begin{equation}
\frac{d b^{2}_{r}(\theta)}{d \theta} = 
\exp(2r^{2}\cos(\theta))\frac{1}{n \pi}(1-2r^{2}\theta \sin(\theta))
\end{equation}

Thus, from the properties of function: $\theta \rightarrow \theta \sin(\theta)$ and the fact that $r \geq 1$, we conclude that both derivatives are first nonnegative, then nonpositive and then nonnegative abd that the unique local maximum on the interval $[0, \pi]$ is achieved for $\theta \leq \frac{\pi}{2}$.
Note also that $b^1_{r}(\theta),b^1_{r}(\theta) \geq 0$ and $b^{1}_{r}(0)=b^{2}_{r}(0)=0$, $b^{1}_{r}(\pi) = (1-\frac{1}{n})\exp(-2r^{2})$, $b^{2}_{r}(\pi)=\frac{1}{n}\exp(-2r^{2})$.
We conclude that global maximum for $b^{i}_{r}$ on the interval $[0, \pi]$ for $i=1,2$ is achieved either in its unique local maximum on that interval or for $\theta=\pi$. 
Let us consider first: $b^{1}_{r}$. In its local maximum on $[0, \pi]$ we have:
\begin{equation}
\theta^{*} sin(\theta^{*}) = \frac{1}{r^{2}}    
\end{equation}
Since $\theta \leq \sin(\theta) \cdot \frac{\pi}{2}$ on $[0, \frac{\pi}{2}]$, we get:
\begin{equation}
(\theta^{*})^{2} \leq \frac{\pi}{2}\frac{1}{r^{2}}, 
\end{equation} i.e.:
\begin{equation}
\theta^{*} \leq \sqrt{\frac{\pi}{2}}\frac{1}{r}    
\end{equation}
Therefore:
\begin{equation}
b^1_{r}(\theta^{*}) \leq (1-\frac{1}{n})\frac{1}{2\pi r^{2}}\exp(2r^{2}) \geq b^{1}_{r}(\pi)    
\end{equation}
We thus conclude that:
\begin{equation}
\max_{\theta \in [0, \pi]} b^{1}_{r}(\theta) \leq (1-\frac{1}{n})\frac{1}{2\pi r^{2}}\exp(2r^{2})
\end{equation}
By the completely analogous analysis applied to $b^{2}_{r}$, we obtain:
\begin{equation}
\max_{\theta \in [0, \pi]} b^{1}_{r}(\theta) \leq \frac{1}{2n\sqrt{\pi} r^{2}}\exp(2r^{2})
\end{equation}
Now, using Equation \ref{hyb-rel-error-1},
Equation \ref{hyb-rel-error-2}, Equation \ref{hyb-rel-error-3}, we obtain:
\begin{equation}
\eps_{S(r)}(\widehat{\mathrm{SM}})^{\mathrm{hybang}}_{m,n} \leq \frac{\exp(2r^{2})}{\sqrt{2m}r}(1-\exp(-4r^{2}))\sqrt{\frac{1}{\pi} - \frac{1}{n \pi} + \frac{1}{n\sqrt{\pi}}}
\end{equation}
and that completes the first part of the proof (proof of Inequality \ref{hybang_upper}).
Equation \ref{lim_eq} is directly implied by the fact that:
\begin{equation}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}}) = \frac{\exp(2r^{2})}{\sqrt{2m}}\sqrt{h_{r}(\theta)}    
\end{equation}
\end{proof}


\subsubsection{Truncated-Gaussian bipolar hybrid estimators}



If $\mathbf{x}$ and $\mathbf{y}$ have fixed L2 norm ($\|\mathbf{x}\|_2=\|\mathbf{y}\|_2=r$), we could propose a truncated gaussian hybrid estimator $\lambda: \mathbb{R} \rightarrow \mathbb{R}$ such that $\lambda(0)=0$ and $\lambda(\pi)=1$, and furthermore zeroes out the variance of $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ in \textbf{both}: $\theta=0$ and $\theta=\pi$:

$\lambda$ in our truncated-gaussian hybrid estimator is defined as:
\begin{equation}
\label{definition:truncated-gaussian-estimator1}
\lambda(\mathbf{x},\mathbf{y}) = \frac{1-\exp(-\frac{\sigma^2}{2}\|\mathbf{x-y}\|^{2})}{\rho} 
\end{equation}

where $\rho$ is given as:
\begin{equation}
\rho=1-\exp(-2\sigma^2r^2)
\end{equation}

The parameter $\sigma$ controls the smoothness of the gaussian kernel.

The exponential in $\lambda$ could be estimated by tri-geometric random features, and therefore we could derive the following estimator for $\lambda$:

\begin{equation}
\widehat{\lambda}(\mathbf{x},\mathbf{y}) = \frac{1}{\rho} - \frac{1}{n\rho}\sum_{i=1}^n \cos(\sigma (\omega_i^{\top}(\mathbf{x}-\mathbf{y})))
\end{equation}



Thus we can construct random feature maps for $\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}) = a - (\phi_{n}^{\lambda}(\sigma \mathbf{x}))^{\top}
\phi_{n}^{\lambda}(\sigma \mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = \frac{1}{\rho} \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{n\rho}}(\sin(\tau_{1}^{\top}\mathbf{z}), \cos(\tau_{1}^{\top}\mathbf{z}),...,\sin(\tau_{n}^{\top}\mathbf{z}), \cos(\tau_{n}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{n} \sim \mathcal{N}(0,\mathbf{I}_{d})$.




Using Theorem \ref{general-hybrid}, we conclude that:

\begin{theorem}[MSE of the truncated-gaussian bipolar hybrid estimator]
\label{truncated-gaussian-hybrid}
Take the truncated-gaussian bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\mathbf{x},\mathbf{y})$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$). Then the following holds:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{equation}

where 
\begin{equation}
\mathbb{E}[(\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \frac{1}{\rho^2}(1-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 
\end{equation}
\begin{equation}
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] =\frac{1}{\rho^2}((1-\rho)-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2
\end{equation}

Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator remains the same.

\end{theorem}



\begin{proof}

We could calculate $\mathbb{E}[(\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2]$ and $\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2]$ as follows:

\begin{equation}
\begin{split}
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \frac{1}{\rho^2} \mathbb{E}[(\rho-1+\frac{1}{n}\sum_{i=1}^n \cos(\sigma \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\ 
=\frac{(1-\rho)^2}{\rho^2}+\frac{2(\rho-1)}{\rho^2}\mathbb{E}[\cos(\sigma \omega^{\top}(\mathbf{x}-\mathbf{y}))]+\frac{1}{\rho^2}\mathbb{E}[(\frac{1}{k}\sum_{i=1}^n\cos(\sigma \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\
= \frac{(1-\rho)^2}{\rho^2}+\frac{2(\rho-1)}{\rho^2}\exp(-\frac{\sigma^2}{2}\|\Delta\|^{2})+\frac{1}{\rho^2}\exp(-\sigma^2\|\Delta\|^2) + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 \\
= \frac{1}{\rho^2}((1-\rho)-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 
\end{split}
\end{equation}





\begin{equation}
\begin{split}
\mathbb{E}[(\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] = 1-2\mathbb{E}[1-\widehat{\lambda}(\mathbf{x},\mathbf{y})] + \mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= -1 + \frac{2}{\rho}- \frac{2}{\rho}\exp(-\frac{\sigma^2}{2}\|\Delta\|^{2}) + \mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= \frac{1}{\rho^2}(1-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 
\end{split}
\end{equation}

And the theorem holds by plugging in these two parts.

Note that if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$ apply the exact same sets of random projections, then $(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))$ in $\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\mathbf{x},\mathbf{y}))$ becomes zero in Theorem \ref{truncated-gaussian-hybrid}, therefore the MSE remains the same.


\end{proof}





We could rewrite Eq. \ref{definition:truncated-gaussian-estimator1} and provide another definition for $\lambda$ by replacing $\mathbf{x}$ and $\mathbf{y}$ with their angle $\theta$ and norm $r$:


\begin{equation}
\label{definition:truncated-gaussian-estimator2}
\lambda(\theta,r) =  \frac{1-\exp(-2\sigma^2r^2\sin(\frac{\theta}{2})^2)}{\rho}
\end{equation}




\begin{theorem}[MSE of the truncated-gaussian bipolar hybrid estimator with $\theta$ and $r$]
\label{truncated-gaussian-hybrid2}
We could rewrite Theorem \ref{truncated-gaussian-hybrid} with $\theta$ and $r$ as follows:
Take the truncated-gaussian bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\theta,r)$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\theta,r)$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$). Then the following holds:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{equation}
where 
\begin{equation}
\mathbb{E}[(\widehat{\lambda}(\theta, r))^2] = \frac{1}{\rho^2}(1-\exp(-2\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-4\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{equation}
\begin{equation}
\mathbb{E}[(1-\widehat{\lambda}(\theta, r))^2] =\frac{1}{\rho^2}((1-\rho)-\exp(-2\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-4\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{equation}
Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator will remain the same.
\end{theorem}



\begin{proof}
For $\|x\|^2=\|y\|^2=r^2$, the following holds for $\Delta=\mathbf{x}-\mathbf{y}$:
\begin{equation}
\|\Delta\|^2 = 4r^2\sin(\frac{\theta}{2})^2
\end{equation}

And this theorem holds trivially by replacing $\|\Delta\|^2$ in Theorem \ref{truncated-gaussian-hybrid}.

\end{proof}



\subsubsection{Hybrid Gaussian-Mixtures Estimators with Clusters}



If the input matrices $\mathbf{Q}, \mathbf{K}$ can be clustered into $n_q$ and $n_k$ groups respectively (using k-means clustering algorithm for example), with the center point of each group as $\mathbf{r}_i\in \mathbb{R}^d$, ($i=1,...,n_k$) and $\mathbf{r}_j\in \mathbb{R}^d$, ($j=1,...,n_q$), then there exist $n_q n_k$ pairs of $(\mathbf{r}_i, \mathbf{r}_j)$, ($i=1,...,n_q, j=1,...,n_k$), so we can construct $n_q n_k$ softmax estimators to estimate cross-group softmax values. In the following text, we use $\mathbf{x}$ and $\mathbf{y}$ to represent a pair of such centers $\mathbf{r}_i$ and $\mathbf{r}_j$.



Consider $\mathbf{z} = \mathbf{A}\mathbf{r}_i + \mathbf{(A^{\top})^{-1}}\mathbf{r}_j$ for an invertible (in $\mathbb{C}^{d \times d})$ matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$, an estimator based on this mechanism has variance equal to $0$ if:
\begin{equation}
\label{eq:z_ax_by_0}
\mathbf{z} = \mathbf{A}\mathbf{r}_i + \mathbf{(A^{\top})^{-1}}\mathbf{r}_j = 0
\end{equation}

We assume here that $\mathbf{A}$ is a diagonal matrix, so $\mathbf{A}=\mathbf{A^{\top}}$. Then we can rewrite the above equation as:
\begin{equation}
\mathbf{z} = \mathbf{A}\mathbf{r}_i + \mathbf{(A)^{-1}}\mathbf{r}_j = 0
\end{equation}

Since position $(k,k)$ in matrix $\mathbf{A}$ is a composite value with the form $\alpha_k + \beta_k i$, we need to satisfy the following equation for each k=1,...,d:
\begin{equation}
(\alpha_k + \beta_k i)r_{i,k} + \frac{1}{\alpha_k + \beta_k i}r_{j,k} = 0
\end{equation}

\begin{equation}
(\alpha_k + \beta_k i)r_{i,k} + \frac{\alpha_k - \beta_k i}{\alpha_k^2 + \beta_k^2 }r_{j,k} = 0
\end{equation}

where $r_{i,k}$ is the $k$-th entry of vector $\mathbf{r}_i$.

We can simplify this equation and separate into real and imaginary part:
\begin{equation}
\label{eq:gaussian-mixtures-with-clusters}
\left\{ \begin{array}{rcl}
\mathbf{Re}: (\alpha_k^2+\beta_k^2)\alpha_k r_{i,k} + \alpha_k r_{j,k} = 0 \\ 
\mathbf{Im}: (\alpha_k^2+\beta_k^2)\beta_k r_{i,k}- \beta_k r_{j,k} = 0 \\ 
\end{array}\right.
\end{equation}

Our goal now is to choose values for $\alpha_k$ and $\beta_k$ given $\mathbf{r}_i$ and $\mathbf{r}_j$.

If $r_{i,k} r_{j,k}>0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=0 \\ 
\beta_k=\sqrt{r_{j,k}/r_{i,k}} \\ 
\end{array}\right.
\end{equation}

And if $r_{i,k} r_{j,k}<0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=\sqrt{-r_{j,k}/r_{i,k}} \\ 
\beta_k= 0\\ 
\end{array}\right.
\end{equation}


When $r_{i,k}=r_{i,k}=0$,  we could assume $\alpha_k=\beta_k=1$. If $r_{i,k}=0, r_{j,k}\neq 0$ or the opposite, then we cannot satisfy the above equation perfectly. We could assume $\alpha_k$ to some large positive value and set $\beta_k=0$ when $r_{i,k}=0, r_{j,k}\neq 0$, and set $\alpha_k=\beta_k$ to some small positive value close to zero when $r_{i,k}\neq0, r_{j,k}=0$. 

In the following text, we define matrix $\mathbf{A}$ calculated from Eq. \ref{eq:gaussian-mixtures-with-clusters} given $\mathbf{r}_i$ and $\mathbf{r}_j$ as $\mathbf{A}^{i,j}$.




For arbitrary vectors $\mathbf{x}, \mathbf{y} \in \mathbb{R}^d$, we know from equation (16):
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2})  
\mathrm{exp}(\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2})\mathrm{SM}(\mathbf{x},\mathbf{y})  
= \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{A}^{i,j}\mathbf{x}+(\mathbf{A}^{i,j})^{-1}\mathbf{y})]
\end{equation}


Therefore, the softmax can be estimated as:

\begin{equation}
\label{eq:sm_decompo}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})]
\end{equation}


with $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})$ given by:


\begin{equation}
\label{def:rfm-sm-x}
\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j}\mathbf{x}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j}\mathbf{x}))^{\top}
\end{equation}

\begin{equation}
\label{def:rfm-sm-y}
\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}),...,\mathrm{exp}(\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}))^{\top}
\end{equation}

for $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$.

And such softmax estimator will have variance of zero if $\mathbf{x}=\mathbf{r}_i$ and $\mathbf{y}=\mathbf{r}_j$. For other pairs of vectors $(\mathbf{x}, \mathbf{y})$ close to $\mathbf{r}_i$ and $\mathbf{r}_j$, the variance should be small.  


We could also define the gaussian lambda coefficient estimator that gets it maximum value when $\mathbf{x}=\mathbf{r}_i, \mathbf{y}=\mathbf{r}_j$ as $\lambda^{i,j}(\mathbf{x}, \mathbf{y})$. Such estimator could be constructed with $\mathbf{A}^{i,j}$ in a similar way. 

It could be decomposed in the following manner:


\begin{align}
\begin{split}
\lambda^{i,j}(\mathbf{x}, \mathbf{y}) = \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x} + (\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2\tau^2}) 
= \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2\tau^2})\mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2\tau^2})\mathrm{SM}(\frac{\mathbf{x}}{\tau},\frac{\mathbf{-y}}{\tau})
\end{split}
\end{align}

where $\mathrm{SM}({\mathbf{x}}/{\tau},{\mathbf{-y}}/{\tau})$ could be estimated with similar random feature maps as given by Eq. \ref{eq:sm_decompo}.

Therefore, the gaussian lambda coefficients could be estimated as:


\begin{align}
\begin{split}
\lambda^{i,j}(\mathbf{x}, \mathbf{y}) = \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x} + (\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2\tau^2}) = \mathbb{E}[\Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} 
\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})]
\end{split}
\end{align}

with $\Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y})$ given by:


\begin{equation}
\label{def:rfm-lambda-x}
\Psi^{\tau, m}_{\mathbf{A}^{i,j}} (\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j} \mathbf{x}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau))^{\top}
\end{equation}

\begin{equation}
\label{def:rfm-lambda-y}
\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau))^{\top}
\end{equation}

  
for $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$ chosen independently with $\omega$'s used in softmax estimators defined before.









\begin{definition}[Hybrid Gaussian-Mixtures Estimators with Clusters]
\label{truncated-gaussian-hybrid2}

If the matrices $\mathbf{Q}, \mathbf{K} \in \mathbb{R}^{d\times d}$ can be clustered into $n_q$ and $n_k$ groups respectively, with the center point of each group as $\mathbf{r}_i$ and $\mathbf{r}_j\in \mathbb{R}^d$, ($i=1,...,n_k$, $j=1,...,n_q$),  then we denote $\mathbf{A}^{i,j}$ as the composite matrix satisfies Eq. (\ref{eq:gaussian-mixtures-with-clusters}) with center $\mathbf{r}_i, \mathbf{r}_j$, and denote $\mathcal{E}=( \widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of the softmax-kernel $\mathrm{SM}^{i,j}(\mathbf{x},\mathbf{y})$ and $\Lambda = \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of $\lambda^{i,j}(\mathbf{x},\mathbf{y})$ constructed independently from $\mathcal{E}$.

Then our hybrid estimator takes the following:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y})
\end{equation}

with constraint:

\begin{equation}
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) = 1
\end{equation}

the lambda coefficients and softmax value are estimated with random feature maps:

\begin{equation}
\widehat{\lambda}^{i,j}(\mathbf{x}, \mathbf{y}) = \Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} \Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) 
\end{equation}

\begin{equation}
\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top}\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})
\end{equation}


where $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}), \Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y}), \Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x}), \Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y})$ are given by Eq. (\ref{def:rfm-sm-x}, \ref{def:rfm-sm-y}, \ref{def:rfm-lambda-x}, \ref{def:rfm-lambda-y}).


\end{definition}




















\begin{definition}[Hybrid Zero-One-Mixtures Estimators with Clusters]
\label{truncated-gaussian-hybrid2}

If the matrices $\mathbf{Q}, \mathbf{K} \in \mathbb{R}^{d\times d}$ can be clustered into $n_q$ and $n_k$ groups respectively, with the center point of each group as $\mathbf{r}_i$ and $\mathbf{r}_j\in \mathbb{R}^d$, ($i=1,...,n_k$, $j=1,...,n_q$),  then we denote $\mathbf{A}^{i,j}$ as the composite matrix satisfying Eq. (\ref{eq:gaussian-mixtures-with-clusters}) with center $\mathbf{r}_i, \mathbf{r}_j$, and denote $\mathcal{E}=( \widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of the softmax-kernel $\mathrm{SM}^{i,j}(\mathbf{x},\mathbf{y})$ and $\Lambda = \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of $\lambda^{i,j}(\mathbf{x},\mathbf{y})$ constructed independently from $\mathcal{E}$.

Then our hybrid estimator takes the following:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y})
\end{equation}

with constraint:

\begin{equation}
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) = 1
\end{equation}

the lambda coefficients and softmax value are estimated with random feature maps:

\begin{equation}
\widehat{\lambda}^{i,j}(\mathbf{x}, \mathbf{y}) = \Psi_i(\mathbf{x})  \Psi_j(\mathbf{y})
\end{equation}

\begin{equation}
\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top}\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})
\end{equation}


where $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}), \Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})$ are given by Eq. (\ref{def:rfm-sm-x}, \ref{def:rfm-sm-y}) and $\Psi_i(\mathbf{x})$ is a scalar indicating whether $\mathbf{x}$ belongs to the $i$-th cluster of $\mathbf{Q}$ and similarly 
$\Psi_j(\mathbf{y})$ is a scalar indicating whether $\mathbf{y}$ belongs to the $j$-th cluster of $\mathbf{K}$. 

\end{definition}


==> computation_arccos_kernels.tex <==
%% Add some of my results on arc cos kernels 
\subsection{Definitions and Some Results}
Arc cosine kernels introduced in~\cite{arccosnips, arccos} is defined as
\begin{equation}~\label{eqn:arccoskernel}
    k_n(x,y)  = 2 \int dw \frac{e^{\frac{-||w||^2}{2}}}{(2\pi)^{d/2}} \Theta(w\cdot x) \Theta(w \cdot y)(w \cdot x)^{n}(w \cdot y)^{n}.
     \end{equation}
     where, 
     $\Theta(x) = \frac{1}{2}(1+ \text{sign}(x))$ is the Heaviside function. 
     These kernels can be computed analytically for non-negative integers $n$ and moreover the integral converges for $n > - \frac{1}{2}$. 
     
    The above integral has a simple dependence on the magnitudes of $x$ and $y$ but a complicated relation on the angle $\theta$ between them. This dependence will be explored in detail below. Write, 
    \begin{equation}~\label{eqn:splitkernel}
        k_n(x,y) = \frac{1}{\pi} ||x||^{n}||y||^n J_n(\theta)
    \end{equation}

$J_n (\theta)$ is given the following differential equation. 
\begin{equation}~\label{eqn:cosdiff}
J_n(\theta)  =  (-1)^{n}(\text{sin}\theta)^{2n+1}\bigg(\frac{1}{sin\theta}\frac{\partial}{\partial \theta}\bigg)^{n} \bigg(\frac{\pi - \theta}{\text{sin}\theta}\bigg)
\end{equation}
Alternatively, $J_n(\theta)$ also has an integral representation
\begin{equation}~\label{eqn:cosint}
J_n(\theta) = n! (\text{sin}\theta)^{2n+1} \int_{0} ^{\pi/2}d\psi \frac{\text{cos}^{n}\psi}{(1-\text{cos}\theta \text{cos}\psi)^{n+1}}
\end{equation}
    
\begin{lemma}~\label{recrel}
$J_n(\theta)$ satisfies a recurrence relation of the form
\begin{equation*}
    J'_n(\theta) = (2n+1)\text{cot}(\theta)J_n(\theta) - \text{csc}(\theta)J_{n+1}(\theta)
\end{equation*}
\end{lemma}
\begin{proof}
Proof is a straightforward application of chain rule and differentiation under the integral sign. In the proof of the lemma we used the integral representation of $J_n (\theta)$~(Equation~\ref{eqn:cosint}). 
\end{proof}
%% Can come in handy for some other proofs

\subsection{Variants of the Arc Cos Kernel}
$J_0$ is not differentiable, since $\text{cos}^{-1}(z)$ is not differentiable at $z = \pm 1$. However the following easy lemma is true: 
\begin{lemma}
$\frac{J^{n}_{0}}{\pi^n}$ is differentiable at $\theta =0$ for $n \geq 2 $. 
\end{lemma}
\begin{proof}
Proof is a simple application of L'Hopital's rule.
\end{proof}
% An easy observation is : the variance of $\frac{J^{n}_{0}}{\pi^n}$ is a decreasing function of $n$. \\
However the above functions are still not differentiable at $\pi$. But the higher order $J_n$'s are. 

%%% Talk about the smoothed version and higher powers of J_0 and show that higher powers of J_0 are differentiable at 1. 

\section{Hybrid Kernels}
\subsection{Definition and Basic Properties}
The basic idea behind the hybrid kernels is to interpolate using the arc cosine kernels between the trigonometric kernel~\cite{rawat2019sampled} and the FAVOR+ kernel~\cite{performers}. The idea stems from the fact that in the two extreme data regimes, trigonometric and Favor+ kernels become deterministic. 

\begin{definition} (Hybrid Kernels)
Hybrid kernels $K(x,y)$ is defined as 
\begin{equation}
    K(x,y):= \frac{J_n(\theta)}{J_n(0)}K^{trig}(x,y) + (1-\frac{J_n(\theta)}{J_n(0)})K^{Favor+}(x,y)
\end{equation}
where $\theta$ is the angle between $x$ and $y$. 
\end{definition}
We can also replace $\frac{J_n(\theta)}{J_n(0)}$ by $\frac{J^n_{0}}{\pi^n}$ as well. Let $SM(x,y)$ denote the softmax kernel. Then,
\begin{lemma}
$\mathbb{E}(K(x,y)) = SM(x,y)$
\end{lemma}
\begin{proof}
Follows directly using the proof of lemma 1 and Theorem 1 in~\cite{orf}. 
\end{proof}
Thus these hybrid kernels are unbiased estimators of the softmax kernel.  \\

How to figure out the best weighing? 
The goal is to find the $\theta$ such that MSE($\hat{\text{K}}_{\text{trig}}) > $ MSE($\hat{\text{K}}_{\text{exp}})$ when $||x|| = ||y|| = 1$. 
\begin{proposition}
Let $||x|| = ||y|| =1.$ Then, MSE($\hat{\text{K}}_{\text{trig}}) > $ MSE($\hat{\text{K}}_{\text{exp}})$, iff $\text{cos}(\theta) < 1-\frac{1}{4}\text{log}(2e^{4}-1)$ 
\end{proposition}
\begin{proof}
 We use the MSE errors as proved in~\cite{performers}. Since $||x|| = ||y|| =1$, rewrite $x^{T}y = cos(\theta)$, $||x-y||^2 = 2 - 2\text{cos}(\theta)$ and similarly for $||x+y||^2$. The proof follows by plugging in the above relations in the MSE error formula.
\end{proof}

The proof shows that the MSE($\hat{\text{K}}_{\text{trig}}) > $ MSE($\hat{\text{K}}_{\text{exp}})$ when $\theta \in (11\pi/20, \pi)$. This gives us the justification that our weighing is optimal over all possible arc cos kernels~\cite{arccos}.
%%%Add more details. 

==> count_Sketches.tex <==
\section{Tensor sketching and its potential application to composite random feature}

\textbf{Brief summary of polynomial tensor sketching}

Given that $x, y \in \mathbb{R}^{d}$, we want to find out a random feature map $f(\cdot) : \mathbb{R}^{d} \rightarrow \mathbb{R}^{D}$ such that $\mathbb{E}[\langle f(x), f(y)\rangle] = {\langle x, y\rangle}^{p}$. When $p = 1$, we can apply count sketch to obtain random feature \cite{weinberger2009feature}. The random feature is constructed based on two 2-wise independent hash functions:
\begin{equation*}
    h(\cdot): [d] \rightarrow [D]\quad\quad s(\cdot): [d] \rightarrow \{-1, +1\}
\end{equation*}
The $k$-th dimension of random feature $f(x)$ for $x$ is defined as
\begin{equation*}
    f(x)_{k} = \sum_{i = 1}^{d}s(i)\delta\{h(i) = k\}x_{i} 
\end{equation*}

\textbf{Lemma}\quad $\mathbb{E}[\langle f(x), f(y) \rangle] = \langle x, y \rangle.$\\
Proof is provided in \cite{weinberger2009feature}. A general idea is:
\begin{align*}
    \mathbb{E}[\langle f(x), f(y) \rangle] &= \mathbb{E}_{h}[\mathbb{E}_{s}[\sum_{k = 1}^{D}\sum_{i, j = 1}^{d} s(i)s(j) \delta\{h(i) = k\}\delta\{h(j) = k\} x_{i}y_{j}]]\\
    &= \mathbb{E}_{h}[\mathbb{E}_{s}[\sum_{i, j = 1}^{d} s(i)s(j) x_{i}y_{j} \delta_{h(i)}^{T}\delta_{h(j)}]]\\
    &= \mathbb{E}_{h}[\sum_{i = 1}^{d} s(i)^{2} x_{i}y_{i} \delta_{h(i)}^{T}\delta_{h(i)}]\\
    &= \mathbb{E}_{h}[\sum_{i = 1}^{d}\sum_{k = 1}^{D}\delta\{h(i) = k\}x_{i}y_{i}]\\
    &= \sum_{i = 1}^{d}\mathbb{E}_{h}[\sum_{k = 1}^{D}\delta\{h(i) = k\}]x_{i}y_{i}\\
    &= \langle x, y\rangle
\end{align*}

Also, according to \citep{scholkopf2002learning} proposition 2.1, $\langle x^{(p)}, y^{(p)} \rangle = {\langle x, y\rangle}^{p}$, where $x^{(p)}$ denotes $p$-level tensor product and $x^{(p)} \in \mathbb{R}^{d^{p}}$. A simple case is that when $p=2$, $x^{(2)} = xx^{T}$. Therefore, if we can find a count sketch $C(x^{(p)})$ for $x^{(p)}$, then $\mathbb{E}[\langle C(x^{(p)}), C(y^{(p)}) \rangle] = {\langle x, y\rangle}^{p}$. \cite{pagh2013compressed} proposes a method to speed up the computation of the count sketch of two vectors' outer product $C(xy^{T})$. \cite{pham2013fast} generalizes the calculation to the $p$-th power when $y = x$. 

A simple case of $p = 2$ is demonstrated as an example. Given $x \in \mathbb{R}^{d}$, we leverage two different count sketches $\phi_{1}, \phi_{2}$ to obtain its random features, where $\phi_{1} = \{h_{1}, s_{1}\}$, $\phi_{2} = \{h_{2}, s_{2}\}$, and $h_{1}$, $s_{1}$, $h_{2}$, $s_{2}$ are two-wise independent. According to \cite{pagh2013compressed}, the count sketch of the outer product of two vectors can be approximated by the count sketch of the outer product of their corresponding count sketches. Consider independent and decomposable hash functions $H(\cdot): \mathbb{R}^{d\times d} \rightarrow \mathbb{R}^{D}$, and $S(\cdot): \mathbb{R}^{d\times d} \rightarrow \{-1, +1\}.$ Then we can decompose $H$ and $S$ by letting
\begin{equation*}
    H(i, j) = h_{1}(i) + h_{2}(j) \ mod\ D;\ \ S(i, j) = s_{1}(i) s_{2}(j)
\end{equation*}
Since the outer product of two different count sketches can be computed by polynomial multiplication, we can leverage FFT to reduce the computational time complexity. We represent $C_{1}(x) = [\sum_{i = 1}^{d}\delta\{h_{i} = 1\}s_{1}(i)x_{i}, ..., \sum_{i = 1}^{d}\delta\{h_{i} = D\}s_{1}(i)x_{i}]^{T} \in \mathbb{R}^{D}$ as a $D-1$ degree polynomial $P_{1}^{(x)}(\omega) = \sum_{i = 1}^{d}s_{1}(i)x_{i}\omega^{h_{1}(i)}$. Similar for $C_{2}(x)$, we can obtain a $D-1$ degree polynomial $P_{2}^{(x)}(\omega) = \sum_{i = 1}^{d}s_{2}(i)x_{i}\omega^{h_{2}(i)}$. Then the polynomial for the count sketch of $x^{(2)}$ with $\phi = {H, S}$ can be calculated as follows:
\begin{align*}
    P^{(x^{(2)})}(\omega) &= \sum_{i,j = 1}^{d} S(i, j)x_i x_j \omega^{H(i, j)}\\
    &= IFFT(FFT(P_{1}^{(x)}) \odot FFT(P_{2}^{(x)}))
\end{align*}
Then the coefficient of $P^{(x^{2})}(\omega)$ is exactly the count sketch of $x^{(2)}$. The time complexity is $\mathcal{O}(d + D\log D)$. Similar for $p$-level tensor product, we construct two 2-wise independent and decomposable hash functions $H$ and $S$ such that:
\begin{equation*}
    H(i_{1}, ..., i_{p}) = \sum_{j = 1}^{p}h_{i}(i_{j}) \ mod\ D;\ \ S(i_{1}, ..., i_{p}) = \Pi_{j = 1}^{p}s_{i}(i_{j})
\end{equation*}
Then the polynomial for the count sketch of $x^{(p)}$ with $\phi = {H, S}$ can be calculated as follows:
\begin{align*}
    P^{(x^{(p)})}(\omega) &= \sum_{i_{1},..., i_{p} = 1}^{d} S(i_{1}, ..., i_{p})\Pi_{k = 1}^{p}x_{i_{k}} \omega^{H(i_{1}, ..., i_{p})}\\
    &= IFFT(FFT(P_{i_{1}}^{(x)}) \odot ... \odot FFT(P_{i_{p}}^{(x)}))
\end{align*}
The computational time complexity is reduced from $\mathcal{O}(nd^{p})$ to $\mathcal{O}(np(d + D\log D))$.

\textbf{Relation to speed up composite random feature computation}

Instead of directly computing the composite random feature and perform dot product operation $\langle CRF(x), CRF(y) \rangle$, where $CRF(x)\in \mathbb{R}^{D_{1}\times D_{2}}$, and $D_{1}, D_{2}$ are dimensions of two different random features, we compute the count sketch of $CRF(x)$ and $CRF(y)$ as $C(CRF(x))$ and $C(CRF(y)) \in \mathbb{R}^{D}$. Since the count sketch of the outer product of the vectors can be approximated using the count sketch of the outer product of their corresponding count sketch, we compute count sketches $C_{1} (RF_1(x))$ and $C_{2} (RF_2(x))\in \mathbb{R}^{D}$, where $RF_1(x)RF_2(x)^{T} = CRF(x)$. Therefore,
\begin{align*}
    C(CRF(x)) &= C(RF_1(x)RF_2(x)^{T}) \\
    &= C( C_{1} (RF_1(x)) C_{2} (RF_2(x))^{T}) \\
    &= \text{coeff}(IFFT (FFT(P^{({RF_1(x)})}_1) \odot FFT(P^{({RF_2(x)})}_2))
\end{align*}
Then $\langle CRF(x), CRF(y) \rangle$ can be approximated by $\langle C(CRF(x), C(CRF(y) \rangle$. There is time complexity gain if we compute the dot product of composite random feature in this way. Originally, we require $\mathcal{O}(D_{1}D_{2}d)$ in order to compute the kernel approximation. Right now, we only need $\mathcal{O}(D_{1}d + D_{2}d + D\log D)$. However, an important problem is that we cannot guarantee the sketch for composite random feature is positive.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

% \url{https://arxiv.org/pdf/1609.04309.pdf}
% \url{https://papers.nips.cc/paper/7130-svd-softmax-fast-softmax-ap% proximation-on-large-vocabulary-neural-networks.pdf}
% \url{https://openreview.net/pdf?id=rkmDI85ge}
% All of the above is on softmax of word embeddings

%%%Wikitext2 Benchmark results https://arxiv.org/abs/1609.07843
To understand how close the random trigonometric features and the random positive orthogonal features approximate the softmax sampling, we evaluated it empirically on three datasets, \textbf{(a)} Penn Tree Bank, \textbf{(b)} WikiText2 and \textbf{(c)} WikiText103. 
%% Write a bit about the datasets. 
For the Penn Tree Bank dataset, we trained a $2$-layer LSTM with hidden size of $200$ and we tied the weights of the word embedding layer and the decoder layer. Thus we can treat the masked language modeling problem as minimizing the cross entropy loss between the dot product of the model output and the class embedding obtained from the embedding layer with the target word. After training, we replaced the softmax layer with the variants, \textbf{(a)} Random Trigonometric Features, \textbf{(a)} Positive Orthogonal Random Features and \textbf{(c)} Hybrid Random Features. To understand the relationship between the softmax distribution and the distribution coming from random features, we used Wasserstein metric to compute the difference between the distributions. Unlike the trigonometric or the hybrid variant, we can normalize the positive features across the classes and can treat them as probability distributions. We can easily compute the Wasserstein distance between the histograms given by the softmax sampling and the normalized positive features. However normalizing the trigonometric features yields negative probabilities.  In fact, we found examples where all the entries for a given row in our matrix is negative. (Other hack is normalize, apply ReLu and then normalize. Not sure if it is worth doing or a fair/proper comparison). So for a proper comparison, we normalized all the matrices (should we not do it?) and treated the vectors as samples from an empirical distribution. That allowed to compute the entropic regularized $2$-Wasserstein distance ~\cite{Cuturi} and the Sliced Wasserstein distance. For all the experiments, number of random features were chosen to be $64$. 

\begin{table}[h]
\begin{center}
\caption{Empirical Results comparing distributions from random features to the true softmax distribution}
\label{tab:wass}
\begin{tabular}{l c c c c} 
 \toprule
 Method &  \begin{tabular}[c]{@{}c@{}} Trigonometric Random \\ Features \end{tabular} & \begin{tabular}[c]{@{}c@{}} Positive Orthogonal\\  Random Features \end{tabular} & \begin{tabular}[c]{@{}c@{}} Hybrid Random \\ Features \end{tabular}  \\
 \midrule
 \begin{tabular}[c]{@{}c@{}} $1D$ Wasserstein Distance\\  between Histograms \end{tabular} &  N/A & $.0015 $ & N/A \\
 \begin{tabular}[c]{@{}c@{}} Entropic Regularized \\ Wasserstein Distance \end{tabular} & .0995  & .0902 & - \\
Sliced Wasserstein Distance & .0027  & .003 & - \\
 \bottomrule
\end{tabular}
\end{center}
\end{table}
%
% With the FavorPlus mechanism, the test losses for Penn Tree Bank are 9.3, 9.1, 8.7, 8.3 and the RMSE between Favorplus and the true softmax is .003, .003, .001, .0005 for 64,128, 256 and 512 features respectively. For RFF, the test losses are 9.4, 9.2, 8.8 and 8.3 respectively and the RMSE is .004, .003, .002 and .0006 for 64,128,256 and 512 features respectively and with the same features matrix. Surprisingly none of the dot products of trigonometric features is negative.

% Results for Wikitext2:
% ALL WITH UNNORMALIZED FEATURES:
% FAVORPLUS: 
% 64 random features : 11.98\\
% 128 random features: 11.08 \\
% 256 random features: 10.87 \\
% 512 random features: 10.2 \\
%% TODO Do normalized embeddings and the choose various \tau
RFF:
With 64 no negative features
64 random features: 12.01\\

\vspace{-2mm}
\small
\begin{table}[h]
    \caption{\small{NLP softmax sampling experiments.}}
    \begin{center}
    \vspace{-1mm}
    \scalebox{0.85}{
     \begin{tabular}{ c  c  c  c  c  c  c} 
    \toprule
      $\textbf{\textrm{Method}}$ & \multicolumn{2}{c}{$\textbf{\textrm{PTB}}$} & \multicolumn{2}{c}{$\textbf{\textrm{WikiText2}}$} & \multicolumn{2}{c}{$\textbf{\textrm{WikiText103}}$}\\
    
    & Test loss & RMSE & Test loss & RMSE & Test loss & RMSE\\
    \toprule
    $\textbf{\textrm{RFF (m = 64)}}$ & $9.4$ & $ .004$ & $12.01$ & & & \\ 
    $\textbf{\textrm{RFF (m = 128)}}$ & $9.2$ & $ .003$ & & & & \\ 
    $\textbf{\textrm{RFF (m = 256)}}$ & $8.8$ & $ .002$ & & & & \\ 
    $\textbf{\textrm{RFF (m = 512)}}$ & $8.3$ & $ .0006$ & & & & \\ 
    $\textbf{\textrm{Favor+ (m = 64)}}$ & $9.3$ & $ .003$ & $11.98$ & & & \\ 
    $\textbf{\textrm{Favor+ (m = 128)}}$ & $9.1$ & $ .003$ & $11.08$ & & & \\ 
    $\textbf{\textrm{Favor+ (m = 256)}}$ & $8.7$ & $ .001$ & $10.87$& & & \\ 
    $\textbf{\textrm{Favor+ (m = 512)}}$ & $8.3$ & $ .0005$ & $10.20$ & & & \\
    \bottomrule
     \end{tabular}}
\label{table:softmax_sampling}    
\end{center}
\end{table}
\normalsize

To understand why these hybrid estimators do not provide accuracy in sampling, we looked at the angles between keys and queries. The following figure~\ref{fig:hist-ptb} shows most of the angles are clustered around $\pi/2$. \\
To understand the nature of misclassifications, we calculated the average Euclidean distance between the true target embedding and the predicted target embedding. The following table shows the results for this difference between the Euclidean distances. 
\begin{figure}[h]

	\includegraphics[width=.49\columnwidth]{img/plots_arijit/Angle-Hist-PTB.png}
	\includegraphics[width=.49\columnwidth]{img/plots_arijit/Angle-Hist-wikitext2.png}
	\caption{Histogram of angles between keys and test query embeddings from our LSTM trained on Penn Tree Bank (Left) and WikiText2 (Right).}
	\label{fig:hist-ptb}
\end{figure}

\begin{figure}[h]

	\includegraphics[width=.33\columnwidth]{img/PTB_softmax_value_dist.png}
    \includegraphics[width=.33\columnwidth]{img/PTB_query_len_dist.png}
	\includegraphics[width=.33\columnwidth]{img/PTB_key_len_dist.png}
	\caption{Cumulative distribution plot about softmax values, and histogram plots for key length, query length in PTB dataset.}
	\label{ vhist2-ptb}
\end{figure}

\begin{table}[h]
    \centering
   \resizebox{\columnwidth}{!} {\begin{tabular}{cccc} 
   Number of random features  &  \begin{tabular}[c]{@{}c@{}}  Distance between predicted logits \\ 
   via regular softmax and actual targets \end{tabular} & \begin{tabular}[c]{@{}c@{}}  Distance between predicted logits \\ 
   via RFF and actual targets \end{tabular}
         & \begin{tabular}[c]{@{}c@{}}  Distance between predicted logits \\ via FAVOR and actual targets \end{tabular} \\
         \midrule
      512   &  .036  & .088 & .025 \\
      \bottomrule
    \end{tabular}
    }
    \caption{Average Euclidean Distance between predicted classes and true classes in the Penn Tree Bank}
    \label{tab:my_label}
\end{table}

%% Still need help in calculating the metrics for the full dataset. This crashes when I try to run it. I can only do 1D Wasserstein distance. 
For the Sliced Wasserstein distance, we took $60$ random projections where the dimensions are spaced evenly on a log scale in $[1,4]$. \\
The code for the numerical experiments can be found at \url{https://github.com/arijitthegame/hybrid-sampling}.
Question: Should we look at the Alias sampling~\cite{walker1977} for positive features? 


We compare the average 1D Wasserstein distance and Kolmogorov–Smirnov distance between the true softmax matrix and the approximated softmax matrix with different random feature techniques. The number of random features for FAVOR+ and RFF are $64, 128, 256, 512$. In order to maintain the same budget, we use $48, 112, 240, 496$ random features for base estimators, and $16$ for coefficient estimators. The results shown in Figure \ref{fig:PTB_1d_wass} and \ref{fig:PTB_ks} are obtained by averaging over $10$ repetitions.

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/PTB_wass_dist.png}
    \end{center} 
    \label{fig:PTB_1d_wass}
    \caption{1D Wasserstein distances with different random feature techniques for estimating softmax value matrix in PTB dataset.}
\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/PTB_KS_dist.png}
    \end{center} 
    \label{fig:PTB_ks}
    \caption{Kolmogorov–Smirnov distances with different random feature techniques for estimating softmax value matrix in PTB dataset.}
\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/PTB_KL_dist.png}
    \end{center} 
    \label{fig:PTB_ks}
    \caption{KL divergence with different random feature techniques for estimating softmax value matrix  in PTB dataset.}
\end{figure}



Results for hybrid estimators based on clustering, for two   
normalized clusters with Gaussian noise in $\R^{50}$. The mean square errors is computed by running 5 times of simulations. Here $\tau$ is the $\tau$ used in the lambda estimator expressed by
(\ref{hybrid for matrix x}) and (\ref{hybrid for matrix y}).


 




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/cluster_synthetic_dim_50_nrff_50.png}
    \end{center}
    \end{minipage}	\caption{Results for synthetic Gaussian clusters when the number of random features is 50}
\end{figure}


\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/cluster_synthetic_dim_50_nrff_150.png}
    \end{center}  \caption{Results for synthetic Gaussian clusters when the number of random features is 150}
\end{figure}




\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/new_plots/Cluster_FAVOR_PLUS_results}
    \end{center}  \caption{Results for synthetic normalized two Gaussian clusters with FAVOR+ as the base estimator}
\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/new_plots/Cluster_Trig_results.eps}
    \end{center}  \caption{Results for synthetic normalized two Gaussian clusters with Trigonometry as the base estimator}
\end{figure}


\clearpage

==> intro.tex <==
\section{Introduction}



==> proofs_MSE.tex <==
\section*{APPENDIX: Proofs for MSE of Multiple Estimators}



% $\lambda_n(x,y)=\mathbb{E}_{\omega \sim N(0,1_d)}[(\frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{x})}{2}(\mathbf{\omega}^{\top}\mathbf{x})^n)(\frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{y})}{2}(\mathbf{\omega}^{\top}\mathbf{y})^n)]$


% $\lambda_0(x,y)=\mathbb{E}_{\omega \sim N(0,1_d)}[\frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{x})}{2}  \frac{1+\mathrm{sign}(\mathbf{\omega}^{\top}\mathbf{y})}{2}]$


% let $ u_i \sim N(0,1_d),  v_i \sim N(0,1_d), \omega_i \sim N(0,1_d)$ chosen independently

% $\hat{\lambda}_0(x,y)=\frac{1}{r}\sum_{i=1}^{r}\xi_{\lambda}(\mathbf{x},\omega_i)\xi_{\lambda}(\mathbf{y},\omega_i) $

% where $\xi_{\lambda}(\mathbf{x},\omega^1_i)=\frac{1+\mathrm{sign}(\mathbf{\omega_i}^{\top}\mathbf{x})}{2}$

% $\mathbb{E}[\hat{\lambda}_0(x,y)]=\mathbb{E}[\frac{1+\mathrm{sign}(\mathbf{\omega_i}^{\top}\mathbf{x})}{2}\frac{1+\mathrm{sign}(\mathbf{\omega_i}^{\top}\mathbf{y})}{2}]=\frac{1}{4}+$


% $\mathbb{E}[\hat{\lambda}_0(x,y)^2]=$




% $\phi_m^{1,++}(\mathbf{x})=\frac{1}{\sqrt{2}}\exp(-\frac{\|\mathbf{x} \|^{2}}{2})\exp({\mathbf{u}}^{\top}\mathbf{x}),   \phi_m^{2,++}(\mathbf{x})=\frac{1}{\sqrt{2}}\exp(-\frac{\|\mathbf{x} \|^{2}}{2})\exp({-\mathbf{u}}^{\top}\mathbf{x})$

% $\phi_m^{1,\mathrm{trig}}(\mathbf{x})=\exp(\frac{\|\mathbf{x} \|^{2}}{2})\sin({\mathbf{v}}^{\top}\mathbf{x}),   \phi_m^{2,\mathrm{trig}}(\mathbf{x})=\frac{1}{\sqrt{2}}\exp(-\frac{\|\mathbf{x} \|^{2}}{2})\cos({\mathbf{v}}^{\top}\mathbf{x})$



% \begin{align}
% \begin{split}
% \widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})=\widehat{\lambda}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y}) + (1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y}) \\
% = (\frac{1}{r}\sum_{i=1}^r \xi_{\lambda}(\mathbf{x},\omega_i)\xi_{\lambda}(\mathbf{y},\omega_i))(\frac{1}{m}\sum_{j=1}^2 \sum_{k=1}^m \phi_{m,k}^{j,++}(\mathbf{x})\phi_{m,k}^{j,++}(\mathbf{y}))  \\ + (1 - \frac{1}{r}\sum_{i=1}^r \xi_{\lambda}(\mathbf{x},\omega_i)\xi_{\lambda}(\mathbf{y},\omega_i))(\frac{1}{m}\sum_{j=1}^2 \sum_{k=1}^m \phi_{m,k}^{j,\mathrm{trig}}(\mathbf{x})\phi_{m,k}^{j,\mathrm{trig}}(\mathbf{y})) \\
% = \frac{1}{mr}\sum_{i=1}^{r}\sum_{k=1}^{m}(\xi_{\lambda}(\mathbf{x},\omega_i)\phi_{m,k}^{1,++}(\mathbf{x})\xi_{\lambda}(\mathbf{y},\omega_i)\phi_{m,k}^{1,++}(\mathbf{y})+\xi_{\lambda}(\mathbf{x},\omega_i)\phi_{m,k}^{2,++}(\mathbf{x})\xi_{\lambda}(\mathbf{y},\omega_i)\phi_{m,k}^{2,++}(\mathbf{y})) \\
% + 
% \end{split}
% \end{align}


In the following subsections, $k$ represents the number of samples we use to estimate $\hat{\lambda}(\mathbf{x},\mathbf{y})$. $m_1$ and $m_2$ are the number of samples we use to estimate $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$ respectively.


\subsection{Lambda-Angular Hybrid Estimator}


\begin{equation}
\lambda(\theta) = \frac{\theta}{\pi} = 
\frac{1}{2} - \frac{1}{2}\mathbb{E}[(\phi_{n}^{\mathrm{ang}}(\mathbf{x}))^{\top}\phi_{n}^{\mathrm{ang}}(\mathbf{y})]
\end{equation}

\begin{equation}
\hat{\lambda}(\theta) =
\frac{1}{2} - \frac{1}{2k}\sum_{i=1}^k \mathrm{sgn}(\tau_{i}^{\top}\mathbf{x})\mathrm{sgn}(\tau_{i}^{\top}\mathbf{y})
\end{equation}


Thus we can construct random feature maps for $\widehat{\lambda}_{k}(\mathbf{x},\mathbf{y}) = a - (\phi_{k}^{\lambda}(\mathbf{x}))^{\top}
\phi_{k}^{\lambda}(\mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = \frac{1}{2} \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{2k}}(\mathrm{sgn}(\tau_{1}^{\top}\mathbf{z}),...,\mathrm{sgn}(\tau_{n}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{k} \sim \mathcal{N}(0,\mathbf{I}_{d})$.


To calculate the MSE, we have:

\begin{align}
\begin{split}
\mathrm{Var}[\hat{\lambda}(\theta)]=\mathrm{Var}[\frac{1}{2} - \hat{\lambda}(\theta)]=\mathrm{Var}[\frac{1}{2k}\sum_{i=1}^k\mathrm{sgn}(\tau_{i}^{\top}\mathbf{x})\mathrm{sgn}(\tau_{i}^{\top}\mathbf{y})] 
=\frac{1}{4k}\mathrm{Var}[\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y})]\\
=\frac{1}{4k}(\mathbb{E}[(\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y}))^2] - \mathbb{E}[\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y})]^2) 
= \frac{1}{4k}(1 - (1-
\frac{2\theta}{\pi})^2) 
=\frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})]
\end{split}
\end{align}


\begin{align}
\begin{split}
\mathrm{E}[\hat{\lambda}(\theta)^2] = Var[\hat{\lambda}] + \mathrm{E}[\hat{\lambda}(\theta)]^2 = \frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] + \frac{\theta^2}{\pi^2} 
\end{split}
\end{align}


\begin{align}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\theta))^2] = 1-2\mathrm{E}[\hat{\lambda}(\theta)] + \mathrm{E}[\hat{\lambda}(\theta)^2] = 1 - \frac{2\theta}{\pi} + \frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] + \frac{\theta^2}{\pi^2}
 = (1-\frac{\theta}{\pi})^2 +\frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] 
\end{split}
\end{align}



\begin{align}
\begin{split}
\mathrm{E}[\hat{\lambda}(\theta)(1-\hat{\lambda}(\theta))] = \mathrm{E}[\hat{\lambda}(\theta)] - \mathrm{E}[\hat{\lambda}(\theta)^2] = \frac{\theta}{\pi} - (\frac{1}{k}[\frac{\theta}{\pi}(1-\frac{\theta}{\pi})] + \frac{\theta^2}{\pi^2} ) = \frac{\theta}{\pi}(1-\frac{\theta}{\pi})(1-\frac{1}{k})
\end{split}
\end{align}


If we generate $\omega_i$ independently for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
= [\frac{\theta^2}{\pi^2}+ \frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y}))  +  [(1-\frac{\theta}{\pi})^2 +\frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{split}
\end{align}


with $\|x\|^2=\|y\|^2=r^2$:

\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)) \\
= [\frac{\theta^2}{\pi^2}+ \frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r))  +  [(1-\frac{\theta}{\pi})^2 +\frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{split}
\end{align}


If we use exactly the same $\omega_i$ for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))\\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]\\
= [\frac{\theta^2}{\pi^2}+ \frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y}))  +  [(1-\frac{\theta}{\pi})^2 +\frac{1}{k}(\frac{\theta}{\pi}(1-\frac{\theta}{\pi}))]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\frac{\theta}{\pi}(1-\frac{\theta}{\pi})(1-\frac{1}{k})
\end{split}
\end{align}



$\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r))$ will remain the same when $\|x\|^2=\|y\|^2=r^2$ since $\cos(\|x\|_2^2-\|y\|_2^2)=1$.





\subsection{Arc-cosine Kernel with $n\geq1$}

We could derive MSE for arccosine kernel with $n\geq1$ if we could calculate the following expectation:
 $\mathbb{E}_{\tau \sim N(0,1_d)}[\mathrm{sgn}(\tau^{\top}\mathbf{x})\mathrm{sgn}(\tau^{\top}\mathbf{y})(\tau^{\top}\mathbf{x})^{2n}(\tau^{\top}\mathbf{y})^{2n}]$, where $n\in N^{+}$ .
 
 
 
\subsection{Gaussian Hybrid Estimator}
 
\begin{equation}
\lambda(\mathbf{x},\mathbf{y}) = 1- \exp(-\frac{\lambda^2}{2}\|\mathbf{x-y}\|^{2}) = 1- \mathbb{E}[\cos(\lambda \omega^{\top}(\mathbf{x-y}))]
\end{equation}

\begin{equation}
\hat{\lambda}(\mathbf{x},\mathbf{y}) = 1- \frac{1}{k}\sum_{i=1}^k \cos(\lambda (\omega_i^{\top}(\mathbf{x}-\mathbf{y})))
\end{equation}



Thus we can construct random feature maps for $\widehat{\lambda}_{k}(\mathbf{x},\mathbf{y}) = a - (\phi_{k}^{\lambda}(\mathbf{x}))^{\top}
\phi_{k}^{\lambda}(\mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = 1 \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{k}}(\sin(\tau_{1}^{\top}\mathbf{z}), \cos(\tau_{1}^{\top}\mathbf{z}),...,\sin(\tau_{k}^{\top}\mathbf{z}), \cos(\tau_{k}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{k} \sim \mathcal{N}(0,\mathbf{I}_{d})$.


To calculate the MSE, we have:



Using the fact that (see: Lemma 1 in \cite{yu2016ORF}):

\begin{equation}
\mathrm{Var}[\cos(\lambda\omega^{\top}\Delta)] = \frac{1}{2}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{equation}

\begin{equation}
\mathrm{E}[\cos(\lambda\omega^{\top}\Delta)] = \exp(-\frac{\lambda^2}{2}\|\Delta\|^2)
\end{equation}

Then we could derive:

\begin{equation}
\begin{split}
\mathrm{E}[\cos(\lambda\omega^{\top}\Delta)^2] = \mathrm{Var}[\cos(\lambda\omega^{\top}\Delta)] + \mathrm{E}[\cos(\lambda\omega^{\top}\Delta)]^2   = \frac{1}{2}(1-\exp(-\lambda^2\|\Delta\|^2))^2 + \exp(-\frac{\lambda^2}{2}\|\Delta\|^2)^2
\\ = \frac{1}{2} + \frac{1}{2}\exp(-2\lambda^2\|\Delta\|^2) -\exp(-\lambda^2\|\Delta\|^2) + \exp(-\lambda^2\|\Delta\|^2) 
= \frac{1}{2}(1+\exp(-2\lambda^2\|\Delta\|^2))
\end{split}
\end{equation}


Therefore, 

\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \mathrm{E}[(\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega_i^{\top}\Delta))^2] = 
\frac{1}{k}\mathrm{E}[\cos(\lambda \omega^{\top}\Delta)^2] + (1-\frac{1}{k})\mathrm{E}[\cos(\lambda \omega^{\top}\Delta)]^2 \\= 
 \frac{1}{2k}(1+\exp(-2\lambda^2\|\Delta\|^2)) + (1-\frac{1}{k})\exp(-\lambda^2\|\Delta\|^2) \\
 = \exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1+\exp(-2\lambda^2\|\Delta\|^2)-2\exp(-\lambda^2\|\Delta\|^2)) \\
 = \exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}




\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})^2] = 1-2\mathrm{E}[1-\hat{\lambda}(\mathbf{x},\mathbf{y})] + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] 
= 1 - 2\mathrm{E}[\cos(\lambda\omega^{\top}\Delta)] + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= 1 - 2 \exp(-\frac{\lambda^2}{2}\|\Delta\|^2) +  \exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= (1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}



\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))] = \mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})] - \mathrm{E}[(\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\ 
= 1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}) - (1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 - \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}))-\frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 
\end{split}
\end{equation}


For $\|x\|_2^2=\|y\|_2^2=r^2$, we could rewrite as:

\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{r},\mathbf{\theta}))^2] 
 = \exp(-4\lambda^2 r^2 \sin(\frac{\theta}{2})^2) + \frac{1}{2k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}


\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{r},\mathbf{\theta})^2] 
= (1-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}




If we generate $\omega_i$ independently for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
= [(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{split}
\end{align}





\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)) \\
=  [(1-\exp(-2\lambda^2r^2\sin(\frac{\theta}{2})^2))^2 + \frac{1}{2k}(1-\exp(-4\lambda^2r^2\sin(\frac{\theta}{2})^2))^2]   \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) \\ +      [\exp(-4\lambda^2r^2\sin(\frac{\theta}{2})^2) + \frac{1}{2k}(1-\exp(-4\lambda^2r^2\sin(\frac{\theta}{2})^2))^2] \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{split}
\end{align}




If we use exactly the same $\omega_i$ for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))\\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]\\
= [(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
-\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))[\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}))-\frac{1}{2k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]
\end{split}
\end{align}





If we do not have the condition $\|x\|^2=\|y\|^2=r^2$, the MSE of gaussian hybrid estimator will be positive (rather than equal to zero) at $\theta=\pi$. This might be problematic since $\lambda(\mathbf{x}, \mathbf{y})$ is a very small positive number at $\theta=\pi$.





\subsection{Truncated Gaussian Hybrid Estimator}

If we have the condition $\|x\|^2=\|y\|^2=r^2$, we could propose a truncated version of the gaussian hybrid estimator, which will satisfy ${\lambda}(\mathbf{x},\mathbf{y})=0$ at $\theta=0$, and ${\lambda}(\mathbf{x},\mathbf{y})=1$ at $\theta=\pi$.

\begin{equation}
\lambda(\mathbf{x},\mathbf{y}) = \frac{1-\exp(-\frac{\lambda^2}{2}\|\mathbf{x-y}\|^{2})}{1-\exp(-2\lambda^2r^2)} = \frac{1-\exp(-2\lambda^2r^2\sin(\frac{\theta}{2})^2)}{1-\exp(-2\lambda^2r^2)}
\end{equation}

Take $\gamma=1-\exp(-2\lambda^2r^2)$, we have:

\begin{equation}
\lambda(\mathbf{x},\mathbf{y}) = \frac{1-\exp(-\frac{\lambda^2}{2}\|\mathbf{x-y}\|^{2})}{\gamma} \\ 
= \frac{1- \mathbb{E}[\cos(\lambda \omega^{\top}(\mathbf{x-y}))]}{\gamma}
\end{equation}


\begin{equation}
\hat{\lambda}(\mathbf{x},\mathbf{y}) = \frac{1}{\gamma} - \frac{1}{k\gamma}\sum_{i=1}^k \cos(\lambda (\omega_i^{\top}(\mathbf{x}-\mathbf{y})))
\end{equation}



Thus we can construct random feature maps for $\widehat{\lambda}_{k}(\mathbf{x},\mathbf{y}) = a - (\phi_{k}^{\lambda}(\mathbf{x}))^{\top}
\phi_{k}^{\lambda}(\mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = \frac{1}{\gamma} \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{k\gamma}}(\sin(\tau_{1}^{\top}\mathbf{z}), \cos(\tau_{1}^{\top}\mathbf{z}),...,\sin(\tau_{k}^{\top}\mathbf{z}), \cos(\tau_{k}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{k} \sim \mathcal{N}(0,\mathbf{I}_{d})$.


To calculate the MSE, we have:


\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \frac{1}{\gamma^2} \mathrm{E}[(\gamma-1+\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\ 
= \frac{1}{\gamma^2} \mathrm{E}[ (\gamma-1)^2 + 2(\gamma-1)(\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y}))) + (\frac{1}{k}\sum_{i=1}^k \cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y})))^2 ] \\
=\frac{(1-\gamma)^2}{\gamma^2}+\frac{2(\gamma-1)}{\gamma^2}\mathrm{E}[\cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y}))]+\frac{1}{\gamma^2}\mathrm{E}[(\frac{1}{k}\sum_{i=1}^k\cos(\lambda \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\
= \frac{(1-\gamma)^2}{\gamma^2}+\frac{2(\gamma-1)}{\gamma^2}\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})+\frac{1}{\gamma^2}\exp(-\lambda^2\|\Delta\|^2) + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= \frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}



\begin{equation}
\begin{split}
\mathrm{E}[(\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] = 1-2\mathrm{E}[1-\hat{\lambda}(\mathbf{x},\mathbf{y})] + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] 
= -1 + \frac{2}{\gamma}- \frac{2}{\gamma}\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}) + \mathrm{E}[(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= -1 + \frac{2}{\gamma}- \frac{2}{\gamma}\exp(-\frac{\lambda^2}{2}\|\Delta\|^{2}) + \frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 \\
= \frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2
\end{split}
\end{equation}



\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})(1-\hat{\lambda}(\mathbf{x},\mathbf{y}))] = \mathrm{E}[\hat{\lambda}(\mathbf{x},\mathbf{y})] - \mathrm{E}[(\hat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\ 
= \frac{1}{\gamma}(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})) - \frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 - \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 
\end{split}
\end{equation}




For $\|x\|_2^2=\|y\|_2^2=r^2$, we could rewrite as:

\begin{equation}
\begin{split}
\mathrm{E}[(1-\hat{\lambda}(\mathbf{r},\mathbf{\theta}))^2] 
 = \frac{1}{\gamma^2}((1-\gamma)-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}


\begin{equation}
\begin{split}
\mathrm{E}[\hat{\lambda}(\mathbf{r},\mathbf{\theta})^2] 
= \frac{1}{\gamma^2}(1-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{split}
\end{equation}


This truncated version with be the same as the vanilla version if $\gamma=1$.




If we generate $\omega_i$ independently for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\
= [\frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{split}
\end{align}





\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)) \\
=  [\frac{1}{\gamma^2}(1-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2]   \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) \\ +      [\frac{1}{\gamma^2}((1-\gamma)-\exp(-2\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-4\lambda^2r^2 \sin(\frac{\theta}{2})^2))^2] \mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{split}
\end{align}




If we use exactly the same $\omega_i$ for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m_1}(\mathbf{x},\mathbf{y})$ and  $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m_2}(\mathbf{x},\mathbf{y})$:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))\\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]\\
= [\frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) \\ +  [\frac{1}{\gamma^2}((1-\gamma)-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) 
-\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})* \\
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))  [\frac{1}{\gamma}(1- \exp(-\frac{\lambda^2}{2}\|\Delta\|^{2})) - \frac{1}{\gamma^2}(1-\exp(-\frac{\lambda^2}{2}\|\Delta\|^2))^2 - \frac{1}{2\gamma^2 k}(1-\exp(-\lambda^2\|\Delta\|^2))^2 ]
\end{split}
\end{align}






\subsection{Product Hybrid Estimator}

We could rewrite the softmax kernel as product of $\mathrm{SM}^{++}(\mathbf{x},\mathbf{y})$ and $\mathrm{SM}^{\mathrm{trig}}(\mathbf{x},\mathbf{y})$:

\begin{equation}
\exp(2\mathbf{x}^{\top} \mathbf{y}) = \exp(-\frac{\|\mathbf{x}-\mathbf{y}\|^2}{2})\exp(\frac{\|\mathbf{x}+\mathbf{y}\|^2}{2}) = \mathrm{E}[\cos(\omega^{\top}\Delta)]\mathrm{E}[\frac{\exp(\omega^{\top}\mathbf{z})+\exp(-\omega^{\top}\mathbf{z})}{2}] 
\end{equation}


Define:
\begin{equation}
\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\mathbf{x},\mathbf{y}) = \frac{1}{m_1}\sum_{i=1}^{m_1} \cos(\omega_i^{\top}\Delta)
\end{equation}

\begin{equation}
\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\mathbf{x},\mathbf{y}) = \frac{1}{2 m_2}\sum_{j=1}^{m_2} (\exp(\omega_j^{\top}\mathbf{z})+\exp(-\omega_j^{\top}\mathbf{z}))
\end{equation}

Then our hybrid estimator could be defined as:
\begin{equation}
\widehat{\mathrm{SM}}_{m_1,m_2}^{\mathrm{hyb}}(\mathbf{x},\mathbf{y}) = \widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})
\end{equation}

Next, the variance of these two estimators are:

\begin{equation}
\mathrm{Var}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\mathbf{x},\mathbf{y})] = \frac{1}{2 m_1}(1-\exp(-\|\Delta\|^2))^2
\end{equation}

\begin{equation}
\mathrm{Var}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\mathbf{x},\mathbf{y})] = \frac{1}{2 m_2}(\exp(\|\mathbf{z}\|^2)-1)^2
\end{equation}


We could then calculate the MSE of this hybrid estimator:


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m_1, m_2}(\mathbf{x},\mathbf{y})) 
= \mathrm{Var}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]\mathrm{Var}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})] \\
+ \mathrm{Var}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]\mathrm{E}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]^2 + \mathrm{Var}[\widehat{\mathrm{SM}}_{m_2}^{\mathrm{++}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]\mathrm{E}[\widehat{\mathrm{SM}}_{m_1}^{\mathrm{trig}}(\frac{\mathbf{x}}{\sqrt{2}},\frac{\mathbf{y}}{\sqrt{2}})]^2 \\
= \frac{1}{4 m_1 m_2}(1-\exp(-\frac{\|\Delta\|^2}{2}))^2(\exp(\frac{\|\mathbf{z}\|^2}{2})-1)^2 \\
+ \frac{1}{2 m_1}(1-\exp(-\frac{\|\Delta\|^2}{2}))^2\exp(\frac{\|\mathbf{z}\|^2}{2}) + \frac{1}{2 m_2}(\exp(\frac{\|\mathbf{z}\|^2}{2})-1)^2\exp(-\frac{\|\Delta\|^2}{2})
\end{split}
\end{align}


\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m_1, m_2}(r,\mathbf{\theta})) 
= \frac{1}{4 m_1 m_2}(1-\exp(-2r^2\sin(\frac{\theta}{2})^2))^2(1-\exp(2r^2\cos(\frac{\theta}{2})^2))^2 \\
+ \frac{1}{2 m_1}(1-\exp(-2r^2\sin(\frac{\theta}{2})^2))^2\exp(2r^2\cos(\frac{\theta}{2})^2) + \frac{1}{2 m_2}(1-\exp(2r^2\cos(\frac{\theta}{2})^2))^2\exp(-2r^2\sin(\frac{\theta}{2})^2)
\end{split}
\end{align}








\newpage


\subsection{Lambda Hybrid Estimator}

If the input matrices $\mathbf{Q}, \mathbf{K}$ can be clustered into $n_q$ and $n_k$ groups respectively (using k-means clustering algorithm for example), with the center point of each group as $\mathbf{r}_i$, ($i=1,...,n_k$) and $\mathbf{r}_j$, ($j=1,...,n_q$), then there exist $n_q n_k$ pairs of $(\mathbf{r}_i, \mathbf{r}_j)$, ($i=1,...,n_q, j=1,...,n_k$), so we can construct $n_q n_k$ softmax estimators to estimate cross-group softmax values. \textcolor{red}{In the next subsection, we use $\mathbf{x}$ and $\mathbf{y}$ to represent a pair of such centers $\mathbf{r}_i$ and $\mathbf{r}_j$}.


\subsubsection{Construction for matrix $\mathbf{A}$}

Consider $\mathbf{z} = \mathbf{Ax} + \mathbf{(A^{\top})^{-1}y}$ for an invertible (in $\mathbb{C}^{d \times d})$ matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$, an estimator based on this mechanism has variance equal to $0$ if:
\begin{equation}
\label{eq:z_ax_by_0}
\mathbf{z} = \mathbf{Ax} + \mathbf{(A^{\top})^{-1}y} = 0
\end{equation}

We assume here that $\mathbf{A}$ is a diagonal matrix, so $\mathbf{A}=\mathbf{A^{\top}}$. Then we can rewrite the above equation as:
\begin{equation}
\mathbf{z} = \mathbf{Ax} + \mathbf{(A)^{-1}y} = 0
\end{equation}

Since position $(k,k)$ in matrix $\mathbf{A}$ has the form $\alpha_k + \beta_k i$, we need to satisfy the following equation for each k=1,...,d:
\begin{equation}
(\alpha_k + \beta_k i)x_k + \frac{1}{\alpha_k + \beta_k i}y_k = 0
\end{equation}

\begin{equation}
(\alpha_k + \beta_k i)x_k + \frac{\alpha_k - \beta_k i}{\alpha_k^2 + \beta_k^2 }y_k = 0
\end{equation}

We can simplify this equation and separate into real and imaginary part:
\begin{equation}
\left\{ \begin{array}{rcl}
\mathbf{Re}: (\alpha_k^2+\beta_k^2)\alpha_k x_k + \alpha_k y_k = 0 \\ 
\mathbf{Im}: (\alpha_k^2+\beta_k^2)\beta_k x_k - \beta_k y_k = 0 \\ 
\end{array}\right.
\end{equation}

Our goal now is to choose values for $\alpha_k$ and $\beta_k$ given $x_k$ and $y_k$.

If $x_k y_k>0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=0 \\ 
\beta_k=\sqrt{y_k/x_k} \\ 
\end{array}\right.
\end{equation}

And if $x_k y_k<0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=\sqrt{-y_k/x_k} \\ 
\beta_k= 0\\ 
\end{array}\right.
\end{equation}


When $x_k=y_k=0$,  we could assume $\alpha_k=\beta_k=1$. However, if $x_k=0, y_k\neq 0$ or $x_k\neq 0, y_k=0$, then we cannot satisfy the above equation perfectly. We could assume $\alpha_k$ to some large positive value and set $\beta_k=0$ if  $x_k=0, y_k\neq 0$. And assume $\alpha_k=\beta_k$ to be some small positive value close to zero if $x_k\neq 0, y_k=0$.


Now suppose 
$\mathbf{A} = \mathrm{diag}(a_1,\cdots,a_d) \in \R^{d \times d}$, then maybe we cannot make
$\mathbf{Ax} + \mathbf{(A)^{-1}y} = 0$. However, we can still    minimize $\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|
= \sqrt{\sum_{k=1}^d (a_k x_k + \frac{1}{a_k}y_k)^2}$ by taking

\begin{equation}
 a_k = \sqrt{\left|
\frac{y_k}{x_k}
\right|} 
\end{equation}

if $x_k \neq 0$. If $x_k = 0$, we could set $a_k$ to some large positive value.




\subsubsection{Construction for Softmax Estimator}

From equation (16):
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{Ax}\|^{2}}{2})  
\mathrm{exp}(\frac{\|\mathbf{A}^{-1}\mathbf{y}\|^{2}}{2})\mathrm{SM}(\mathbf{x},\mathbf{y})  
= \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{Ax}+\mathbf{A}^{-1}\mathbf{y})]
\end{equation}


The softmax can be estimated as:

\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{\mathbf{A}^{-1}}(\mathbf{y})]
\end{equation}

where

\begin{equation}
\Psi^{m}_{\mathbf{A}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{Ax}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{Ax}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Ax}))^{\top}
\end{equation}

\begin{equation}
\Psi^{m}_{\mathbf{A^{-1}}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A^{-1}y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A^{-1}y}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A^{-1}y}))^{\top}
\end{equation}

for $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$.

And such softmax estimator will have variance of zero if $\mathbf{x}=\mathbf{r}_x$ and $\mathbf{y}=\mathbf{r}_y$, where $\mathbf{r}_x$ and $\mathbf{r}_y$ are the centes vector $\mathbf{x}$ and $\mathbf{y}$ belong to respectively. For other pairs of vectors close to $\mathbf{r}_x$ and $\mathbf{r}_y$, the variance should be small.  


\subsubsection{Construction for Lambda Coefficients}
\begin{align}
\begin{split}
\mathrm{exp}(-\frac{\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|^{2}}{2\tau^2}) = 
\mathrm{exp}(-\frac{\|\mathbf{Ax}\|^2 + \|\mathbf{(A)^{-1}y}\|^{2} + 2 (\mathbf{Ax})^{\top}(\mathbf{(A)^{-1}y})}{2\tau^2}) \\
= \mathrm{exp}(-\frac{\|\mathbf{Ax}\|^{2}}{2\tau^2})\mathrm{exp}(-\frac{\|\mathbf{(A)^{-1}y}\|^{2}}{2\tau^2})\mathrm{exp}(\frac{\mathbf{x}^{\top}(\mathbf{-y})}{\tau^2})
\end{split}
\end{align}

where $\mathrm{exp}(\frac{\mathbf{x}^{\top}(\mathbf{-y})}{\tau^2}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}}(\mathbf{x}/\tau)^{\top} 
\Psi^{m}_{\mathbf{A}^{-1}}(\mathbf{-y}/\tau)]$

and $\Psi^{m}_{\mathbf{A}}(\mathbf{z}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{Mz}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{Mz}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Mz}))^{\top}$ and $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$, for $\mathbf{z}=\{\frac{\mathbf{x}}{\tau}, \frac{\mathbf{-y}}{\tau}$\}.


we can put it together and derive:
\begin{align}
\begin{split}
\mathrm{exp}(-\frac{\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|^{2}}{2\tau^2}) = \mathbb{E}[\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{\tau, m}_{\mathbf{A}^{-1}}(\mathbf{-y})]
\end{split}
\end{align}

where
\begin{equation}
\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{Ax}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{Ax}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Ax}/\tau))^{\top}
\end{equation}
\begin{equation}
\Psi^{\tau, m}_{\mathbf{A^{-1}}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|\mathbf{(A^{-1}y)}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}\mathbf{A^{-1}\mathbf{y}}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}\mathbf{A^{-1}\mathbf{y}}/\tau))^{\top}
\end{equation}


Recall from (\ref{exp - norm cos}) that
\begin{equation} 
\mathrm{exp}(-\frac{\|\mathbf{x}-\mathbf{y}\|^{2}}{2}) = \mathbb{E}[\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))],   
\end{equation}
we can derive


\begin{align}
\begin{split}
\mathrm{exp}(-\frac{\|\mathbf{Ax} + \mathbf{(A)^{-1}y}\|^{2}}{2\tau^2}) = \mathbb{E}[\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{\tau, m}_{\mathbf{A}^{-1}}(\mathbf{-y})]
\end{split}
\end{align}

where
\begin{equation} \label{hybrid for matrix x}
\Psi^{\tau, m}_{\mathbf{A}}(\mathbf{x}) =     
\sqrt{\frac{1}{m}}
(\sin(\omega_{1}^{\top}\mathbf{Ax}/\tau),
\cos(\omega_{1}^{\top}\mathbf{Ax}/\tau),
...,
\sin(\omega_{m}^{\top}\mathbf{Ax}/\tau),
\cos(\omega_{m}^{\top}\mathbf{Ax}/\tau)
)^{\top}
\end{equation}

\begin{equation} \label{hybrid for matrix y}
\Psi^{\tau, m}_{\mathbf{A^{-1}}}(\mathbf{y}) =   
\sqrt{\frac{1}{m}}  
(\sin(-\omega_{1}^{\top}\mathbf{A^{-1}y}/\tau),
\cos(-\omega_{1}^{\top}\mathbf{A^{-1}y}/\tau),
...,
\sin(-\omega_{m}^{\top}\mathbf{A^{-1}y}/\tau),
\cos(-\omega_{m}^{\top}\mathbf{A^{-1}y}/\tau)
)^{\top}
\end{equation}

\subsubsection{Multiple Softmax Estimators}

We assume here that we need $p=n_q n_k$ softmax estimators, with $n_q, n_k$ defined at the beginning of this section. Then as stated in Section 1.5, we denote $\mathcal{E}=( \widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of the softmax-kernel $\mathrm{SM}^{i,j}(\mathbf{x},\mathbf{y})$ and $\Lambda = \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of $\lambda^{i,j}(\mathbf{x},\mathbf{y})$ for some functions $\lambda^{i,j}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, constructed independently from $\mathcal{E}$.

Then our hybrid estimator takes the following:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y})
\end{equation}

with constraint:

\begin{equation}
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) = 1
\end{equation}


If we define $\mathbf{A}^{i,j}$ as the composite matrix satisfies Eq. \ref{eq:z_ax_by_0} with $\mathbf{x}, \mathbf{y}$ replaced by center $\mathbf{r}_i, \mathbf{r}_j$ from $\mathbf{Q}$ and $\mathbf{K}$, then:

\begin{equation}
\widehat{\lambda}^{i,j}(\mathbf{x}, \mathbf{y}) = \Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} \Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) 
\end{equation}

with $\Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y})$ given by:


\begin{equation}
\Psi^{\tau, m}_{\mathbf{A}^{i,j}} (\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j} \mathbf{x}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau))^{\top}
\end{equation}

\begin{equation}
\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau))^{\top}
\end{equation}



\begin{equation}
\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top}\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})
\end{equation}

with $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})$ given by:

\begin{equation}
\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j}\mathbf{x}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j}\mathbf{x}))^{\top}
\end{equation}

\begin{equation}
\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}),...,\mathrm{exp}(\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}))^{\top}
\end{equation}




% \subsubsection{Multiple Softmax Estimators}

% we assume here that we need $p+1={n \choose 2}+1$ softmax estimators, with the fist ${n \choose 2}$ estimators generated with of $(\mathbf{r}_i,\mathbf{r}_j)$, ($i\neq j \in 1, ..., n$), and the last one as tri-geometric softmax estimator.


% As stated in Section 1.5, we denote $\mathcal{E}=( \asm )_{k=1}^{p+1}$ as a list of estimators of the softmax-kernel $\sm$ and $\Lambda = ( \alamgen )_{k=1}^{p}$ as a list of estimators of: 
% $\{\lambda^{k}(\mathbf{x},\mathbf{y})\}_{k=1}^{p}$ for some functions
% $\lambda^{k}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, constructed independently from $\mathcal{E}$.

% Then our hybrid
% Take the following estimator of $\sm$:
% \begin{equation}
% \widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
% \sum_{k=1}^{p} \alamgen \asm + \left(1-\sum_{k=1}^{p} \alamgen \right)\widehat{\mathrm{SM}}^{p+1}(\mathbf{x},\mathbf{y})
% \end{equation}

% where 
% \begin{equation}
% \hat{\lambda}^k(\mathbf{x}, \mathbf{y}) = \Psi^{\tau, m}_{\mathbf{A_k}}(\mathbf{x})^{\top} \Psi^{\tau, m}_{\mathbf{A_k^{-1}}}(\mathbf{-y}) 
% \end{equation}

% with $\Psi^{\tau, m}_{\mathbf{A_k}}(\mathbf{x})$ and $\Psi^{\tau, m}_{\mathbf{A_k^{-1}}}(\mathbf{-y})$ given by:


% \begin{equation}
% \Psi^{\tau, m}_{\mathbf{A}_k}(\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{A_k x}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{A_k x}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A_k x}/\tau))^{\top}
% \end{equation}
% \begin{equation}
% \Psi^{\tau, m}_{\mathbf{A_k^{-1}}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|\mathbf{(A^{-1}_k y)}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}\mathbf{A^{-1}_k \mathbf{y}}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}\mathbf{A^{-1}_k \mathbf{y}}/\tau))^{\top}
% \end{equation}


% and $\mathbf{A}_k$ constructed from $(\mathbf{r}_i,\mathbf{r}_j)$, ($i\neq j \in 1, ..., n$) as stated in subsection 2.6.1.

% \begin{equation}
% \widehat{\mathrm{SM}}^{\mathrm{k}}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}_k}(\mathbf{x})^{\top}\Psi^{m}_{\mathbf{A^{-1}}_k}(\mathbf{y})
% \end{equation}

% with $\Psi^{m}_{\mathbf{A}_k}(\mathbf{x})$ and $\Psi^{m}_{\mathbf{A^{-1}}_k}(\mathbf{y})$ given by:

% \begin{equation}
% \Psi^{m}_{\mathbf{A_k}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A_k x}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A_k x}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A_k x}))^{\top}
% \end{equation}

% \begin{equation}
% \Psi^{m}_{\mathbf{A_k^{-1}}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A_k^{-1}y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A_k^{-1}y}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A_k^{-1}y}))^{\top}
% \end{equation}


% and the last softmax estimator is just the tri-geometric estimator:
% \begin{equation}
% \widehat{\mathrm{SM}}^{p+1}(\mathbf{x},\mathbf{y}) = \widehat{\mathrm{SM}}^{\mathrm{trig}}_m(\mathbf{x},\mathbf{y})
% \end{equation}






\newpage


\newpage


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1 d=64 m=128 unmodified.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1 d=64 m=16384 unmodified.png}}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Angular r=1, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Gaussian r=1, d=64 sigma=4.png}
    \end{center}
    \end{minipage}
\end{figure}



\newpage


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.25 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.25 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep16 ERR Angular r=1.25, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep16 ERR Gaussian r=1.25, d=64 sigma=4.png}
    \end{center}
    \end{minipage}
\end{figure}




\newpage




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.5 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep17 ERR Trig Pos r=1.5 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1.5 d=64 m=128 unmodified.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=1.5 d=64 m=16384 unmodified.png}}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Angular r=1.5, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Gaussian r=1.5, d=64 sigma=2.png}
    \end{center}
    \end{minipage}
\end{figure}




\newpage



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep17 ERR Angular r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep16 ERR Gaussian r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\iffalse


\newpage

\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=128.png}} 
    \subfigure[]{\includegraphics[width=0.49\textwidth]{img/new_plots/Sep16 ERR Trig Pos r=2 d=64 m=16384.png}}
    \end{center}
    \end{minipage}
\end{figure}




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/With relative error Angular r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/With relative error Truncated Gaussian r=2, sigma=1, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/With relative error Angular r=2, d=64.png}
    \end{center}
    \end{minipage}
\end{figure}



\newpage

\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/new_plots/TrigPos r=2 d=64 m=128.png}
    \end{center}
    \end{minipage}
\end{figure}



\fi


\newpage


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/Sep26 Comparison on PTB Dataset.png}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.99\linewidth]{img/new_plots/ComparisonOfFullSoftmaxWithDifferentTau.png}
    \end{center}
    \end{minipage}
\end{figure}





\iffalse

\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/r=1, lambda=1, k=m=32.png}
    \end{center}
    \end{minipage}
\end{figure}




\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/r=1.5, lambda=1, k=m=32.png}
    \end{center}
    \end{minipage}
\end{figure}





\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.82\linewidth]{img/r=2, lambda=1, k=m=32.png}
    \end{center}
    \end{minipage}
\end{figure}


\begin{figure}[h]
\vspace{-3mm}
    \begin{minipage}{1.0\textwidth}
    \begin{center}
    \includegraphics[width=.55\linewidth]{img/new_plots/TrigPos r=1 d=64 m=128.png}
    \end{center}
    \end{minipage}
\end{figure}








\fi



==> redo_wasserstein.tex <==
POS:  normalize=True (i.e. divide by sqrt(D)) (Need this otherwise too spiky gets division by 0 or blows up) 
Wass between 1 D :
(Current issues with the logic. Redo )
-----
64 dims : (previous calc: 0.0001733546709
3873.522346493703

128 dims:
(Prev calc : 0.0001751364405407047)
3834.3128269357208

256 dims:
(prev calc: 0.00017551147489137665)
3836.4489776151413

512 dims : 
prev calc: 0.0001757072986050169
3832.2541091130906

------
RFF (Same normalization as before)
64 dims: #neg probabilities = 389655751
1273 rows of all negatives
(prev calc: 0.00017034180235048712)
3918.9444470390827

128 dims: 382700527
1200 rows of all negatives
(prev calc: 0.00017037847641404884)
3919.3135769811192

256 dims: 380736251
1092 rows of all negs
(prev calc: 0.00017053129410996915)
3917.8634291038607

512 dims: 366352621
965 rows of all negs
(prev calc: 0.00017061456789765432)
3913.5533617588962

1024 dims: 348862312
907 rows of all negatives 

------
Hybrid features
64 dim: no neg 
3998.771141585179

128 dim: no neg values
3994.5118933801004

256 dim: no neg values
3993.625978735541

512 dim:
3994.526124077072

-----
Hybrid (ang-hyb-att)
64 feats (8,8) 129550769 negs and no rows where all the rows are negative
3860.6802630547463

(32,4) 128 feats 148405849 negs and no rows all neg
3877.355791158878

(16,8): 128711703 negs
3872.474239515384

(8,16) 132652334 negs
3851.985026028889

256 feats:
----
(16,16)
128957063 negs
3882.2713117105845

(32, 8)
130409083 negs
3876.2982834701675

(8,32)
126829994 negs
3870.452882061927

512 feats:
(32,32) 128023674 negs
3879.110326448242

(64,8) 127018768 negs
3896.134624287219

(8, 64)
126331310 negs
University 3863.3471578142558

---------------------------------------------

WIKITEXT:
POS : 64
3.091665103802842e-05

128:
4.574975195924697e-05

256:
3.09050922059733e-05

512:
3.1471821742058816e-05

==> related_work-HRF.tex <==
\section{Related work}

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

==> theory.tex <==
\section{Robust Estimation of Softmax and Gaussian Kernels}
\label{sec:theory}

\subsection{Preliminaries}
\label{sec: prel}

In this work we focus on the following kernel functions:

\begin{definition}[Softmax and Gaussian kernel]
For $\mathbf{x},\mathbf{y} \in \mathbb{R}^{d}$, the softmax ($\mathrm{SM}$) and Gaussian kernels are defined as follows:
\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y})\overset{\mathrm{def}}{=}\exp(\mathbf{x}^{\top}\mathbf{y}), \qquad \mathrm{K}_{\mathrm{gauss}} \overset{\mathrm{def}}{=}\exp(-\frac{\|\mathbf{x}-\mathbf{y}\|_{2}^{2}}{2}).
\end{equation}
\end{definition}

We will approximate these kernels with estimators leveraging random feature map representations.

\begin{definition}[Kernel with a Random Feature Map Representation]
We say that a kernel function $\mathrm{K}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ \textit{admits a random feature map representation} if it can be written as:
\begin{equation}
\mathrm{K}(\mathbf{x},\mathbf{y}) = \mathbb{E}_{\omega \sim \Omega}\left[\sum_{i=1}^{l} \xi_{i}(\mathbf{x},\omega)\xi_{i}(\mathbf{y},\omega)\right]  ,  
\end{equation}
for some $\xi_{i}: \mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, and where $\omega$ is sampled from some probabilistic distribution $\Omega \in \mathcal{P}(\mathbb{R}^{d})$.
The corresponding regular random feature map, for a given $m \in \mathbb{N}$, is defined as:
\begin{equation}
\label{random_feature_map_formula}
\phi^{\mathrm{iid}}_{m}(\mathbf{u}) = \frac{1}{\sqrt{m}} \phi_{m}^{1}(\mathbf{u}) \star ... \star \phi_{m}^{l}(\mathbf{u}) \in \mathbb{R}^{ml},  
\end{equation}
where $\phi_{m}^{i} = (\xi_{i}(\mathbf{u},\omega_{1}),...,\xi_{i}(\mathbf{u},\omega_{m}))^{\top}$ for $i=1,...,l$, the symbol $\star$ stands for vertical concatenation, and %furthermore 
$\omega_{1},...,\omega_{m} \overset{\mathrm{iid}}{\sim} \Omega$.
\end{definition}
It is not hard to see that regular feature maps can be used to unbiasedly approximate corresponding kernels, leading to estimators of the form: 
\begin{equation}
\widehat{\mathrm{K}}^{\mathrm{iid}}(\mathbf{x},\mathbf{y}) = \phi^{\mathrm{iid}}_{m}(\mathbf{x})^{\top}
\phi^{\mathrm{iid}}_{m}(\mathbf{y}).    
\end{equation}

If $\Omega$ is isotropic, there exists another procedure for constructing random feature maps that still leads to the unbiased estimator, yet often implies better concentration results. In that procedure $\omega_{1},...,\omega_{m}$ are sampled in such a way that $\omega_{i} \sim \Omega$ still holds for $i=1,...,m$, however this time different $\omega_{i}$ are constrained to be exactly orthogonal, i.e. $\omega_{i}^{\top}\omega_{j}=0$ for $i \neq j$ (with probability $1$, not only on expectation). See: \citep{unrea} for straightforward explicit constructions of such ensembles.
We call feature maps $\phi^{\mathrm{ort}}_{m}$ obtained in such a way, \textit{orthogonal random feature maps}. Of course for the above construction we assume that $m \leq d$ (there exist extensions of the above mechanism for $m > d$, where vectors $\omega$ are partitioned into independently choden blocks such that vectors within a block are orthogonal).

\textbf{Note:} It was shown in \citep{geometry} that orthogonal random features asymptotically for large enough $d$ lower the variance of the estimation, yet this result cannot be extended to any $d$. The analysis breaks for arbitrary $d$ because produced random features can be of arbitrary signs.

It is a well known fact (\cite{fourierapprox}) that Gaussian kernel admits random feature map representation utilizing trigonometric functions, namely: $l=2$, $\Omega=\mathcal{N}(0,\mathbf{I}_{d})$ (see: Eq. \ref{random_feature_map_formula}) and:
\begin{equation}
\xi_{1}(\mathbf{u},\omega) = \sin(\omega^{\top}\mathbf{u}), \textrm{ } \xi_{2}(\mathbf{u}, \omega) = \cos(\omega^{\top}\mathbf{u}).    
\end{equation}

This decomposition directly leads to the random feature map mechanism for the softmax kernel with:
\begin{equation}
\label{trig-features}
\xi_{1}(\mathbf{u},\omega) = \exp(\frac{\|\mathbf{u}\|^{2}}{2})\sin(\omega^{\top}\mathbf{u}), \textrm{ }     
\xi_{2}(\mathbf{u},\omega) = \exp(\frac{\|\mathbf{u}\|^{2}}{2})\cos(\omega^{\top}\mathbf{u}),
\end{equation}
since:
\begin{equation}
\label{gaussian_to_softmax}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \exp(\frac{\|\mathbf{x}\|^{2}}{2})\mathrm{K}_{\mathrm{gauss}}(\mathbf{x},\mathbf{y})\exp(\frac{\|\mathbf{y}\|^{2}}{2}). 
\end{equation}

\subsection{Positive Random Features}

The above mechanism produces random features that in principle can be negative even though values of kernels under consideration are strictly positive. This is not a problem if approximated kernel values are bounded away from $0$ since introduced estimators are unbiased.
However if very small kernel values are involved, the quality of the approximation deteriorates and using the mechanism is even more problematic if those kernel values appear in denominators of more complex expressions (for instance in renormalization procedures as in standard softmax mechanism producing discrete probabilistic distributions). 

In response, a new random feature map mechanism for unbiasedly approximating softmax kernels and thus consequently, also Gaussian kernels was introduced in \citep{performers}. This mechanism can be further integrated with the orthogonal random feature techniques described above, to provide more accurate, still unbiased mechanism, with provably lower estimation variance for any $d>0$, as we later show.
\begin{lemma}[Positive Random Features]
\label{pos_random_features_lemma}
For $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$, the following is true:
\begin{equation}
\label{main_eq}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = 
\mathbb{E}_{\omega \sim \mathcal{N}(0,\mathbf{I}_{d})}\left[\mathrm{exp}(\omega^{\top}\mathbf{x} - \frac{\|\mathbf{x}\|^{2}}{2})\mathrm{exp}(\omega^{\top}\mathbf{y}-\frac{\|\mathbf{y}\|^{2}}{2})\right]=\\
\Lambda \mathbb{E}_{\omega \sim \mathcal{N}(0,\mathbf{I}_{d})}\cosh(\omega^{\top}\mathbf{z})
\end{equation}
for $\mathbf{z}=\mathbf{x}+\mathbf{y}$ and $\Lambda = \exp(-\frac{\|\mathbf{x}\|^{2}+\|\mathbf{y}\|^{2}}{2})$.
Consequently, softmax kernel admits a positive random feature map decomposition with $l=1$ and $\xi_{1}(\mathbf{u}, \omega) = \mathrm{exp}(\omega^{\top}\mathbf{u} - \frac{\|\mathbf{u}\|^{2}}{2})$, (and by Eq. \ref{gaussian_to_softmax} so does Gaussian kernel with $l=1$ and 
$\xi_{1}(\mathbf{u}, \omega)=
\mathrm{exp}(\omega^{\top}\mathbf{u} - \|\mathbf{u}\|^{2})$).
Furthermore, softmax kernel admits also a hyperbolic random feature map decomposition (leveraging the formula for hyperbolic cosine) with $l=2$ and: $\xi_{1}(\mathbf{u},\omega)=\frac{1}{\sqrt{2}}\exp(\omega^{\top}\mathbf{u}-\frac{\|\mathbf{u}\|^{2}}{2})$, $\xi_{2}(\mathbf{u},\omega)=\frac{1}{\sqrt{2}}\exp(-\omega^{\top}\mathbf{u}-\frac{\|\mathbf{u}\|^{2}}{2})$.

\end{lemma}





\subsection{Positive versus Trigonometric Random Features}

The following is true:

\begin{lemma}[positive versus trigonometric random features]
\label{mse-lemma}
Denote by $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})$ an estimator of the value $\mathrm{SM}(\mathbf{x}, \mathbf{y})$ of the softmax kernel
in points $\mathbf{x}, \mathbf{y} \in \mathbb{R}^{d}$ using trigonometric mechanism from Equation \ref{trig-features} and independent random projections $\omega_{1}^{\mathrm{iid}}, ..., \omega_{m}^{\mathrm{iid}}$. Denote by $\widehat{\mathrm{SM}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})$ its analogue using independent positive random features from Lemma \ref{pos_random_features_lemma} with $l=1$ and by $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})$ the one with $l=2$. The mean squared errors ($\mathrm{MSE}$s) of these estimators are given by:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})) =
\frac{1}{2m} \exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})
(1-\mathrm{exp}(-\|\Delta\|^{2}))^{2}, \\ 
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{+}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2})),\\
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{2m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2}))^{2},
\end{split}
\end{align}
where $\Delta = \mathbf{x} - \mathbf{y}$ and $\mathbf{z} = \mathbf{x} + \mathbf{y}$.
\end{lemma}

From now on we will focus on $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$.
An interesting special case to analyze is for $\|\mathbf{x}\|=\|\mathbf{y}\|=r$. Denote by $\theta \in [0, \pi]$ and angle between $\mathbf{x}$ and $\mathbf{y}$. The following is a direct implication of Lemma \ref{mse-lemma}.

\begin{lemma}
\label{normalized_input_lemma}
The following is true for $\|\mathbf{x}\|=\|\mathbf{y}\|=r$ with an angle $\theta \in [0, \pi]$ between them:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{2m}\exp(2r^{2})(1-\exp(-4r^{2}\sin^{2}(\frac{\theta}{2})))^{2}\\ 
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y})) = \frac{1}{2m}\exp(8r^{2}\cos^{2}(\frac{\theta}{2})-2r^{2})
(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2})))^{2}
\end{split}
\end{align}
\end{lemma}

\subsection{Positive \& Trigonometric Random Features as Special Cases of the complex Exponential Estimator}

We present below the unification angle of the techniques presented above, showing that these are just two special instantiations of the more general mechanism.

We start with the following lemma which is a simple consequence of the theory of complex functions, yet also a gateway to the aforementioned unification:

\begin{lemma}
\label{complex}
Let $\omega \sim \mathcal{N}(0,\mathbf{I}_{d})$. Then for every $\mathbf{z} \in \mathbb{C}^{d}$ the following holds:
\begin{equation}
\mathbb{E}[\exp(\omega^{\top}\mathbf{z})] = \exp(\frac{\mathbf{z}^{2}}{2}),    
\end{equation}
where $\mathbf{z}^{2} \overset{\mathrm{def}}{=}  z_{1}^{2} + ... + z_{d}^{2}$.
\end{lemma}
\begin{proof}
From the independence of $\omega_{1},...,\omega_{d}$ we get:
\begin{equation}
\mathbb{E}[\exp(\omega^{\top}\mathbf{z})] = \prod_{i=1}^{d} \mathbb{E}[\mathrm{exp}(\omega_{i}z_{i})]    
\end{equation}
Thus it suffices to show that for $g \sim \mathcal{N}(0,1)$ and any $z \in \mathbb{C}$ the following holds:
\begin{equation}
\mathbb{E}[\mathrm{exp}(gz)] = \mathrm{exp}(\frac{z^{2}}{2})    
\end{equation}
Define $f(z) = \mathbb{E}[\mathrm{exp}(gz)]$. 
Note that $f(z) = \mathrm{exp}(\frac{z^{2}}{2})$ for $z = \mathbf{i}x$, where $\mathbf{i}^{2}=-1$ and $x \in \mathbb{R}$ which follows from the formulae of the characteristic function of the gaussian distribution. Similarly, $f(z) = \mathrm{exp}(\frac{z^{2}}{2})$ for $z \in \mathbb{R}$ which follows from the formulae of the moment generating function of the gaussian distribution.
We now use the fact from complex analysis that if two analytic functions $\mathbb{C} \rightarrow \mathbb{C}$ are identical on uncountably many points then they are equal on $\mathbb{C}$ to complete the proof (we leave to the reader checking that both $f(z)$ and $g(z)\overset{\mathrm{def}}{=}\mathrm{exp}(\frac{z^{2}}{2})$ are analytic).
\end{proof}

Take: $\mathbf{z} = \mathbf{i}(\mathbf{x}-\mathbf{y})$. Using Lemma \ref{complex}, we get:
\begin{equation} \label{exp - norm cos}
\mathrm{exp}(-\frac{\|\mathbf{x}-\mathbf{y}\|^{2}}{2}) = \mathbb{E}[\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))],   
\end{equation}
which leads to the trigonometric estimator.
Now take: $\mathbf{z} = \mathbf{x} + \mathbf{y}$.
Using Lemma \ref{complex}, we get:
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{x}+\mathbf{y}\|^{2}}{2}) = \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{x}+\mathbf{y}))],    
\end{equation}
which implies the estimator based on positive random features (nonhyperbolic one). 

Finally, consider $\mathbf{z} = \mathbf{Ax} + \mathbf{(A^{\top})^{-1}y}$ for an invertible (in $\mathbb{C}^{d \times d})$ matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$. Using Lemma \ref{complex}, we get this time:
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{Ax}\|^{2}}{2})  
\mathrm{exp}(\frac{\|(\mathbf{A}^{\top})^{-1}\mathbf{y}\|^{2}}{2})\mathrm{SM}(\mathbf{x},\mathbf{y}) 
= \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{Ax}+(\mathbf{A}^{\top})^{-1}\mathbf{y})]
\end{equation}
Thus for 
$\Psi^{m}_{\mathbf{M}}(\mathbf{z}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{Mz}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{Mz}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{Mz}))^{\top}$ and $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$:
\begin{equation}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{\top})^{-1}}(\mathbf{y})]
\end{equation}

Therefore we have a new random feature map mechanism leading to an estimator unbiasedly approximating softmax kernel. In general it is asymmetric (different parameterization for $\mathbf{x}$ and $\mathbf{y}$; one uses $\mathbf{A}$, the other one $\mathbf{A}^{-1}$).
We call an estimator $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y})$ defined as:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y}) \overset{\mathrm{def}}{=} \Psi^{m}_{\mathbf{A}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{\top})^{-1}}(\mathbf{y})    
\end{equation}
a \textit{complex exponential} estimator of the softmax kernel.

Note that if we take $\mathbf{A} \overset{\mathrm{def}}{=} \mathbf{i}\mathbf{I}_{d}$ then $\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y})$ becomes $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}(\mathbf{x},\mathbf{y})$ and if we take $\mathbf{A} \overset{\mathrm{def}}{=} \mathbf{I}_{d}$ then
$\widehat{\mathrm{SM}}^{\mathrm{cexp}}_{m}(\mathbf{x},\mathbf{y})$ becomes $\widehat{\mathrm{SM}}_{m}^{\mathrm{+}}(\mathbf{x},\mathbf{y})$.

Note also that an estimator based on this mechanism has variance equal to $0$ if:
\begin{equation}
\mathbf{x} = -(\mathbf{A}^{-1})(\mathbf{A}^{\top})^{-1}\mathbf{y}    
\end{equation}
In fact we can relax the above condition. It is easy to check that for the variance to zero out, we only need:
\begin{equation}
\left\{ \begin{array}{rcl}
\mathrm{Re}(\mathbf{A})\mathbf{x} + \mathrm{Re}((\mathbf{A}^{T})^{-1})\mathbf{y}=0 \\ 
\mathrm{Im}(\mathbf{A})\mathbf{x} + \mathrm{Im}((\mathbf{A}^{T})^{-1})\mathbf{y}=0
\end{array}\right.
\end{equation}



\subsection{Hybrid Random Features for the Softmax Kernel}
\label{hybrid}

Denote by $\mathcal{E}=( \asm )_{k=1}^{p+1}$ a list of estimators of $\sm$ (the so-called \textit{base estimators}) and by $\Lambda = ( \alamgen )_{k=1}^{p}$ a list of estimators of: 
$\{\lambda^{k}(\mathbf{x},\mathbf{y})\}_{k=1}^{p}$ for some functions
$\lambda^{k}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$, constructed independently from $\mathcal{E}$.
Take the following estimator of $\sm$:
\begin{equation}
\label{gen-hyb-eque}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{k=1}^{p} \alamgen \asm + \left(1-\sum_{k=1}^{p} \alamgen \right)\widehat{\mathrm{SM}}^{p+1}(\mathbf{x},\mathbf{y})
\end{equation}
We call $\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y})$ a \textit{general hybrid estimator} of $\sm$ parameterized by $\mathcal{E},\Lambda$. Note that if elements of $\mathcal{E}$ are unbiased estimators of $\sm$, then trivially $\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y})$ is also an unbiased estimator of $\sm$. Assume that each $\asm$ is of the form:
\begin{equation}
\asm = (\phi_{m}^{k}(\mathbf{x}))^{\top}\phi_{m}^{k}(\mathbf{y})    
\end{equation}
for $\phi_{m}^{k}(\mathbf{z}) = \frac{1}{\sqrt{m}} 
\phi_{m}^{1,k}(\mathbf{z}) \star ... \star \phi_{m}^{t_{k},k}(\mathbf{z})$ and some: $t_{k}>0$ and $\phi_{m}^{1,k},..., \phi_{m}^{t_{k},k}:\mathbb{R}^{d} \rightarrow \mathbb{R}^{m}$. Assume also that $\lambda^{k}(\mathbf{x},\mathbf{y})$ can be written as:
\begin{equation}
\label{lambda-eq}
\lambda^{k}(\mathbf{x},\mathbf{y}) = a_{k} + \mathbb{E}_{\tau \sim \Lambda}[\sum_{i=1}^{l_{\lambda_{k}}}\xi^{i}_{\lambda_{k}}(\mathbf{x},\tau)\xi^{i}_{\lambda_{k}}(\mathbf{y}, \tau)]  
\end{equation}
for some scalars $a_{k} \in \mathbb{R}$, distribution $\Lambda \in \mathcal{P}(\mathbb{R}^{d})$ and mappings $\xi^{i,k}_{\lambda}:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ and that the corresponding estimator $\widehat{\lambda}^{k}(\mathbf{x},\mathbf{y})=\widehat{\lambda}^{k}_{n}(\mathbf{x},\mathbf{y})$ is of the form:
\begin{equation}
\label{lambda-eq-estimate}
\widehat{\lambda}^{k}_{n}(\mathbf{x},\mathbf{y}) = a_{k} + (\phi_{n}^{\lambda_{k}}(\mathbf{x}))^{\top}    
\phi_{n}^{\lambda_{k}}(\mathbf{y})
\end{equation}
for 
\begin{equation}
\phi_{n}^{\lambda_{k}}(\mathbf{x}) =  \frac{1}{\sqrt{n}}\phi_{n}^{1,\lambda_{k}}(\mathbf{x}) \star ... \star \phi_{n}^{l_{\lambda_{k}},\lambda_{k}}(\mathbf{x})
\end{equation}
and $\phi_{n}^{i,\lambda_{k}}(\mathbf{x})=
(\xi^{i}_{\lambda_{k}}(\mathbf{x},\tau_{1}),...,\xi^{i}_{\lambda_{k}}(\mathbf{x},\tau_{n}))^{\top}$ for $\tau_{1},...,\tau_{n} \sim \Lambda$.
We then get:
\begin{align}
\begin{split}
\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y}) = \sum_{k=1}^{p}
\frac{a_{k}}{m}(\phi_{m}^{1,k}(\mathbf{x}) \star ... \star \phi_{m}^{t_{k},k}(\mathbf{x}))^{\top}(\phi_{m}^{1,k}(\mathbf{y}) \star ... \star \phi_{m}^{t_{k},k}(\mathbf{y})) + \\
\frac{1}{mn}\sum_{k=1}^{p}\sum_{i=1}^{l_{\lambda_{k}}}\sum_{j=1}^{t_{k}}
(\phi_{n}^{i,\lambda_{k}}(\mathbf{x}) \otimes \phi_{m}^{j,k}(\mathbf{x}))^{\top}(\phi_{n}^{i,\lambda_{k}}(\mathbf{y}) \otimes \phi_{m}^{j,k}(\mathbf{y}))+ \\
\frac{1-\sum_{k=1}^{p} a_{k}}{m}(\phi_{m}^{1,p+1}(\mathbf{x}) \star ... \star \phi_{m}^{t_{p+1},p+1}(\mathbf{x}))^{\top}(\phi_{m}^{1,p+1}(\mathbf{y}) \star ... \star \phi_{m}^{t_{p+1},p+1}(\mathbf{y})) - \\
\frac{1}{mn}\sum_{k=1}^{p}\sum_{i=1}^{l_{\lambda_{k}}}\sum_{j=1}^{t_{p+1}}
(\phi_{n}^{i,\lambda_{k}}(\mathbf{x}) \otimes \phi_{m}^{j,p+1}(\mathbf{x}))^{\top}(\phi_{n}^{i,\lambda_{k}}(\mathbf{y}) \otimes \phi_{m}^{j,p+1}(\mathbf{y})) = 
\Psi(\mathbf{x})^{\top}\Psi(\mathbf{y}),
\end{split}
\end{align}
where $\mathbf{u} \otimes \mathbf{v}$ stands for the vectorized outer-product of $\mathbf{u}$ and $\mathbf{v}$ and furthermore 
\begin{equation}
\label{hyb-all-1}
\Psi(\mathbf{z})=\Psi_{1}(\mathbf{z}) \star \Psi_{2}(\mathbf{z}) \star \Psi_{3}(\mathbf{z}) \star \Psi_{4}(\mathbf{z})
\end{equation}
for $\Psi_{1},\Psi_{2}, \Psi_{3}, \Psi_{4}$ defined as:

\begin{align}
\begin{split}
\label{hyb-all-2}
\Psi_{1}(\mathbf{z})=\prod_{k=1,...,p}^{\star} \sqrt{\frac{a_{k}}{m}}\phi_{m}^{1,k}(\mathbf{z})\star ... \star \phi_{m}^{t_{k},k}(\mathbf{z})\\
\Psi_{2}(\mathbf{z})=\frac{1}{\sqrt{mn}}\prod_{k=1,...,p}^{\star} \prod^{\star}_{i,j \in \{1,...,l_{\lambda_{k}}\}\times\{1,...,t_{k}\}} \phi_{n}^{i,\lambda_{k}}(\mathbf{z}) \otimes \phi_{m}^{j,k}(\mathbf{z})\\
\Psi_{3}(\mathbf{z})=\sqrt{\frac{1-\sum_{k=1}^{p} a_{k}}{m}}\phi_{m}^{1,p+1}(\mathbf{z})\star ... \star \phi_{m}^{t_{p+1},p+1}(\mathbf{z})\\
\Psi_{4}(\mathbf{z})=\frac{\mathbf{i}}{\sqrt{mn}}\prod_{k=1,...,p}^{\star} \prod^{\star}_{i,j \in \{1,...,l_{\lambda_{k}}\}\times\{1,...,t_{p+1}\}} \phi_{n}^{i,\lambda_{k}}(\mathbf{z}) \otimes \phi_{m}^{j,p+1}(\mathbf{z})\\
\end{split}    
\end{align}
Here $\prod^{*}$ stands for the concatenation operator and $\mathbf{i}^{2}=-1$. 
We conclude that $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ admits a random feature map representation.

\subsubsection{Scoring different general hybrid estimators}

To rank different hybrid estimators that we will consider later in the paper, we define softmax-kernel estimator's error in the following way. 

\begin{definition}
Assume that the inputs to the estimators are taken from some given bounded set $\mathcal{C} \subseteq \mathbb{R}^{d}$. For a given hybrid estimator $\widehat{\mathrm{SM}}$ on feature vectors $\mathbf{x},\mathbf{y} \in \mathcal{C}$, we define its max-relative-error with respect to $\mathcal{C}$ as:
\begin{equation}
\epsilon_{\mathcal{C}}(\widehat{\mathrm{SM}}) = \max_{\mathbf{x},\mathbf{y} \in \mathcal{C}} \eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}}), \textrm{where }
\eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}})=\frac{\sqrt{\mathrm{MSE}(\widehat{\mathrm{SM}}(\mathbf{x},\mathbf{y}))}}{\mathrm{SM}(\mathbf{x},\mathbf{y})}.
\end{equation}
\end{definition}

This definition captures the critical observation that in several applications of the softmax-kernel estimation, e.g. efficient softmax-sampling or linear-attention Transformers \citep{performer}, small relative errors are a much more meaningful measure of the quality of the method than small absolute errors.
As we will show below, it is also a gateway to find hidden symmetries between different estimators. 
Before providing specific instantiations of the class of general hybrid estimators given above and analyzing their corresponding error functions, we conduct such an analysis for the base estimators $\tri$ and $\expo$.

\begin{lemma}
\label{tri-exp-imp-lemma}
Denote by $S(r)$ a sphere centered at $0$ and of radius r. Let 
$\eps_{\theta, r}(\widehat{\mathrm{SM}})=\eps_{\mathbf{x},\mathbf{y}}(\widehat{\mathrm{SM}})$ for $\mathbf{x},\mathbf{y} \in S(r)$ and such that $\theta=\theta_{\mathbf{x},\mathbf{y}}$ (note that the mean squared errors of the considered estimators depend only on the angle $\theta_{\mathbf{x},\mathbf{y}}$ for $\mathbf{x},\mathbf{y}$ chosen from a fixed sphere). Then the following holds:
\begin{align}
\begin{split}
\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}})=\frac{1}{\sqrt{2m}}\exp(2r^{2}\sin^{2}(\frac{\theta}{2}))\left(1-\exp(-4r^{2}\sin^{2}(\frac{\theta}{2}))\right)\\
\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}})=\frac{1}{\sqrt{2m}}\exp(2r^{2}\cos^{2}(\frac{\theta}{2}))
\left(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2}))\right),
\end{split}
\end{align} and consequently for $W(r)=\exp(2r^{2})
\left(1-\exp(-4r^{2})\right)$:
\begin{equation}
\epsilon_{S(r)}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}) = 
\epsilon_{S(r)}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}) = \lim_{\theta \rightarrow \pi} \epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}) = 
\lim_{\theta \rightarrow 0} \epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}) =
\sqrt{\frac{1}{2m}}W(r)
\end{equation}
\end{lemma}
Thus interestingly there is a symmetry between both the mechanisms that is captured by the defined relative error since $\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}})$ can be obtained from $\epsilon_{\theta, r}(\widehat{\mathrm{SM}}_{m}^{\mathrm{++}})$ by the transformation $\theta \rightarrow \pi - \theta$.

Thus both mechanisms achieve the same max-relative-error yet, as we have noticed before, in different regions of space. Estimator $\widehat{\mathrm{SM}}_{m}^{\mathrm{++}}$ works much better than $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}$ for linear attention in Performers \citep{performer}, since in the attention tensor there are many more small values (where it is more accurate) than large values (where the latter one is more accurate).

\begin{proof}
The first two equations follow directly from Lemma \ref{normalized_input_lemma}:
Notice that this error is the increasing function of $\sin^{2}(\frac{\theta}{2})$ and thus is largest for $\theta=\pi$. Plugging in this value into the formula of the max-relative-error gives us thee expression from the statement of the lemma. By the analogous analysis, we obtain second equation (this time the error is maximized for $\theta=0$).
\end{proof}

\subsubsection{Computational gains of hybrid estimators}

Consider the general hybrid estimator of $\mathrm{SM}(\mathbf{x},\mathbf{y})$ from Equation \ref{gen-hyb-eque}, using $p+1$ base estimators.
Assume that the $k^{th}$ base estimator for $k=1,...,p+1$ applies $m$ random features in each of the corresponding $t_{k}$ random maps  and that $n$ random features are used in each of the corresponding $l_{\lambda_{k}}$ random maps to approximate $k^{th}$ $\lambda$-coefficient for $k=1,...,p$.
From Equation \ref{hyb-all-1} and Equation \ref{hyb-all-2}, we conclude that time complexity of constructing $\Psi(\mathbf{z})$ is:
\begin{equation}
T = O\left((t_{1}+...+t_{p+1})md + 
(nd + md + mn)\sum_{k=1}^{p+1}\sum_{r=1}^{p}t_{k}l_{\lambda_{r}}\right)
\end{equation}
Thus the resulting $\Theta(mn)$-dimensional random feature map $\Psi(\mathbf{z})$. 



\subsubsection{Hybrid Gaussian-mixtures estimators}

We consider now the prominent special case of the general hybrid estimator mechanism described above, the so-called \textit{hybrid gaussian-mixtures estimators}. In that setting, functions $\alamgen$ are defined as:
\begin{equation}
\alamgen = \exp(-\frac{\|\mathbf{x}+\mathbf{M}_{k}\mathbf{y}\|_{2}^{2}}{2\tau_{k}^{2}}),    
\end{equation}
for some $\mathbf{M}_{1},...,\mathbf{M}_{p} \in \mathbb{R}^{d \times d}$ and $\tau_{1},...,\tau_{p} \in \mathbb{R}$. Since lambda-coefficients are here the values of the Gaussian kernel between vectors: $\frac{\mathbf{x}}{\tau_{k}}$ and $-\frac{\mathbf{M}_{k}\mathbf{y}}{\tau_{k}}$ and furthermore Gaussian and softmax-kernels are related as given by Eq. \ref{gaussian_to_softmax}, we can take $a_{k}=0$ and define corresponding $\phi_{n}^{\lambda_{k}}$ as:

\begin{equation}
\left\{ \begin{array}{rcl}
\phi_{n}^{\lambda_{k}}(\mathbf{z}) = \exp(-\frac{\|\mathbf{z}\|_{2}^{2}}{2\tau_{k}^{2}})\phi_{n}^{\mathrm{SM}}(\frac{\mathbf{z}}{\tau_{k}}) \textrm{ if $\mathbf{z}=\mathbf{x}$}  \\
\phi_{n}^{\lambda_{k}}(\mathbf{z}) = \exp(-\frac{\|\mathbf{M}_{k}\mathbf{z}\|_{2}^{2}}{2\tau_{k}^{2}})\phi_{n}^{\mathrm{SM}}(-\frac{\mathbf{M}_{k}\mathbf{z}}{\tau_{k}}) \textrm{ if $\mathbf{z}=\mathbf{y}$}
\end{array}\right.
\end{equation}

where $\phi_{n}^{\mathrm{SM}}$ is the random feature map corresponding to a particular estimator of the softmax-kernel.



\subsubsection{Bipolar hybrid estimators}
Now take another special case of the general hybrid estimator defined above,
where $\mathcal{E} = (\widehat{\mathrm{SM}}^{++}(\mathbf{x},\mathbf{y}),\widehat{\mathrm{SM}}^{\mathrm{trig}}(\mathbf{x},\mathbf{y}))$. Thus consider estimator $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ of the softmax kernel $\mathrm{SM}$:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}(\mathbf{x},\mathbf{y})=\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x}, \mathbf{y}) + (1-\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x}, \mathbf{y}).   
\end{equation}

The question arises what concentration results can be obtained for $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ and how they compare to those for $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$ and $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$. That of course depends also on the choice of $\lambda:\mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$.

If we consider a renormalized case where all input vectors have the same norm $r$, we can rewrite $\lambda(\mathbf{x},\mathbf{y})$ ad $\lambda(\theta_{\mathbf{x},\mathbf{y}})$, where $\theta_{\mathbf{x},\mathbf{y}}$ is an angle between $\mathbf{x}$ and $\mathbf{y}$ (we will use shorter notation $\theta$ if $\mathbf{x}$ and $\mathbf{y}$ are known from the context).
If $\|\mathbf{x}\|=\|\mathbf{y}\|=r$, then by Lemma \ref{normalized_input_lemma} we know that $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}$ becomes perfect for $\theta=\pi$ and $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}$ becomes perfect for $\theta=0$. That suggests particular forms of the mapping $\lambda$. Before exploring this further, we provide some general concentration results regarding bipolar hybrid estimators.

\subsubsection{General results for bipolar hybrid estimators}
\label{general-hybrid-section}

Below we present several general concentration results regarding hybrid estimators. We will refer to those estimators as
$\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})$ since the implicit dependence on $n$ will be hidden in the expressions involving estimators $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ that we will treat as blackboxes now. Analysis of the particular important instantiations of $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ will be conducted later.

\begin{theorem}[MSE of the general bipolar hybrid estimator]
\label{general-hybrid}
Take the bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$). Then the following holds:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{equation}
Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator is further reduced, namely we have:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})) \\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\mathbb{E}[\widehat{\lambda}(\mathbf{x},\mathbf{y})(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))]
\end{split}
\end{align}
\end{theorem}

\begin{proof}
The following holds:
\begin{align}
\begin{split}
\label{main_var_formulae}
\mathrm{Var}(\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m}(\mathbf{x},\mathbf{y})) = 
\mathrm{Var}\left(\widehat{\lambda}(\theta)\widehat{\mathrm{SM}}^{++}_{m}(\mathbf{x},\mathbf{y})\right) + \mathrm{Var}\left((1-\widehat{\lambda}(\theta))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})\right) + \\
2\mathrm{Cov}\left(\widehat{\lambda}(\theta)\widehat{\mathrm{SM}}^{++}_{m}(\mathbf{x},\mathbf{y}), (1-\widehat{\lambda}(\theta))\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})\right) 
\end{split}
\end{align}

We will focus now on the covariance term.
Assume first easier to analyze case where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently. Then the following is true:

\begin{align}
\begin{split}
\cov\left(\alam \expo, \aonelam \tri\right) = \\ 
\mathbb{E}[\alam \aonelam \expo \tri] - \mathbb{E}[\alam \expo]\mathbb{E}[\aonelam \tri] \\
= \left(\mathbb{E}[\alam \aonelam]-\mathbb{E}[\alam]\mathbb{E}[\aonelam]\right)\mathbb{E}[\expo]\mathbb{E}[\tri] \\ = -(\sm)^{2}\var(\alam)
\end{split}
\end{align}


Now assume that $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ use the exact same random projections. Then, using similar analysis as before, we get:
\begin{align}
\begin{split}
\cov\left(\alam \expo, \aonelam \tri\right) = \\
\mathbb{E}[\expo \tri]\mathbb{E}[\alam \aonelam] - (\sm)^{2}\mathbb{E}[\alam]\mathbb{E}[\aonelam]
\end{split}    
\end{align}
This time however it is no longer the case that $\mathbb{E}[\expo \tri]\mathbb{E}[\alam \aonelam] = \mathbb{E}[\expo]\mathbb{E}[\tri]=(\sm)^{2}$ since $\expo$ and $\tri$ are no longer independent.
In order to compute $\mathbb{E}[\expo \tri]\mathbb{E}[\alam \aonelam]$, we will first introduce useful denotation.

Denote by $\omega_{1},...,\omega_{m} \overset{\mathrm{iid}}{\sim} \mathcal{N}(0,\mathbf{I}_{d})$ the random projections sampled to construct both $\expo$ and $\tri$. Denote: $Y_{i}=\cosh(\omega_{i}^{\top}(\mathbf{x}+\mathbf{y}))\overset{\mathrm{def}}{=}\frac{\exp(\omega_{i}^{\top}(\mathbf{x}+\mathbf{y}))+\exp(-\omega_{i}^{\top}(\mathbf{x}+\mathbf{y}))}{2}$. We have:
\begin{equation}
\expo = \exp\left(-\frac{\|\mathbf{x}\|^{2}+\|\mathbf{y}\|^{2}}{2}\right)\frac{Y_{1}+...+Y_{m}}{m}    
\end{equation}
If we denote: $Z_{i} = \cos(\omega_{i}^{\top}(\mathbf{x}-\mathbf{y}))$, then we can write $\tri$ as:
\begin{equation}
\tri = \exp\left(\frac{\|\mathbf{x}\|^{2}+\|\mathbf{y}\|^{2}}{2}\right)\frac{Z_{1}+...+Z_{m}}{m}    
\end{equation}

We can then rewrite $\mathbb{E}[\expo \tri]$ as:
\begin{align}
\begin{split}
\mathbb{E}[\expo \tri] = 
\frac{1}{m^{2}}\left[\sum_{i \neq j} \mathbb{E}[Y_{i}Z_{j}] +  \sum_{i=1}^{m}\mathbb{E}[Y_{i}Z_{i}]\right]
= \\ \frac{1}{m^{2}}\left[ {m \choose 2} (\sm)^{2} + m \mathbb{E}[\cosh(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))]\right],
\end{split}
\end{align}
where $\omega \sim \mathcal{N}(0,\mathbf{I}_{d})$. The equality follows from the unbiasedness of $\tri$ and $\expo$ and the fact that different $\omega_{i}$ are chosen independently. Thus it remains to compute $\rho = \mathbb{E}[\cosh(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))]$. Note first that 
$\rho = \mathbb{E}[\exp(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))]$
since $-\omega \sim \gauss$ and $\cos$ is an even function. Denote $\mathbf{z}=\mathbf{x}+\mathbf{y} + \mathbf{i}(\mathbf{x}-\mathbf{y})$. We have:
\begin{align}
\begin{split}
\mathbb{E}[\exp(\omega^{\top}(\mathbf{x}+ \mathbf{y}))\cos(\omega^{\top}(\mathbf{x}-\mathbf{y}))] 
= \mathrm{Re}\left[\mathbb{E}[\exp(\omega^{\top}\mathbf{z})]\right] = \mathrm{Re}[\prod_{i=1}^{d}\exp(\frac{z_{i}^{2}}{2})] = \\
\mathrm{Re}\left[\exp\left(\frac{\sum_{j=1}^{d}(x_{j}+y_{j})^{2}+2\mathbf{i}(x_{j}^{2}-y_{j}^{2})-(x_{j}-y_{j})^{2}}{2}\right)\right]=(\sm)^{2}\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2})
\end{split}
\end{align}
Thus we conclude that:
\begin{equation}
\mathbb{E}[\expo \tri] = (1-\frac{1}{m})(\sm)^{2} + \frac{1}{m}(\sm)^{2}\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2})    
\end{equation}

Therefore we get the formulae for the covariance term in both: the setting where random projections of $\tri$ and $\expo$ are shared (variant II) and when they are not (variant I). The following is true 
for $Z=\frac{1}{m}(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2})\mathbb{E}[\alam \aonelam]$:

\begin{equation}
\cov(\alam \expo, \aonelam \tri)=
\left\{ \begin{array}{rcl}
-(\sm)^{2}\mathrm{Var}(\alam) \textrm{ for variant I}  \\ 
-(\sm)^{2}(\mathrm{Var}(\alam)+Z) \textrm{ for variant II}
\end{array}\right.
\end{equation}

We also have the following:
\begin{align}
\begin{split}
\mathrm{Var}(\alam \expo) = \mathbb{E}[(\alam)^{2} (\expo)^{2}] - (\mathbb{E}[\alam \expo])^{2} = \\
\mathbb{E}[(\alam)^{2}]\left(\mathrm{MSE}(\expo)+(\sm)^{2}\right) - (\mathbb{E}[\alam])^{2}(\sm)^{2} = \\
(\sm)^{2}\mathrm{Var}(\alam) + \mathbb{E}[(\alam)^{2}]\mathrm{MSE}(\expo)
\end{split}
\end{align}
and furthermore (by the analogous analysis):
\begin{equation}
\mathrm{Var}(\aonelam \tri)  =    
(\sm)^{2}\mathrm{Var}(\alam) + \mathbb{E}[\aonelam^{2}]\mathrm{MSE}(\tri)
\end{equation}

By putting the derived formulae for the above variance terms as well as covariance terms back in the Equation \ref{main_var_formulae}, we complete the proof of the theorem (note that the mean squared error of the hybrid estimator is its variance since it is unbiased).

\end{proof}

\subsubsection{Lambda-angular bipolar hybrid estimators}

From the discussion just before Section \ref{general-hybrid-section}, we conclude that, for the renormalized case,  by choosing $\lambda: \mathbb{R} \rightarrow \mathbb{R}$ such that $\lambda(0)=0$ and $\lambda(\pi)=1$, and furthermore: $\widehat{\lambda}(0)=\widehat{\lambda}(\pi)=0$, we zero out the variance of $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ in \textbf{both}: $\theta=0$ and $\theta=\pi$ rather than just in one of these points (as it is the case for $\widehat{\mathrm{SM}}_{m}^{++}$ or $\widehat{\mathrm{SM}}_{m}^{\mathrm{trig}}$). Below we propose such a $\lambda$ and $\widehat{\lambda}$.
The easiest choice is to take $\lambda$ to be linear, i.e.:
\begin{equation}
\lambda(\theta) = \frac{\theta}{\pi}    
\end{equation}
To construct $\widehat{\lambda}$, we notice first that the random feature map $\phi_{\mathrm{ang}}$ for the \textit{angular kernel} given as:
\begin{equation}
\mathrm{K}_{\mathrm{ang}}(\mathbf{x},\mathbf{y}) = 1 - \frac{2\theta_{\mathbf{x},\mathbf{y}}}{\pi}    
\end{equation}
is, for $\tau_{1},...,\tau_{n} \sim \mathcal{N}(0,\mathbf{I}_{d})$, defined as:
\begin{equation}
\phi_{n}^{\mathrm{ang}}(\mathbf{z}) = \frac{1}{\sqrt{n}}(\mathrm{sgn}(\tau_{1}^{\top}\mathbf{z}),...,\mathrm{sgn}(\tau_{n}^{\top}\mathbf{z}))^{\top} 
\end{equation}
Therefore we have: 
\begin{equation}
\lambda(\theta) = \frac{\theta}{\pi} = 
\frac{1}{2} - \frac{1}{2}\mathbb{E}[(\phi_{n}^{\mathrm{ang}}(\mathbf{x}))^{\top}\phi_{n}^{\mathrm{ang}}(\mathbf{y})]
\end{equation}
Thus we can construct $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ from Equation \ref{lambda-eq} by taking: 
\begin{equation}
\left\{ \begin{array}{rcl}
a = \frac{1}{2} \\ 
\phi_{n}^{\lambda}(\mathbf{z}) = \frac{i}{\sqrt{2}}\phi_{n}^{\mathrm{ang}}(\mathbf{z})
\end{array}\right.
\end{equation}

We call a hybrid estimator applying such a $\widehat{\lambda}$ as the \textit{lambda-angular bipolar hybrid estimator}. 

We will now compute:
$\alpha = \mathbb{E}[\widehat{\lambda}(\theta)^{2}], \beta = \mathbb{E}[\aonelam^{2}]$ and $\gamma = \mathbb{E}[\alam \aonelam]$ to obtain the formulae of the MSE of the lambda-angular bipolar hybrid estimator according to Theorem \ref{general-hybrid}.
Denote: 
$X_{i} = (\phi_{n}^{\mathrm{ang}}(\mathbf{x}))[i]\phi_{n}^{\mathrm{ang}}(\mathbf{y})[i]$. We have:
\begin{equation}
\widehat{\lambda}(\theta) = \frac{1}{2}\left(1 - 
\sum_{i=1}^{n}X_{i}\right).
\end{equation}
Note first that by the construction of $\widehat{\lambda}(\theta)$, we have: $\mathbb{E}[\widehat{\lambda}(\theta)] = \frac{\theta}{\pi}$ and thus: $\mathbb{E}[\sum_{i=1}^{n} X_{i}] = 1-\frac{2\theta}{\pi}$.
Therefore we conclude that:
\begin{align}
\begin{split}
\label{alpha_eq}
\alpha = \frac{1}{4}\mathbb{E}\left[1-2\sum_{i=1}^{n}X_{i}+
\left(\sum_{i=1}^{n}X_{i}\right)^{2}\right]
= \frac{1}{4}\left(1-2(1-\frac{2\theta}{\pi})+\sum_{i=1}^{n}\mathbb{E}[X_{i}^{2}]+\sum_{i \neq j}\mathbb{E}[X_{i}]\mathbb{E}[X_{j}]\right) \\ =
\frac{1}{4}\left(1-2(1-\frac{2\theta}{\pi})+n \cdot \frac{1}{n^{2}}+n(n-1) \cdot \frac{1}{n^{2}}(1-\frac{2\theta}{\pi})^{2}\right)=
\frac{1}{4}\left(4\frac{\theta}{\pi} + (1-\frac{1}{n})(1-\frac{2\theta}{\pi})^{2}\right) \\
= \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)
\end{split}
\end{align}

Now to calculate $\beta$, it suffices to observe that $1 - \widehat{\lambda}(\theta)$ has the same distribution as $\widehat{\lambda}(\mathbf{x},-\mathbf{y})$. Therefore we only need to substitute in Equation \ref{alpha_eq} angle $\theta$ with $\pi - \theta$ and we get:
\begin{equation}
\beta = \frac{\pi-\theta}{\pi}\left(\frac{\pi-\theta}{\pi}-\frac{\pi-\theta}{n\pi}+\frac{1}{n}\right) = 
\left(1-\frac{\theta}{\pi}\right)\left(1-\frac{\theta}{\pi}+\frac{\theta}{n\pi}\right)
\end{equation}
Finally, the following holds:
\begin{equation}
\gamma = \mathbb{E}[\widehat{\lambda}(\theta)] - \alpha = 
\frac{\theta}{\pi} - \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right) = \frac{\theta}{\pi}
\left(1-\frac{1}{n}-\frac{\theta}{\pi}+\frac{\theta}{n \pi}\right)
\end{equation}

Using Theorem \ref{general-hybrid}, we conclude that:

\begin{theorem}[MSE of the lambda-angular bipolar hybrid estimator]
\label{lambda-bipolar-hybrid}
Take the lambda-angular bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$). Then the following holds:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})) = \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)\frac{1}{2m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2}))^{2} + \\   
= 
\left(1-\frac{\theta}{\pi}\right)\left(1-\frac{\theta}{\pi}+\frac{\theta}{n\pi}\right)\frac{1}{2m} \exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})
(1-\mathrm{exp}(-\|\Delta\|^{2}))^{2}
\end{split}
\end{align}
for $\Delta = \mathbf{x} - \mathbf{y}$ and $\mathbf{z} = \mathbf{x} + \mathbf{y}$.
Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator is further reduced, namely we have:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})) = \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)\frac{1}{2m}\exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})(1-\exp(-\|\mathbf{z}\|^{2}))^{2} + \\   
\left(1-\frac{\theta}{\pi}\right)\left(1-\frac{\theta}{\pi}+\frac{\theta}{n\pi}\right)\frac{1}{2m} \exp(\|\mathbf{z}\|^{2})\mathrm{SM}^{-2}(\mathbf{x},\mathbf{y})
(1-\mathrm{exp}(-\|\Delta\|^{2}))^{2} \\ -\frac{2}{m}\mathrm{SM}^{2}(\mathbf{x},\mathbf{y})
(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))\frac{\theta}{\pi}
\left(1-\frac{1}{n}-\frac{\theta}{\pi}+\frac{\theta}{n \pi}\right)
\end{split}
\end{align}
\end{theorem}

Thus, based on the above and Lemma \ref{normalized_input_lemma}, if $\|\mathbf{x}\|_{2}=\|\mathbf{y}\|_{2}=r$ then regardless of whether the same sets of random projections are applied or not, we get:
\begin{align}
\begin{split}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybang}}_{m,n}(\mathbf{x},\mathbf{y})) = \frac{\theta}{\pi}\left(\frac{\theta}{\pi}-\frac{\theta}{n\pi}+\frac{1}{n}\right)\frac{1}{2m}\exp(8r^{2}\cos^{2}(\frac{\theta}{2})-2r^{2}) \cdot \\
(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2})))^{2} +    
\frac{\theta}{\pi}
\left(1-\frac{1}{n}-\frac{\theta}{\pi}+\frac{\theta}{n \pi}\right)\frac{1}{2m}\exp(2r^{2})(1-\exp(-4r^{2}\sin^{2}(\frac{\theta}{2})))^{2}
\end{split}
\end{align}

Below we estimate the max-relative-error of the lambda-angular bipolar hybrid estimator on the sphere $S(r)$ of radius r. We see that the max-relative-error scales as:
$\frac{1}{r}\exp(2r^{2})$ in $r$ as opposed to $\exp(2r^{2})$ as it is the case for the estimators based solely on positive or trigonometric random features (see: Lemma \ref{tri-exp-imp-lemma}). Furthermore, the max-relative-error scales as $\sqrt{\theta}$ and $\sqrt{\pi-\theta}$ as $\theta \rightarrow 0$ and $\theta \rightarrow \pi$ respectively, in particular goes to $0$ in both critical cases. This is not the case for the estimators based solely on positive or trigonometric random features (for a fixed radius $r$ and the number of random features used).  

\begin{theorem}
The max-relative-error of the lambda-angular bipolar hybrid estimator on the sphere $S(r)$ of radius $r \geq 1$ satisfies for $W(r)=\exp(2r^{2})
\left(1-\exp(-4r^{2})\right)$:
\begin{equation}
\label{hybang_upper}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}}) \leq \frac{1}{r}\sqrt{\frac{1}{2m}}W(r)\sqrt{\frac{1}{\pi} - \frac{1}{n \pi} + \frac{1}{n\sqrt{\pi}}}  
\end{equation}
Furthermore:
\begin{equation}
\label{lim_eq}
\lim_{\theta \rightarrow 0} \frac{\eps_{\theta, r}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}})}{\sqrt{\theta}}= 
\lim_{\theta \rightarrow \pi} \frac{\eps_{\theta, r}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}})}{\sqrt{\theta-\pi}} = \sqrt{\frac{1}{2\pi mn}}W(r)
\end{equation}
\end{theorem}
\begin{proof}
Note first that from the derived above formulae of the MSE of the lambda-angular bipolar hybrid estimator and the definition of the max-relative-error, we obtain:
\begin{equation}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}}) =
\frac{\exp(r^{2})}{\sqrt{2m}}\sqrt{\max_{\theta \in [0, \pi]} h_{r}(\theta)},
\end{equation}
where:
\begin{align}
\begin{split}
h_{r}(\theta) = a_{r}(\theta) + a_{r}(\pi-\theta)
\end{split}
\end{align}
and $a_{r}(\theta)$ is defined as:
\begin{equation}
a_{r}(\theta)=\frac{\theta}{\pi}(\frac{\theta}{\pi}-\frac{\theta}{n \pi}+\frac{1}{n})\exp(2r^{2}\cos(\theta))\left(1-\exp(-4r^{2}\cos^{2}(\frac{\theta}{2}))\right)^{2}.    
\end{equation}
Therefore we have:
\begin{equation}
\label{hyb-rel-error-1}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}})
\leq \frac{\exp(r^{2})}{\sqrt{m}}\sqrt{\max_{\theta \in [0, \pi]} a_{r}(\theta)}
\end{equation}
Notice that:
\begin{equation}
\label{hyb-rel-error-2}
a_{r}(\theta) \leq b_{r}(\theta)
(1-\exp(-4r^{2}))^{2}
\end{equation}
where:
\begin{equation}
b_{r}(\theta) = b^{1}_{r}(\theta) + b^{2}_{r}(\theta)   
\end{equation}
and
\begin{equation}
b^{1}_{r}(\theta) = (1-\frac{1}{n}) \frac{\theta^{2}}{\pi^{2}}\exp(2r^{2}\cos(\theta)), 
\end{equation}
\begin{equation}
b^{2}_{r}(\theta) = \frac{1}{n}\cdot\frac{\theta}{\pi} \exp(2r^{2}\cos(\theta)).         
\end{equation}
Therefore: 
\begin{equation}
\label{hyb-rel-error-3}
\max_{\theta \in [0, \pi]}b_{r}(\theta) \leq \max_{\theta \in [0, \pi] }b^{1}_{r}(\theta)+
\max_{\theta \in [0, \pi] }b^{2}_{r}(\theta)
\end{equation}
Denote: $b^{1} = \max_{\theta \in [0, \pi] }b^{1}_{r}(\theta)$ and $b^{2} = \max_{\theta \in [0, \pi] }b^{2}_{r}(\theta)$.
Note that:
\begin{equation}
\frac{d b^{1}_{r}(\theta)}{d \theta} = 
\exp(2r^{2}\cos(\theta))
(1-\frac{1}{n})\frac{2\theta}{\pi^{2}}(1-r^{2}\theta \sin(\theta)) 
\end{equation}
and
\begin{equation}
\frac{d b^{2}_{r}(\theta)}{d \theta} = 
\exp(2r^{2}\cos(\theta))\frac{1}{n \pi}(1-2r^{2}\theta \sin(\theta))
\end{equation}

Thus, from the properties of function: $\theta \rightarrow \theta \sin(\theta)$ and the fact that $r \geq 1$, we conclude that both derivatives are first nonnegative, then nonpositive and then nonnegative abd that the unique local maximum on the interval $[0, \pi]$ is achieved for $\theta \leq \frac{\pi}{2}$.
Note also that $b^1_{r}(\theta),b^1_{r}(\theta) \geq 0$ and $b^{1}_{r}(0)=b^{2}_{r}(0)=0$, $b^{1}_{r}(\pi) = (1-\frac{1}{n})\exp(-2r^{2})$, $b^{2}_{r}(\pi)=\frac{1}{n}\exp(-2r^{2})$.
We conclude that global maximum for $b^{i}_{r}$ on the interval $[0, \pi]$ for $i=1,2$ is achieved either in its unique local maximum on that interval or for $\theta=\pi$. 
Let us consider first: $b^{1}_{r}$. In its local maximum on $[0, \pi]$ we have:
\begin{equation}
\theta^{*} sin(\theta^{*}) = \frac{1}{r^{2}}    
\end{equation}
Since $\theta \leq \sin(\theta) \cdot \frac{\pi}{2}$ on $[0, \frac{\pi}{2}]$, we get:
\begin{equation}
(\theta^{*})^{2} \leq \frac{\pi}{2}\frac{1}{r^{2}}, 
\end{equation} i.e.:
\begin{equation}
\theta^{*} \leq \sqrt{\frac{\pi}{2}}\frac{1}{r}    
\end{equation}
Therefore:
\begin{equation}
b^1_{r}(\theta^{*}) \leq (1-\frac{1}{n})\frac{1}{2\pi r^{2}}\exp(2r^{2}) \geq b^{1}_{r}(\pi)    
\end{equation}
We thus conclude that:
\begin{equation}
\max_{\theta \in [0, \pi]} b^{1}_{r}(\theta) \leq (1-\frac{1}{n})\frac{1}{2\pi r^{2}}\exp(2r^{2})
\end{equation}
By the completely analogous analysis applied to $b^{2}_{r}$, we obtain:
\begin{equation}
\max_{\theta \in [0, \pi]} b^{1}_{r}(\theta) \leq \frac{1}{2n\sqrt{\pi} r^{2}}\exp(2r^{2})
\end{equation}
Now, using Equation \ref{hyb-rel-error-1},
Equation \ref{hyb-rel-error-2}, Equation \ref{hyb-rel-error-3}, we obtain:
\begin{equation}
\eps_{S(r)}(\widehat{\mathrm{SM}})^{\mathrm{hybang}}_{m,n} \leq \frac{\exp(2r^{2})}{\sqrt{2m}r}(1-\exp(-4r^{2}))\sqrt{\frac{1}{\pi} - \frac{1}{n \pi} + \frac{1}{n\sqrt{\pi}}}
\end{equation}
and that completes the first part of the proof (proof of Inequality \ref{hybang_upper}).
Equation \ref{lim_eq} is directly implied by the fact that:
\begin{equation}
\eps_{S(r)}(\widehat{\mathrm{SM}}_{m,n}^{\mathrm{hybang}}) = \frac{\exp(2r^{2})}{\sqrt{2m}}\sqrt{h_{r}(\theta)}    
\end{equation}
\end{proof}


\subsubsection{Truncated-Gaussian bipolar hybrid estimators}



If $\mathbf{x}$ and $\mathbf{y}$ have fixed L2 norm ($\|\mathbf{x}\|_2=\|\mathbf{y}\|_2=r$), we could propose a truncated gaussian hybrid estimator $\lambda: \mathbb{R} \rightarrow \mathbb{R}$ such that $\lambda(0)=0$ and $\lambda(\pi)=1$, and furthermore zeroes out the variance of $\widehat{\mathrm{SM}}^{\mathrm{hyb}}_{m,n}$ in \textbf{both}: $\theta=0$ and $\theta=\pi$:

$\lambda$ in our truncated-gaussian hybrid estimator is defined as:
\begin{equation}
\label{definition:truncated-gaussian-estimator1}
\lambda(\mathbf{x},\mathbf{y}) = \frac{1-\exp(-\frac{\sigma^2}{2}\|\mathbf{x-y}\|^{2})}{\rho} 
\end{equation}

where $\rho$ is given as:
\begin{equation}
\rho=1-\exp(-2\sigma^2r^2)
\end{equation}

The parameter $\sigma$ controls the smoothness of the gaussian kernel.

The exponential in $\lambda$ could be estimated by tri-geometric random features, and therefore we could derive the following estimator for $\lambda$:

\begin{equation}
\widehat{\lambda}(\mathbf{x},\mathbf{y}) = \frac{1}{\rho} - \frac{1}{n\rho}\sum_{i=1}^n \cos(\sigma (\omega_i^{\top}(\mathbf{x}-\mathbf{y})))
\end{equation}



Thus we can construct random feature maps for $\widehat{\lambda}_{n}(\mathbf{x},\mathbf{y}) = a - (\phi_{n}^{\lambda}(\sigma \mathbf{x}))^{\top}
\phi_{n}^{\lambda}(\sigma \mathbf{y})$ from Equation \ref{lambda-eq-estimate} by taking: 
\begin{equation}
\left\{ \begin{array}{lcl}
a = \frac{1}{\rho} \\ 
\phi_{k}^{\lambda}(\mathbf{z}) =  \frac{1}{\sqrt{n\rho}}(\sin(\tau_{1}^{\top}\mathbf{z}), \cos(\tau_{1}^{\top}\mathbf{z}),...,\sin(\tau_{n}^{\top}\mathbf{z}), \cos(\tau_{n}^{\top}\mathbf{z}))^{\top} 
\end{array}\right.
\end{equation}
where $\tau_{1},...,\tau_{n} \sim \mathcal{N}(0,\mathbf{I}_{d})$.




Using Theorem \ref{general-hybrid}, we conclude that:

\begin{theorem}[MSE of the truncated-gaussian bipolar hybrid estimator]
\label{truncated-gaussian-hybrid}
Take the truncated-gaussian bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\mathbf{x},\mathbf{y})$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\mathbf{x},\mathbf{y})$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$). Then the following holds:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\mathbf{x},\mathbf{y})) = \mathbb{E}[\widehat{\lambda}^{2}(\mathbf{x},\mathbf{y})]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})) +    
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y}))
\end{equation}

where 
\begin{equation}
\mathbb{E}[(\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \frac{1}{\rho^2}(1-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 
\end{equation}
\begin{equation}
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] =\frac{1}{\rho^2}((1-\rho)-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2
\end{equation}

Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\mathbf{x},\mathbf{y})$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\mathbf{x},\mathbf{y})$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator remains the same.

\end{theorem}



\begin{proof}

We could calculate $\mathbb{E}[(\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2]$ and $\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2]$ as follows:

\begin{equation}
\begin{split}
\mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] = \frac{1}{\rho^2} \mathbb{E}[(\rho-1+\frac{1}{n}\sum_{i=1}^n \cos(\sigma \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\ 
=\frac{(1-\rho)^2}{\rho^2}+\frac{2(\rho-1)}{\rho^2}\mathbb{E}[\cos(\sigma \omega^{\top}(\mathbf{x}-\mathbf{y}))]+\frac{1}{\rho^2}\mathbb{E}[(\frac{1}{k}\sum_{i=1}^n\cos(\sigma \omega^{\top}(\mathbf{x}-\mathbf{y})))^2] \\
= \frac{(1-\rho)^2}{\rho^2}+\frac{2(\rho-1)}{\rho^2}\exp(-\frac{\sigma^2}{2}\|\Delta\|^{2})+\frac{1}{\rho^2}\exp(-\sigma^2\|\Delta\|^2) + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 \\
= \frac{1}{\rho^2}((1-\rho)-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 
\end{split}
\end{equation}





\begin{equation}
\begin{split}
\mathbb{E}[(\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] = 1-2\mathbb{E}[1-\widehat{\lambda}(\mathbf{x},\mathbf{y})] + \mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= -1 + \frac{2}{\rho}- \frac{2}{\rho}\exp(-\frac{\sigma^2}{2}\|\Delta\|^{2}) + \mathbb{E}[(1-\widehat{\lambda}(\mathbf{x},\mathbf{y}))^2] \\
= \frac{1}{\rho^2}(1-\exp(-\frac{\sigma^2}{2}\|\Delta\|^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-\sigma^2\|\Delta\|^2))^2 
\end{split}
\end{equation}

And the theorem holds by plugging in these two parts.

Note that if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$ apply the exact same sets of random projections, then $(1-\cos(\|\mathbf{x}\|_{2}^{2}-\|\mathbf{y}\|_{2}^{2}))$ in $\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\mathbf{x},\mathbf{y}))$ becomes zero in Theorem \ref{truncated-gaussian-hybrid}, therefore the MSE remains the same.


\end{proof}





We could rewrite Eq. \ref{definition:truncated-gaussian-estimator1} and provide another definition for $\lambda$ by replacing $\mathbf{x}$ and $\mathbf{y}$ with their angle $\theta$ and norm $r$:


\begin{equation}
\label{definition:truncated-gaussian-estimator2}
\lambda(\theta,r) =  \frac{1-\exp(-2\sigma^2r^2\sin(\frac{\theta}{2})^2)}{\rho}
\end{equation}




\begin{theorem}[MSE of the truncated-gaussian bipolar hybrid estimator with $\theta$ and $r$]
\label{truncated-gaussian-hybrid2}
We could rewrite Theorem \ref{truncated-gaussian-hybrid} with $\theta$ and $r$ as follows:
Take the truncated-gaussian bipolar hybrid estimator $\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\theta,r)$,
where $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and 
$\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$ are chosen independently i.e. their random projections are chosen independently (note that we always assume that $\widehat{\lambda}(\theta,r)$ is chosen independently from $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$). Then the following holds:
\begin{equation}
\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{hybgauss}}_{m,n}(\theta,r)) = \mathbb{E}[\widehat{\lambda}^{2}(\theta,r)]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)) +    
\mathbb{E}[(1-\widehat{\lambda}(\theta,r))^{2}]\mathrm{MSE}(\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r))
\end{equation}
where 
\begin{equation}
\mathbb{E}[(\widehat{\lambda}(\theta, r))^2] = \frac{1}{\rho^2}(1-\exp(-2\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-4\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{equation}
\begin{equation}
\mathbb{E}[(1-\widehat{\lambda}(\theta, r))^2] =\frac{1}{\rho^2}((1-\rho)-\exp(-2\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2 + \frac{1}{2\rho^2 n}(1-\exp(-4\sigma^2r^2 \sin(\frac{\theta}{2})^2))^2
\end{equation}
Furthermore, if $\widehat{\mathrm{SM}}^{\mathrm{trig}}_{m}(\theta,r)$ and $\widehat{\mathrm{SM}}^{\mathrm{++}}_{m}(\theta,r)$ apply the \textbf{exact} same sets of random projections, the mean squared error of the hybrid estimator will remain the same.
\end{theorem}



\begin{proof}
For $\|x\|^2=\|y\|^2=r^2$, the following holds for $\Delta=\mathbf{x}-\mathbf{y}$:
\begin{equation}
\|\Delta\|^2 = 4r^2\sin(\frac{\theta}{2})^2
\end{equation}

And this theorem holds trivially by replacing $\|\Delta\|^2$ in Theorem \ref{truncated-gaussian-hybrid}.

\end{proof}



\subsubsection{Hybrid Gaussian-Mixtures Estimators with Clusters}



If the input matrices $\mathbf{Q}, \mathbf{K}$ can be clustered into $n_q$ and $n_k$ groups respectively (using k-means clustering algorithm for example), with the center point of each group as $\mathbf{r}_i\in \mathbb{R}^d$, ($i=1,...,n_k$) and $\mathbf{r}_j\in \mathbb{R}^d$, ($j=1,...,n_q$), then there exist $n_q n_k$ pairs of $(\mathbf{r}_i, \mathbf{r}_j)$, ($i=1,...,n_q, j=1,...,n_k$), so we can construct $n_q n_k$ softmax estimators to estimate cross-group softmax values. In the following text, we use $\mathbf{x}$ and $\mathbf{y}$ to represent a pair of such centers $\mathbf{r}_i$ and $\mathbf{r}_j$.



Consider $\mathbf{z} = \mathbf{A}\mathbf{r}_i + \mathbf{(A^{\top})^{-1}}\mathbf{r}_j$ for an invertible (in $\mathbb{C}^{d \times d})$ matrix $\mathbf{A} \in \mathbb{C}^{d \times d}$, an estimator based on this mechanism has variance equal to $0$ if:
\begin{equation}
\label{eq:z_ax_by_0}
\mathbf{z} = \mathbf{A}\mathbf{r}_i + \mathbf{(A^{\top})^{-1}}\mathbf{r}_j = 0
\end{equation}

We assume here that $\mathbf{A}$ is a diagonal matrix, so $\mathbf{A}=\mathbf{A^{\top}}$. Then we can rewrite the above equation as:
\begin{equation}
\mathbf{z} = \mathbf{A}\mathbf{r}_i + \mathbf{(A)^{-1}}\mathbf{r}_j = 0
\end{equation}

Since position $(k,k)$ in matrix $\mathbf{A}$ is a composite value with the form $\alpha_k + \beta_k i$, we need to satisfy the following equation for each k=1,...,d:
\begin{equation}
(\alpha_k + \beta_k i)r_{i,k} + \frac{1}{\alpha_k + \beta_k i}r_{j,k} = 0
\end{equation}

\begin{equation}
(\alpha_k + \beta_k i)r_{i,k} + \frac{\alpha_k - \beta_k i}{\alpha_k^2 + \beta_k^2 }r_{j,k} = 0
\end{equation}

where $r_{i,k}$ is the $k$-th entry of vector $\mathbf{r}_i$.

We can simplify this equation and separate into real and imaginary part:
\begin{equation}
\label{eq:gaussian-mixtures-with-clusters}
\left\{ \begin{array}{rcl}
\mathbf{Re}: (\alpha_k^2+\beta_k^2)\alpha_k r_{i,k} + \alpha_k r_{j,k} = 0 \\ 
\mathbf{Im}: (\alpha_k^2+\beta_k^2)\beta_k r_{i,k}- \beta_k r_{j,k} = 0 \\ 
\end{array}\right.
\end{equation}

Our goal now is to choose values for $\alpha_k$ and $\beta_k$ given $\mathbf{r}_i$ and $\mathbf{r}_j$.

If $r_{i,k} r_{j,k}>0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=0 \\ 
\beta_k=\sqrt{r_{j,k}/r_{i,k}} \\ 
\end{array}\right.
\end{equation}

And if $r_{i,k} r_{j,k}<0$, we can set:
\begin{equation}
\left\{ \begin{array}{rcl}
\alpha_k=\sqrt{-r_{j,k}/r_{i,k}} \\ 
\beta_k= 0\\ 
\end{array}\right.
\end{equation}


When $r_{i,k}=r_{i,k}=0$,  we could assume $\alpha_k=\beta_k=1$. If $r_{i,k}=0, r_{j,k}\neq 0$ or the opposite, then we cannot satisfy the above equation perfectly. We could assume $\alpha_k$ to some large positive value and set $\beta_k=0$ when $r_{i,k}=0, r_{j,k}\neq 0$, and set $\alpha_k=\beta_k$ to some small positive value close to zero when $r_{i,k}\neq0, r_{j,k}=0$. 

In the following text, we define matrix $\mathbf{A}$ calculated from Eq. \ref{eq:gaussian-mixtures-with-clusters} given $\mathbf{r}_i$ and $\mathbf{r}_j$ as $\mathbf{A}^{i,j}$.




For arbitrary vectors $\mathbf{x}, \mathbf{y} \in \mathbb{R}^d$, we know from equation (16):
\begin{equation}
\mathrm{exp}(\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2})  
\mathrm{exp}(\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2})\mathrm{SM}(\mathbf{x},\mathbf{y})  
= \mathbb{E}[\mathrm{exp}(\omega^{\top}(\mathbf{A}^{i,j}\mathbf{x}+(\mathbf{A}^{i,j})^{-1}\mathbf{y})]
\end{equation}


Therefore, the softmax can be estimated as:

\begin{equation}
\label{eq:sm_decompo}
\mathrm{SM}(\mathbf{x},\mathbf{y}) = \mathbb{E}[\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} 
\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})]
\end{equation}


with $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})$ given by:


\begin{equation}
\label{def:rfm-sm-x}
\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j}\mathbf{x}),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j}\mathbf{x}))^{\top}
\end{equation}

\begin{equation}
\label{def:rfm-sm-y}
\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y}) \overset{\mathrm{def}}{=}\mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2}) (\mathrm{exp}(\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}),...,\mathrm{exp}(\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}))^{\top}
\end{equation}

for $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$.

And such softmax estimator will have variance of zero if $\mathbf{x}=\mathbf{r}_i$ and $\mathbf{y}=\mathbf{r}_j$. For other pairs of vectors $(\mathbf{x}, \mathbf{y})$ close to $\mathbf{r}_i$ and $\mathbf{r}_j$, the variance should be small.  


We could also define the gaussian lambda coefficient estimator that gets it maximum value when $\mathbf{x}=\mathbf{r}_i, \mathbf{y}=\mathbf{r}_j$ as $\lambda^{i,j}(\mathbf{x}, \mathbf{y})$. Such estimator could be constructed with $\mathbf{A}^{i,j}$ in a similar way. 

It could be decomposed in the following manner:


\begin{align}
\begin{split}
\lambda^{i,j}(\mathbf{x}, \mathbf{y}) = \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x} + (\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2\tau^2}) 
= \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x}\|^{2}}{2\tau^2})\mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2\tau^2})\mathrm{SM}(\frac{\mathbf{x}}{\tau},\frac{\mathbf{-y}}{\tau})
\end{split}
\end{align}

where $\mathrm{SM}({\mathbf{x}}/{\tau},{\mathbf{-y}}/{\tau})$ could be estimated with similar random feature maps as given by Eq. \ref{eq:sm_decompo}.

Therefore, the gaussian lambda coefficients could be estimated as:


\begin{align}
\begin{split}
\lambda^{i,j}(\mathbf{x}, \mathbf{y}) = \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j}\mathbf{x} + (\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{2\tau^2}) = \mathbb{E}[\Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} 
\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})]
\end{split}
\end{align}

with $\Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})$ and $\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y})$ given by:


\begin{equation}
\label{def:rfm-lambda-x}
\Psi^{\tau, m}_{\mathbf{A}^{i,j}} (\mathbf{x}) =     \mathrm{exp}(-\frac{\|\mathbf{A}^{i,j} \mathbf{x}\|^{2}}{\tau^2})(\mathrm{exp}(\omega_{1}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau),...,\mathrm{exp}(\omega_{m}^{\top}\mathbf{A}^{i,j} \mathbf{x}/\tau))^{\top}
\end{equation}

\begin{equation}
\label{def:rfm-lambda-y}
\Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) =     \mathrm{exp}(-\frac{\|(\mathbf{A}^{i,j})^{-1}\mathbf{y}\|^{2}}{\tau^2})(\mathrm{exp}(-\omega_{1}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau),...,\mathrm{exp}(-\omega_{m}^{\top}(\mathbf{A}^{i,j})^{-1}\mathbf{y}/\tau))^{\top}
\end{equation}

  
for $\omega_{1},...,\omega_{m} \sim \mathcal{N}(0,\mathbf{I}_{d})$ chosen independently with $\omega$'s used in softmax estimators defined before.









\begin{definition}[Hybrid Gaussian-Mixtures Estimators with Clusters]
\label{truncated-gaussian-hybrid2}

If the matrices $\mathbf{Q}, \mathbf{K} \in \mathbb{R}^{d\times d}$ can be clustered into $n_q$ and $n_k$ groups respectively, with the center point of each group as $\mathbf{r}_i$ and $\mathbf{r}_j\in \mathbb{R}^d$, ($i=1,...,n_k$, $j=1,...,n_q$),  then we denote $\mathbf{A}^{i,j}$ as the composite matrix satisfies Eq. (\ref{eq:gaussian-mixtures-with-clusters}) with center $\mathbf{r}_i, \mathbf{r}_j$, and denote $\mathcal{E}=( \widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of the softmax-kernel $\mathrm{SM}^{i,j}(\mathbf{x},\mathbf{y})$ and $\Lambda = \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of $\lambda^{i,j}(\mathbf{x},\mathbf{y})$ constructed independently from $\mathcal{E}$.

Then our hybrid estimator takes the following:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y})
\end{equation}

with constraint:

\begin{equation}
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) = 1
\end{equation}

the lambda coefficients and softmax value are estimated with random feature maps:

\begin{equation}
\widehat{\lambda}^{i,j}(\mathbf{x}, \mathbf{y}) = \Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top} \Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y}) 
\end{equation}

\begin{equation}
\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top}\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})
\end{equation}


where $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}), \Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y}), \Psi^{\tau, m}_{\mathbf{A}^{i,j}}(\mathbf{x}), \Psi^{\tau, m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{-y})$ are given by Eq. (\ref{def:rfm-sm-x}, \ref{def:rfm-sm-y}, \ref{def:rfm-lambda-x}, \ref{def:rfm-lambda-y}).


\end{definition}




















\begin{definition}[Hybrid Zero-One-Mixtures Estimators with Clusters]
\label{truncated-gaussian-hybrid2}

If the matrices $\mathbf{Q}, \mathbf{K} \in \mathbb{R}^{d\times d}$ can be clustered into $n_q$ and $n_k$ groups respectively, with the center point of each group as $\mathbf{r}_i$ and $\mathbf{r}_j\in \mathbb{R}^d$, ($i=1,...,n_k$, $j=1,...,n_q$),  then we denote $\mathbf{A}^{i,j}$ as the composite matrix satisfying Eq. (\ref{eq:gaussian-mixtures-with-clusters}) with center $\mathbf{r}_i, \mathbf{r}_j$, and denote $\mathcal{E}=( \widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of the softmax-kernel $\mathrm{SM}^{i,j}(\mathbf{x},\mathbf{y})$ and $\Lambda = \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) )_{i=1, j=1}^{n_q, n_k}$ as a list of estimators of $\lambda^{i,j}(\mathbf{x},\mathbf{y})$ constructed independently from $\mathcal{E}$.

Then our hybrid estimator takes the following:
\begin{equation}
\widehat{\mathrm{SM}}^{\mathcal{E},\Lambda}(\mathbf{x},\mathbf{y}) = 
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y})\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y})
\end{equation}

with constraint:

\begin{equation}
\sum_{i=1}^{n_q}\sum_{j=1}^{n_k} \widehat{\lambda}^{i,j}(\mathbf{x},\mathbf{y}) = 1
\end{equation}

the lambda coefficients and softmax value are estimated with random feature maps:

\begin{equation}
\widehat{\lambda}^{i,j}(\mathbf{x}, \mathbf{y}) = \Psi_i(\mathbf{x})  \Psi_j(\mathbf{y})
\end{equation}

\begin{equation}
\widehat{\mathrm{SM}}^{i,j}(\mathbf{x},\mathbf{y}) = \Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x})^{\top}\Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})
\end{equation}


where $\Psi^{m}_{\mathbf{A}^{i,j}}(\mathbf{x}), \Psi^{m}_{(\mathbf{A}^{i,j})^{-1}}(\mathbf{y})$ are given by Eq. (\ref{def:rfm-sm-x}, \ref{def:rfm-sm-y}) and $\Psi_i(\mathbf{x})$ is a scalar indicating whether $\mathbf{x}$ belongs to the $i$-th cluster of $\mathbf{Q}$ and similarly 
$\Psi_j(\mathbf{y})$ is a scalar indicating whether $\mathbf{y}$ belongs to the $j$-th cluster of $\mathbf{K}$. 

\end{definition}

